Managed Information: A New Abstraction Mechanism for Handling Information in Software-as-a-Service

Management of information is an important aspect of every application. This includes, for example, protecting user data against breaches (like the one reported in the news about 50 million Facebook profiles being harvested for Cambridge Analytica), complying with data protection laws and regulations (like EU's new General Data Protection Regulation), coping with large databases, and retaining user data across software versions. Today, every application needs to cope with such concerns by itself and on its own. In this paper we introduce Managed Information (MI), an abstraction mechanism for managing extra-functional data related concerns, similar to how managed memory today abstracts away many memory related concerns. MI limits the access applications have to user data, which, in return, relieves them from responsibility over it. This is achieved by hosting them on a Managed Information Platform (MIP), and implementing their logic in a language that supports MI. As evidence for the feasibility of MI we describe the design and implementation of such a platform. For demonstration of MI, we describe a simple social network application built with it. The implementation is open source.

==> axiom/axiom-cljs.tex <==
\section{axiom-cljs.core}\footnote{%
	\SANITIZEDURL{http://axiom-clj.org/axiom-cljs.html}
}
%-- A Client Library
          
\subsection{connection}\par \texttt{connection} creates a connection to the host.\par It takes a URL and a the following optional keyword parameter:\begin{itemize}\item \texttt{:ws-ch}, which defaults to a function of the same name in the chord library, and\item \texttt{:atom}, which defaults to \texttt{clojure.core/atom}, and is used to construct a mutable box to place the user's identity.It returns a map containing the following keys:\item A \texttt{:sub} function for subscribing to events coming from the host.\item A \texttt{:pub} function for publishing events.\item A \texttt{:time} function which returns the current time in milliseconds.\item A \texttt{:uuid} function which returns some universally-unique identifier.\item An \texttt{:identity} atom, which will contain the user's identity once an \texttt{:init} event is received from the host.\end{itemize}
\begin{lstlisting}
connection-1
(async done
       (go
         (let [the-chan (async/chan 10)
               mock-ws-ch (fn [url]
                            (is (= url "ws://some-url"))
                            (go
                              {:ws-channel the-chan}))
               host (ax/connection "ws://some-url"
                                   :ws-ch mock-ws-ch)]
           (is (map? host))
           (is (= @(:identity host) nil)) ;; Initial value
           ;; The host sends an `:init` event
           (async/>! the-chan {:message {:kind :init
                                         :name "some/name"
                                         :identity "alice"}})
           (async/<! (async/timeout 1))
           (is (= @(:identity host) "alice"))
           
           (is (fn? (:pub host)))
           (is (fn? (:sub host)))
           (let [test-chan (async/chan 10)]
             ((:sub host) "foo" #(go (async/>! test-chan %)))
             (async/>! the-chan {:message {:name "bar" :some :event}})
             (async/>! the-chan {:message {:name "foo" :other :event}})
             (is (= (async/<! test-chan) {:name "foo" :other :event}))
             ;; Since our mock `ws-ch` creates a normal channel, publishing into this channel
             ;; will be captured by subscribers
             ((:pub host) {:message {:name "foo" :third :event}})
             (is (= (async/<! test-chan) {:name "foo" :third :event})))

           (is (fn? (:time host)))
           (let [time-before ((:time host))]
             (async/<! (async/timeout 1))
             (is (< time-before ((:time host)))))

           (is (fn? (:uuid host)))
           (is (= (count ((:uuid host))) 36))
           (is (not= ((:uuid host)) ((:uuid host))))
           (done))))
\end{lstlisting}
\par The connection map also has an \texttt{:status} field, which is an atom. It holds the value \texttt{:ok} as long as the WebSocket channel is open, and \texttt{:err} once the channel has been closed.
\begin{lstlisting}
connection-2
(async done
       (go
         (let [the-chan (async/chan 10)
               mock-ws-ch (fn [url]
                            (is (= url "ws://some-url"))
                            (go
                              {:ws-channel the-chan}))
               host (ax/connection "ws://some-url"
                                   :ws-ch mock-ws-ch)]
           (is (= @(:status host) :ok))
           (async/close! the-chan)
           (async/<! (async/timeout 1))
           (is (= @(:status host) :err))
           (done))))
\end{lstlisting}

\subsection{ws-url}\par The connection function receives as parameter a WebSocket URL to connect to. By default, this will be of the form \texttt{ws://<host>/ws}, where \texttt{<host>} represents the value of \texttt{js/document.location.host}.\par \texttt{ws-url} takes a \texttt{js/document.location} object and returns a WebSocket URL according to the above pattern.
\begin{lstlisting}
ws-url-1
    (is (= (ax/ws-url (js-obj "host" "localhost:8080")) "ws://localhost:8080/ws"))
\end{lstlisting}
\par In one case, where the host value corresponds to figwheel running on the local host, we use \texttt{localhost:8080} instead of the original host, to direct WebSockets to Axiom rather than figwheel.
\begin{lstlisting}
ws-url-2
    (is (= (ax/ws-url (js-obj "host" "localhost:3449")) "ws://localhost:8080/ws"))
\end{lstlisting}
\par If a \texttt{hash} exists in the location, and if it contains a \texttt{?},  everything right of the \texttt{?} is appended to the URL as a query string.
\begin{lstlisting}
ws-url-3
    (let [loc (js-obj "host" "localhost:8080"
                      "hash" "#foo?bar")]
      (is (= (ax/ws-url loc) "ws://localhost:8080/ws?bar")))
\end{lstlisting}
\par If a hash exists, but does not have a query string, no change is made to the URL.
\begin{lstlisting}
ws-url-4
    (let [loc (js-obj "host" "localhost:8080"
                      "hash" "#foobar")]
      (is (= (ax/ws-url loc) "ws://localhost:8080/ws")))
\end{lstlisting}
      
\subsection{update-on-dev-ver}\par When in development, Figwheel can be used to update client-side artifacts as they are being modified,  without having to reload the page. However, when updating the Cloudlog logic, we wish to update content of the [views]axiom-cljs.macros.html\#defview) and [queries](axiom-cljs.macros.html\#defquery), and that cannot be done without refreshing.\par \texttt{update-on-dev-ver} is a middleware function that can be called on a connection map, and returns a valid connection map.
\begin{lstlisting}
update-on-dev-ver-0
    (let [ps (ax/pubsub :name)
          host (->  {:sub (:sub ps)
                     :pub (fn [& _])}
                    ax/update-on-dev-ver)
          received (atom nil)]
      ((:sub host) "foo/bar" (partial reset! received))
      ((:pub ps) {:kind :fact
                  :name "foo/bar"
                  :key 1})
      (is (= @received {:kind :fact
                        :name "foo/bar"
                        :key 1})))
\end{lstlisting}
\par It subscribes to \texttt{axiom/perm-versions} events. For each such event it will set the \texttt{app-version} cookie to contain the new version, so that refreshing the browser will capture the new version.
\begin{lstlisting}
update-on-dev-ver-1
    (let [ps (ax/pubsub :name)
          published (atom [])
          host (->  {:sub (:sub ps)
                     :pub (partial swap! published conj)}
                    ax/update-on-dev-ver)
          new-ver (str "dev-" (rand-int 1000000))]
      (is (=@published [{:kind :reg
                         :name "axiom/perm-versions"}]))
      ((:pub ps) {:kind :fact
                  :name "axiom/perm-versions"
                  :key new-ver
                  :change 1})
      (is (= (.get goog.net.cookies "app-version") new-ver)))
\end{lstlisting}
\par This only applies to events with a positive \texttt{:change} (introduction of new versions),  and only applies to development versions (that begin with \texttt{dev-}).
\begin{lstlisting}
update-on-dev-ver-2
    (let [ps (ax/pubsub :name)
          host (->  {:sub (:sub ps)
                     :pub (fn [& _])}
                    ax/update-on-dev-ver)
          new-ver (str "dev-" (rand-int 1000000))]
      ((:pub ps) {:kind :fact
                  :name "axiom/perm-versions"
                  :key new-ver
                  :change 0})
      ((:pub ps) {:kind :fact
                  :name "axiom/perm-versions"
                  :key new-ver
                  :change -1})
      ((:pub ps) {:kind :fact
                  :name "axiom/perm-versions"
                  :key (str "not" new-ver)
                  :change 1})
      (is (not= (.get goog.net.cookies "app-version") new-ver))
      (is (not= (.get goog.net.cookies "app-version") (str "not" new-ver))))
\end{lstlisting}
      
\subsection{wrap-feed-forward}\par Valid events that are \texttt{:pub}lished by the client later return from the server almost unchanged. \texttt{:sub}scribers will receive these events with a certain delay. Unfortunately, this delay may cause undesired behavior, when updates to the desplay are delayed until the events return from the server-side. To overcome this problem, the \texttt{wrap-feed-forward} middleware propagates events immediately from publishers to subscribers, on the client.\par \texttt{wrap-feed-forward} wraps a connection map. It preserves the connection's properties, such that events \texttt{:pub}lished on the client are forwarded to the server, and events coming from the server are received by \texttt{:sub}scribers on the client.
\begin{lstlisting}
wrap-feed-forward-1
 (let [ps (ax/pubsub :name)
     published (atom [])
     subscribed (atom [])
     host (-> {:pub (partial swap! published conj)
               :sub (:sub ps)}
              ax/wrap-feed-forward)]
 ;; Events coming from the server
 ((:sub host) "foo" (partial swap! subscribed conj))
 ((:pub ps) {:kind :fact
             :name "foo"
             :key 1
             :data [2 3]
             :ts 1000
             :change 1
             :readers #{}
             :writers #{}})
 (is (= @subscribed [{:kind :fact
                      :name "foo"
                      :key 1
                      :data [2 3]
                      :ts 1000
                      :change 1
                      :readers #{}
                      :writers #{}}]))
 ;; Event published by the client
 ((:pub host) {:kind :fact
               :name "bar"
               :key 1
               :data [2 3]
               :ts 1000
               :change 1
               :readers #{}
               :writers #{}})
 (is (= @published [{:kind :fact
                     :name "bar"
                     :key 1
                     :data [2 3]
                     :ts 1000
                     :change 1
                     :readers #{}
                     :writers #{}}])))
\end{lstlisting}
\par However, for events published by the client, subscribers on the client get immediate response.
\begin{lstlisting}
wrap-feed-forward-2
 (let [ps (ax/pubsub :name)
     subscribed (atom [])
     host (-> {:pub (fn [& _])
               :sub (:sub ps)}
              ax/wrap-feed-forward)]
 ((:sub host) "foo" (partial swap! subscribed conj))
 ;; Event published by the client
 ((:pub host) {:kind :fact
               :name "foo"
               :key 1
               :data [2 3]
               :ts 1000
               :change 1
               :readers #{}
               :writers #{}})
 ;; is received by the client
 (is (= @subscribed [{:kind :fact
                      :name "foo"
                      :key 1
                      :data [2 3]
                      :ts 1000
                      :change 1
                      :readers #{}
                      :writers #{}}])))
\end{lstlisting}
\par \texttt{wrap-feed-forward} de-duplicates, so that once an event that was forwarded comes back from the server, it is not forwarded again to subscribers.
\begin{lstlisting}
wrap-feed-forward-3
 (let [ps (ax/pubsub :name)
     subscribed (atom [])
     host (-> {:pub (fn [& _])
               :sub (:sub ps)}
              ax/wrap-feed-forward)]
 ((:sub host) "foo" (partial swap! subscribed conj))
 ;; Event published by the client
 ((:pub host) {:kind :fact
               :name "foo"
               :key 1
               :data [2 3]
               :ts 1000
               :change 1
               :readers #{"foo"}
               :writers #{}})
 ;; and received from the server
 ((:pub ps) {:kind :fact
             :name "foo"
             :key 1
             :data [2 3]
             :ts 1000
             :change 1
             ;; The server may change the readers
             :readers #{"bar"}
             :writers #{}})
 ;; is received only once by subscribers
 (is (= (count @subscribed) 1))
 ;; However, if the event is received again it is not blocked.
 ((:pub ps) {:kind :fact
             :name "foo"
             :key 1
             :data [2 3]
             :ts 1000
             :change 1
             :readers #{"bar"}
             :writers #{}})
 (is (= (count @subscribed) 2)))
\end{lstlisting}
 
\subsection{wrap-atomic-updates}\par \texttt{wrap-atomic-updates} is a connection middleware that handles atomic updates, by treating them as two separate events.\par For normal events, \texttt{wrap-atomic-updates} does not modify the way \texttt{:sub} works.
\begin{lstlisting}
wrap-atomic-updates-1
    (let [ps (ax/pubsub :name)
          host (-> {:sub (:sub ps)}
                   ax/wrap-atomic-updates)
          published (atom [])]
      ((:sub host) "foo" (partial swap! published conj))
      ((:pub ps) {:name "foo" :key "bar" :data [1 2 3] :change 1})
      (is (= @published [{:name "foo" :key "bar" :data [1 2 3] :change 1}])))
\end{lstlisting}
\par However, for atomic updates, the subscribed function is called twice: A first time with a negative \texttt{:change} and the \texttt{:removed} value in place of \texttt{:data}, and the a second time with the original value of \texttt{:change} and \texttt{:removed} removed.
\begin{lstlisting}
wrap-atomic-updates-2
    (let [ps (ax/pubsub :name)
          host (-> {:sub (:sub ps)}
                   ax/wrap-atomic-updates)
          published (atom [])]
      ((:sub host) "foo" (partial swap! published conj))
      ((:pub ps) {:name "foo" :key "bar" :data [2 3 4] :removed [1 2 3] :change 1})
      (is (= @published [{:name "foo" :key "bar" :data [1 2 3] :change -1}
                         {:name "foo" :key "bar" :data [2 3 4] :change 1}])))
\end{lstlisting}
			 
\subsection{wrap-reg}\par The WebSocket protocol this library uses to communicate with the gateway uses a special event not used in other places of axiom: the \texttt{:reg} event. This event registers the connection to streams of \texttt{:fact} events, and possibly asks for all existing facts that match cerain criteria. The \texttt{wrap-reg} middleware is used to ensure correct semantics in situations where multiple views or queries register to the same kind of events.\par Consider a situation where two views register to the same \texttt{:fact} pattern (\texttt{:name}+\texttt{:key} combination). Since each view has its own storage atom, they will not know about each other. Each will create a \texttt{:reg} event with these \texttt{:name} and \texttt{:key} and register to incoming events. They will also set the \texttt{:get-existing} to \texttt{true}, to receive all existing facts that match. Unfortunately, since \texttt{:get-existing} was sent twice, the back-end will send two copies of each event. These events will be received by both views and so the value stored in the atom related to these events will be double its actual value on the server.\par \texttt{wrap-reg} is intended to solve this problem. It is a connection middleware that augments the connection's \texttt{:pub} method. If each \texttt{:reg} event is sent only once, the \texttt{:pub} method's behavior remains unchanged.
\begin{lstlisting}
wrap-reg-1
    (let [ps (ax/pubsub :name)
          host (-> {:pub (:pub ps)}
                   ax/wrap-reg)
          published (atom [])]
      ((:sub ps) "some/fact" (partial swap! published conj))
      ((:pub host) {:kind :reg :name "some/fact" :key 1})
      ((:pub host) {:kind :reg :name "some/fact" :key 2})
      (is (= @published [{:kind :reg :name "some/fact" :key 1}
                         {:kind :reg :name "some/fact" :key 2}])))
\end{lstlisting}
\par However, if a \texttt{:reg} event repeats itself, \texttt{wrap-reg} will make sure it is only sent to the back-end once.
\begin{lstlisting}
wrap-reg-2
    (let [ps (ax/pubsub :name)
          host (-> {:pub (:pub ps)}
                   ax/wrap-reg)
          published (atom [])]
      ((:sub ps) "some/fact" (partial swap! published conj))
      ((:pub host) {:kind :reg :name "some/fact" :key 1})
      ((:pub host) {:kind :reg :name "some/fact" :key 2})
      ((:pub host) {:kind :reg :name "some/fact" :key 1}) ;; Sent twice
      (is (= @published [{:kind :reg :name "some/fact" :key 1}
                         {:kind :reg :name "some/fact" :key 2}])))
\end{lstlisting}
\par \texttt{wrap-reg} only de-duplicates \texttt{:reg} events. Other kinds of events (e.g., \texttt{:fact}) pass normally.
\begin{lstlisting}
wrap-reg-3
    (let [ps (ax/pubsub :name)
          host (-> {:pub (:pub ps)}
                   ax/wrap-reg)
          published (atom [])]
      ((:sub ps) "some/fact" (partial swap! published conj))
      (doseq [_ (range 10)]
        ((:pub host) {:kind :fact :name "some/fact" :key 1 :data [2]}))
      (is (= (count @published) 10)))
\end{lstlisting}
      
\subsection{wrap-late-subs}\par One of the problems that exist in the pub/sub pattern is the problem of \emph{late subscribers}. A late subscriber is a subscriber that subscribes to a topic after content has already been published on that topic. In our case this could be a view function that is consulted late in the process, after another view has already requested the data it was interested in. Because we de-duplicate registration, the events are not re-sent to the new subscriber. This results in the new subscriber not having the information it needs.\par \texttt{wrap-late-subs} is intended to solve this problem by persisting all incoming events, and repeating relevant ones to new subscribers. It is a connection middleware that augments the \texttt{:sub} method. If no relevant publications have been made before the call to \texttt{:sub}, the callback will receive only new events.
\begin{lstlisting}
wrap-late-subs-1
    (let [ps (ax/pubsub :name)
          host (-> {:sub (:sub ps)}
                   ax/wrap-late-subs)
          published (atom [])]
      ((:sub host) "some/fact" (constantly nil)) ;; First subscription that causes events to come from the server
      ((:sub host) "some/fact" (partial swap! published conj)) ;; Our subscription
      ((:pub ps) {:kind :fact :name "some/fact" :key 1 :data [2]})
      ((:pub ps) {:kind :fact :name "some/fact" :key 2 :data [3]})
      (is (= @published [{:kind :fact :name "some/fact" :key 1 :data [2]}
                         {:kind :fact :name "some/fact" :key 2 :data [3]}])))
\end{lstlisting}
\par \texttt{wrap-late-subs} makes sure the order between subscribing and publishing is not important. Even if \texttt{:sub} was called after the events have already been \texttt{:pub}lished, they will still be provided to the callback.
\begin{lstlisting}
wrap-late-subs-2
    (let [ps (ax/pubsub :name)
          host (-> {:sub (:sub ps)}
                   ax/wrap-late-subs)
          published (atom [])]
      ((:sub host) "some/fact" (constantly nil)) ;; First subscription that causes events to come from the server
      ((:pub ps) {:kind :fact :name "some/fact" :key 1 :data [2]})
      ((:pub ps) {:kind :fact :name "some/fact" :key 2 :data [3]})
      ((:sub host) "some/fact" (partial swap! published conj)) ;; Our subscription
      (is (= @published [{:kind :fact :name "some/fact" :key 1 :data [2]}
                         {:kind :fact :name "some/fact" :key 2 :data [3]}])))
\end{lstlisting}
			 
\subsection{default-connection}\par \texttt{default-connection} is a high-level function intended to provide a connection-map using the default settings. It uses ws-url to create a WebSocket URL based on \texttt{js/document.location}, it calls connection to create a connection to that URL, and uses wrap-feed-forward and wrap-atomic-updates to augment this connection to work well with views and queries.

\subsection{Under the Hood}
\subsubsection{pubsub}
\par \texttt{pubsub} is a simple synchronous publish/subscribe mechanism. The \texttt{pubsub} function takes a dispatch function as parameter, and returns a map containing two functions: \texttt{:sub} and \texttt{:pub}.
\begin{lstlisting}
pubsub-1
    (let [ps (ax/pubsub (fn [x]))]
      (is (fn? (:pub ps)))
      (is (fn? (:sub ps))))
\end{lstlisting}
\par When calling the \texttt{:pub} function with a value, the dispatch function is called with that value.
\begin{lstlisting}
pubsub-2
    (let [val (atom nil)
          ps (ax/pubsub (fn [x]
                          (reset! val x)))]
      ((:pub ps) [1 2 3])
      (is (= @val [1 2 3])))
\end{lstlisting}
\par The \texttt{:sub} function takes a dispatch value, and a function. When the dispatch function returns that dispatch value, the \texttt{:sub}scribed function is called with the \texttt{:pub}lished value.
\begin{lstlisting}
pubsub-3
    (let [val (atom nil)
          ps (ax/pubsub :name)]
      ((:sub ps) "alice" (partial reset! val))
      ((:pub ps) {:name "alice" :age 28})
      ((:pub ps) {:name "bob" :age 31})
      (is (= @val {:name "alice" :age 28})))
\end{lstlisting}
      
\subsection{Testing Utilities}\par The \texttt{axiom-cljs} library provides some utility functions to help test client-side code. Consider the following code, defining a view and a reagent component for editing tasks.
\begin{lstlisting}
(defview tasks-view [me]
  [:my-app/task me task ts]
  :order-by ts)

(defn tasks-editor [host]
  (let [tasks (tasks-view host (user host))
        {:keys [add]} (meta tasks)]
    [:div
     [:h2 (str (user host) "'s Tasks")]
     [:ul (for [{:keys [ts task del! swap!]} tasks]
            [:li {:key ts}
             [:input {:value task
                      :on-change #(swap! assoc :task (.-target.value %))}]
             [:button {:on-click del!} "Done"]])]
     [:button {:on-click #(add {:ts ((:time host))
                                :task ""})} "Add Task"]]))
\end{lstlisting}
\par We build this code TDD-style, using the following tests. We use reagent-query for querying the generated UI. We start with an empty task-list. We expect to see a \texttt{:div} containing a \texttt{:h2} with the user's name.
\begin{lstlisting}
test1
(let [host (ax/mock-connection "foo")
      ui (tasks-editor host)]
  (is (= (rq/query ui :div :h2) ["foo's Tasks"])))
\end{lstlisting}
\par Now we add two tasks to the view.
\begin{lstlisting}
(defn add-two-tasks [host]
  (let [{:keys [add]} (meta (tasks-view host "foo"))]
    (add {:ts 1000
          :task "One"})
    (add {:ts 2000
          :task "Two"})))
\end{lstlisting}
\par We expect to see them as \texttt{:li} elements inside a \texttt{:ul} element. Each \texttt{:li} element should have a key attribute that matches the timestamp of a task. Additionally, it should contain an \texttt{:input} box, for which the \texttt{:value} attribute contains the task, and a button with the caption "Done".
\begin{lstlisting}
test2
(let [host (ax/mock-connection "foo")]
  (add-two-tasks host)
  (let [ui (tasks-editor host)]
    (is (= (rq/query ui :div :ul :li:key) [1000 2000]))
    (is (= (rq/query ui :div :ul :li :input:value) ["One" "Two"]))
    (is (= (rq/query ui :div :ul :li :button) ["Done" "Done"]))))
\end{lstlisting}
\par The button's \texttt{:on-click} handler removes an item from the list.
\begin{lstlisting}
test3
(let [host (ax/mock-connection "foo")]
  (add-two-tasks host)
  (let [ui (tasks-editor host)
        deleters (rq/query ui :div :ul :li :button:on-click)]
    ;; We click the first button
    ((first deleters))
    ;; We are left with "Two"
    (is (= (rq/query (tasks-editor host) :div :ul :li :input:value) ["Two"]))))
\end{lstlisting}
\par The \texttt{:input} box's \texttt{:on-change} event updates the task.
\begin{lstlisting}
test4
(let [host (ax/mock-connection "foo")]
  (add-two-tasks host)
  (let [ui (tasks-editor host)
        updaters (rq/query ui :div :ul :li :input:on-change)]
    ;; We edit the second input box
    ((second updaters) (rq/mock-change-event "Three"))
    ;; The "Two" value became "Three"
    (is (= (rq/query (tasks-editor host) :div :ul :li :input:value) ["One" "Three"]))))
\end{lstlisting}
\par A "New Task" button creates a new, empty task.
\begin{lstlisting}
test5
(let [host (-> (ax/mock-connection "foo")
               (assoc :time (constantly 555)))]
  (let [ui (tasks-editor host)]
    (is (= (rq/query ui :div :button) ["Add Task"]))
    (let [add-task (first (rq/query ui :div :button:on-click))]
      (add-task))
    ;; A new task should appear, with empty text and timestamp of 555
    (let [ui (tasks-editor host)]
      (is (= (rq/query ui :div :ul :li:key) [555]))
      (is (= (rq/query ui :div :ul :li :input:value) [""])))))
\end{lstlisting}
      
\subsubsection{mock-connection}\par To facilitate tests, \texttt{mock-connection} allows its users to create a \texttt{host} object, similar to the one created by \texttt{default-connection} and \texttt{connection}, but one that does not connect to an actual server.\par The \texttt{mock-connection} function takes one argument: the user identity, to be returned by the \texttt{user} macro.
\begin{lstlisting}
mock-connection1
    (let [host (ax/mock-connection "foo")]
      (is (= (user host) "foo")))
\end{lstlisting}
\par The resulting \texttt{host} map has \texttt{:pub} and \texttt{:sub} members that interact with each other: Publishing on \texttt{:pub} will be seen when subscribing on \texttt{:sub}.
\begin{lstlisting}
mock-connection2
    (let [host (ax/mock-connection "x")
          {:keys [pub sub]} host
          res (atom nil)]
      (sub "foo" #(reset! res (:data %)))
      (pub {:name "foo" :data 123})
      (is (= @res 123)))
\end{lstlisting}
\par The mock host also has a \texttt{:time} function, implementing a counter.
\begin{lstlisting}
mock-connection3
    (let [host (ax/mock-connection "x")
          {:keys [time]} host]
      (is (= (time) 0))
      (is (= (time) 1))
      (is (= (time) 2)))
\end{lstlisting}
      
\subsubsection{query-mock}\par A query involves both a question and answers. To mock the platform's part in a query, we need to:\begin{enumerate}\item Register to receive questions,\item Validate the question we received against the expected one, and\item Provide an answer.\end{enumerate}\par \texttt{query-mock} takes a (mock) host map and a keyword containing the name of the query we wish to mock. It returns an \textit{answer} function, one that takes the expected inputs and provided outputs for a query.\par Consider the following query, with two inputs and two outputs:
\begin{lstlisting}
(defquery foo-query [x y]
  [:something/foo x y -> z w])
\end{lstlisting}
\par In a production scenario, the query function is called at least twice: Once during the initial creation of the UI, when the results are not yet known, and another time (or times), as results start poring in from the platform.\par A test will mimic this behavior by calling the query function twice, either directly (as we do here), or indirectly, by calling the component function. The overall sequence of a typical test is the following:\begin{enumerate}\item Create a query mock function associated with the query.\item Call the UI component function (which calls the query function), expecting empty result.\item Call the query mock function with one or more results, and\item Call the UI component function once again to see the effect of the results.\end{enumerate}\par In the following code we replace the component function with calling the view function directly.
\begin{lstlisting}
query-mock1
    (let [host (ax/mock-connection "x")
          foo-mock (ax/query-mock host :something/foo)]
      ;; It is initially empty
      (is (= (foo-query host 1 2) []))
      ;; Let's add a result
      (foo-mock [1 2] [3 4])
      ;; Now we should see one result
      (is (= (foo-query host 1 2) [{:z 3 :w 4}])))
\end{lstlisting}
\par If the given inputs do not match a query that was made, an exception is thrown.
\begin{lstlisting}
query-mock2
    (let [host (ax/mock-connection "x")
          foo-mock (ax/query-mock host :something/foo)]
      ;; We call foo-mock with [1 2] without having this question asked before
      (is (thrown-with-msg? js/Error #"Query :something.foo was never executed with inputs .1 2."
                            (foo-mock [1 2] [3 4]))))
\end{lstlisting}
        
      
    

    


==> axiom/cloudlog-events.tex <==
\section{% axiom//cloudlog-events.core
	Event Processing
}\footnote{\SANITIZEDURL{http://axiom-clj.org/cloudlog-events.html}}

\subsection{Introduction}\par \texttt{defrule} and \texttt{defclause} allow users to define logic that defines applications. These macros actually define \emph{rule functions}, which are Clojure functions with metadata, intended to process \emph{facts} and create new facts based on them. See core for more details.\par The \texttt{cloudlog.events} package provides functions for applying rule functions on events. An \emph{event} is a Clojure map, containing a single change in the state of the application. This change can be an addition of a fact, a removal of a fact, or the effect of such event on the internal state of a rule. Each event contains the following fields:\begin{itemize}\item \texttt{:kind}: Either \texttt{:fact}, if this event represent a change to a fact, or \texttt{:rule} if it represents a change to a rule.\item \texttt{:name}: A string representing the name of the stream this event belongs to.  See fact-table for details.\item \texttt{:key}: The key of the fact or the rule.  See here for more details.\item \texttt{:ts}: The time (in milliseconds since EPOCH) in which this event was created (for facts.  See below for rules).\item \texttt{:data}: The data tuple representing a fact, or the state of a rule, excluding the key.\item \texttt{:change}: A number representing the change.  Typically, \texttt{1} represents addition, and \texttt{-1} represents removal.\item \texttt{:writers}: The event's \emph{writer-set}, represented as an interset.\item \texttt{:readers}: The event's \emph{reader-set}, represented as an interset.\item \texttt{:removed} (optional): If exists, account for an additional event that is identical to the original one, but with \texttt{:data} = \texttt{:removed}, and \texttt{:change} = -\texttt{:change}.\end{itemize}\par For the examples of this package we will use the following convenience function:
\begin{lstlisting}
(defn event [kind name key data & {:as ev}]
  (merge {:kind kind
          :name name
          :key key
          :data data
          :ts 1
          :change 1
          :writers #{}
          :readers #{}} ev))
\end{lstlisting}

\begin{lstlisting}
(event :fact "foo" 13 ["a" "b"] :ts 2000) => {:kind :fact
                                             :name "foo"
                                             :key 13
                                             :data ["a" "b"]
                                             :ts 2000
                                             :change 1
                                             :writers #{}
                                             :readers #{}}
 (event :fact "foo" 13 ["a" "b"] :ts 2000
      :removed ["b" "a"]) => {:kind :fact
                              :name "foo"
                              :key 13
                              :data ["a" "b"]
                              :ts 2000
                              :change 1
                              :writers #{}
                              :readers #{}
                              :removed ["b" "a"]}
\end{lstlisting}
\subsubsection{Rules}\par In this module we base our examples on the following rules defined here:
\begin{lstlisting}
(cloudlog/defrule foo-yx [y x]
  [:test/foo x y] (cloudlog/by-anyone))

(cloudlog/defrule timeline [user tweet]
  [:test/follows user author] (cloudlog/by-anyone)
  [:test/tweeted author tweet] (cloudlog/by-anyone))
\end{lstlisting}
\subsection{emitter: Create an Event-Emitting Function}\par Rules start by matching a single fact.  An emitter function takes an event representing such a fact and applies the rule function associated with the event.\par For a simple rule, the result is a sequence of derived fact.
\begin{lstlisting}
(let [em (emitter foo-yx)]
 (em (event :fact "test/foo" 2 [3]))
 => [(event :fact "cloudlog-events.core_test/foo-yx" 3 [2]
            ;; writers will be discussed later
            :writers #{"cloudlog-events.core_test"})])
\end{lstlisting}
\par For a join, the result is an event representing the \emph{rule} produced from the fact.\par Here some explanation is in order.  Our notion of facts and rules come from mathematical logic. Facts are what mathematical logic calls \emph{atoms} -- a combination of a name with some arguments, and rules are logic formulas of the form \texttt{a->b}, where the \texttt{->} operator represents logical inference. In the subset of mathematical logic we adopted, the left-hand-side of the \texttt{->} operator must be an atom (a fact).  However, the right-hand side can be any kind of axiom -- fact or rule.  With this we can create compound rules such as \texttt{a->b->c->d}, that should be read as \texttt{a->(b->(c->d))}. This means that the fact \texttt{a} implies the rule \texttt{b->c->d}, which in turn means that the fact \texttt{b} implies \texttt{c->d}, which in turn means that \texttt{c} implies \texttt{d}. In cloudlog.clj, rule functions take whatever matches the left-hand side of the rule, and emit whatever is on the right-hand side, be it a (derived) fact or a rule. Our implementation does not emit the rule syntactically.  Instead it provides a tuple that contains its underlying data.  But we still treat it as a rule.
\begin{lstlisting}
(let [em (emitter timeline)]
 (em (event :fact "test/follows" "alice" ["bob"]))
 => [(event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"]
            :writers #{"cloudlog-events.core_test"})])
\end{lstlisting}
\par The \texttt{:name} component in the produced events is derived from the name of the rule, a 'bang' (\texttt{!}) and the index of the link that emitted this event in the overall rule.  An emitter always represents the first link in a rule, so this value is always 0.
\subsubsection{Readers and Writers}\par The only parts of the event that are not easy to understand are the \texttt{:readers} and \texttt{:writers} keys. The values associated with these keys are conceptually \emph{sets of users}. \texttt{:writers} represents the set of users who \emph{may have created} the event. Each user in this set has permission to create a similar event that, e.g., can cancel the effect of this one (e.g., by creating an event with the same \texttt{:key}, \texttt{:data} \texttt{:readers} and \texttt{writers} but with a complement \texttt{:change} value) and to replace the underlying datum with another one (e.g., by creating an event with the same \texttt{:key}, \texttt{:readers} and \texttt{:writers} but different \texttt{:data}. The \texttt{:writers} set is key to how Clojure applications manage \emph{integrity}.\par When a rule is applied to a fact, the resulting event carries the \texttt{:writers} set associated with the rule, which is its namespace, for reasons we discuss in our discussion of integrity for derived facts.
\begin{lstlisting}
(let [em (emitter foo-yx)]
 (em (event :fact "test/foo" 2 [3] :writers #{:foo :bar}))
 => [(event :fact "cloudlog-events.core_test/foo-yx" 3 [2] :writers #{"cloudlog-events.core_test"})])
\end{lstlisting}
\par \texttt{:readers} represents a set of users allowed to read an axiom. We will revisit \texttt{:readers} when discussing multiplier.\par Rules may pose requirements for \texttt{:writers} and \texttt{:readers}. To support this, we pass them as metadata on the data.
\begin{lstlisting}
(let [some-rule (fn [vec]
                 (when-not (= (meta vec) {:writers #{:w}
                                          :readers #{:r}})
                   (throw (Exception. "Did not get readers and writers as meta"))))
     em (emitter some-rule)]
 (em (event :fact "something" 1 [2 3] :writers #{:w} :readers #{:r}))
 => irrelevant)
\end{lstlisting}
\subsubsection{Atomic Updates}\par When an event contains a \texttt{:removed} key, it is considered an \emph{atomic update}. The reason is that this is a single event that flows through the system,  and removes one piece of data and at the same time (\texttt{:ts}) also adds another piece or data.\par If the \texttt{:removed} field exists, two events will be emitted, one for \texttt{:data} and one for \texttt{:removed}.
\begin{lstlisting}
(let [em (emitter foo-yx)]
 (em (event :fact "test/foo" 2 [3]
            :removed [1]))
 => [(event :fact "cloudlog-events.core_test/foo-yx" 3 [2]
            :writers #{"cloudlog-events.core_test"})
     (event :fact "cloudlog-events.core_test/foo-yx" 1 [2]
            :change -1
            :writers #{"cloudlog-events.core_test"})])
\end{lstlisting}
\subsection{multiplier: Create a Function Applying Rules to Facts}\par The lowest level of event processing is taking two corresponding events  (i.e., an event for a fact and a rule with the same key) and producing a collection of events that are produced from this combination.\par A multiplier is constructed based on a rule function, and a number (>0) representing the link in the rule.
\begin{lstlisting}
(def mult1 (multiplier timeline 1))
\end{lstlisting}
\par The returned function takes two arguments: a \emph{rule event} and a matching \emph{fact event}. It returns a sequence of events created by this combination.
\begin{lstlisting}
(mult1 (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"]
             :writers #{"cloudlog-events.core_test"})
      (event :fact "test/tweeted" "bob" ["something"]))
 => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["something"]
          :writers #{"cloudlog-events.core_test"})]
\end{lstlisting}
\par We call this unit a \emph{multiplier}, because it multiplies the \texttt{:change} field of the rule and the fact event. Imagine we have \texttt{n} facts and \texttt{m} rules with a certain key.  In order to have all possible derived events we should invoke the multiplier function \texttt{n*m} times, once for each combination. Now imagine these \texttt{n} facts are actually the same fact, just added \texttt{n} times, and the \texttt{m} rules are the same rule added \texttt{m} times.  The state of the application can therefore be represented using two events, one for the fact, with \texttt{:change} value of \texttt{n}, and one for the rule with \texttt{:change} value of \texttt{m}. Now if we introduce these two events to the multiplier function, we would like to get the same result as before, that is, applying the rule to the fact \texttt{n*m} times.  To achieve this, the multiplier function multiplies the \texttt{:change} values, so that every event it returns has a \texttt{:change} value of \texttt{n*m}.
\begin{lstlisting}
(mult1 (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"] :change 2)
      (event :fact "test/tweeted" "bob" ["something"] :change 3))
 => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["something"] :change 6)]
\end{lstlisting}
\par Multiplies can handle atomic updates given in the fact:
\begin{lstlisting}
(mult1 (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"])
      (event :fact "test/tweeted" "bob" ["something else"]
             :removed ["something"]))
 => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["something else"]
          :removed ["something"])]}
\end{lstlisting}
\par ... or in the rule.
\begin{lstlisting}
(mult1 (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["eve" "bob"]
             :removed ["alice" "bob"])
      (event :fact "test/tweeted" "bob" ["something"]))
 => [(event :fact "cloudlog-events.core_test/timeline" "eve" ["something"])
   (event :fact "cloudlog-events.core_test/timeline" "alice" ["something"]
          :change -1)]
\end{lstlisting}
\subsubsection{Confidentiality}\par A multiplier is a meeting place of facts with rules, which in turn are derived from other facts. Such a meeting place is where the \emph{confidentiality} of the system is put to the test.\par Consider a dating service, where users can open \emph{tickets} with their personal details, set up a \emph{watch} for tickets that match certain criteria (for simplicity, let's say, gender, location, and age-range). A rule for creating search results can look like this:
\begin{lstlisting}
(cloudlog/defrule ticket-by-gender-and-location [[gender loc] ticket-id age]
  [:test/ticket ticket-id gender age loc] (cloudlog/by-anyone))

(cloudlog/defrule dating-matches [watch-id ticket-id]
  [:test/watch watch-id gender loc min-age max-age] (cloudlog/by-anyone)
  [ticket-by-gender-and-location [gender loc] ticket-id age] (cloudlog/by-anyone)
  (when (and (<= age max-age)
             (>= age min-age))))
\end{lstlisting}
\par \texttt{ticket-by-gender-and-location} is an indexing of raw \texttt{:test/ticket}, performed by the following rule:\par People openning tickets on dating services often wish their tickets to be limited to a certain set of users.  Similarly, people setting up a watch often wish to keep their preferences secret. These preferences are recorded in the \texttt{:readers} set of each fact. \texttt{:readers} is an interset specifying who can read this fact. Each element in \texttt{:readers} represents a \emph{named set} of users, and the \emph{readers set} for the event is an intersection of all these named sets.\par In Cloudlog, rules are not responsible for confidentiality; the Cloudlog implementation is. Imagine a Alice openning a ticket in the dating service, willing to make it visible only to  \texttt{:male} \texttt{:long-time-users} (i.e., to members of the intersection of the \texttt{:male} and \texttt{:long-time-users} named sets).  The event will look like this:
\begin{lstlisting}
(def alices-ticket-event
  (event :fact ":test/ticket" 1234 [:female 35 "NYC"]
         :readers #{:male :long-time-users}))
\end{lstlisting}
\par The \texttt{emitter} applying the \texttt{ticket-by-gender-and-location} rule will keep the \texttt{:readers} set as-is:
\begin{lstlisting}
(def ticket-by-gender-and-location-event
  (let [em (emitter ticket-by-gender-and-location)]
    (first (em alices-ticket-event))))
\end{lstlisting}
\begin{lstlisting}
(:readers ticket-by-gender-and-location-event) => #{:male :long-time-users}
\end{lstlisting}
\par When Bob looks for dates like Alice, he creates \texttt{:test/watch} with an event looking like this:
\begin{lstlisting}
(def bobs-watch-event
  (event :fact ":test/watch" 9876 [:female "NYC" 30 40]
         :readers #{:male [:user= "bob"]}))
\end{lstlisting}
\par He places only himself in the \texttt{:readers} set, so no one else will know he's looking, or what he's looking for. Bob can be seen as an intersection of all the named sets he's a member of.  One such set is \texttt{[:user= "bob"]}, a partition set that contains only him, but Bob is also a member of the \texttt{:male} set. Note that Bob is not a member of the \texttt{:long-time-users} set, since he's new to the service.\par Here too, the \texttt{emitter} function does not change the \texttt{:readers} set.
\begin{lstlisting}
(def dating-matches-event
  (let [em (emitter dating-matches)]
    (first (em bobs-watch-event))))
\end{lstlisting}
\begin{lstlisting}
(:readers dating-matches-event) => #{:male [:user= "bob"]}
\end{lstlisting}
\par Now is where things get interesting.  When the second link of the \texttt{dating-matches} rule kicks in, taking both \texttt{dating-matches-event} as the rule-event and \texttt{ticket-by-gender-and-location-event} as its fact event. What shall the \texttt{:reader} set of the result be?  That of the rule, conveying Bob's wishes, or that of the fact, conveying Alice's wishes?\par The \texttt{:readers} set of the resulting events will be an \emph{intersection} of both \texttt{:readers} sets, (which is actually a union of the Clojure sets).
\begin{lstlisting}
(let [mult (multiplier dating-matches 1)
     ev (first (mult dating-matches-event ticket-by-gender-and-location-event))]
 (:readers ev) => #{:male [:user= "bob"] :long-time-users})
\end{lstlisting}
\par The resulting \texttt{:readers} set is an intersection of \texttt{:male} and \texttt{[:user= "bob"]}, which Bob is a member of, with \texttt{:long-time-users}, which Bob is not a member of.  This places Bob outside the intersection, and therefore unable to see the resulting fact (which is what we expect).
\subsubsection{Integrity}\par Since rules take ownership over the resulting events, the \texttt{:writers} set of events coming out of a multiplier must come from the rule event:
\begin{lstlisting}
(let [mult (multiplier timeline 1)]
 (mult (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"] :writers #{"example.com"})
       (event :fact ":test/tweeted" "bob" ["hello"] :writers #{[:user= "bob"]}))
 => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["hello"] :writers #{"example.com"})])
\end{lstlisting}
\subsubsection{Timestamps}\par Events are stored with a primary key that combines \texttt{:key} and \texttt{:ts}.  Out of these, \texttt{:key} is used for sharding, and \texttt{:ts} is used for sorting. Typically, we will want to query events that share \texttt{:name} and \texttt{:key} values together, so it makes sense to store all of them together. The \texttt{:ts} provides an additional key, so we can refer to specific events that share \texttt{:name} and \texttt{:key}.\par Some event processing systems like Apache Storm guarantee at least once semantics. The advantage of this approach is that they guarantee that everything that needs to be processed gets processed, and do this at relatively low cost.  The disadvantage is that if we use such a mechanism we need to be able to cope with processing being done more than once. We cope with this in two ways:\begin{enumerate}\item All computation is declarative, meaning that if you call a rule function twice with the same input you are guaranteed to get the same output.\item We use a consistent unique key for each result, so that if we get the same result a second time, the new result gets "swallowed" by the old result.\end{enumerate}\par The unique ID we use is the timestamp -- \texttt{:ts}.  Timestamps are given to \emph{fact events} when they are created. An \texttt{emitter} function simply moves the \texttt{:ts} attribute from its input event to its output.
\begin{lstlisting}
(let [em (emitter foo-yx)
     ev (first (em (event :fact ":test/foo" 1 [2] :ts 1234)))]
 (:ts ev) => 1234)
\end{lstlisting}
\par For rule events and derived facts we use a consistent manipulation of the timestamps in the original facts being used. This makes the \texttt{:ts} lose its value as timestamp, but remain consistent and specific, so no matter when a fact and rule met, the \texttt{:ts} of their mutual products only depends on the combination of their \texttt{:ts}.\par A \texttt{multiplier} therefore needs to compute a function of the fact and rule \texttt{:ts} values. This function needs to be specific, so that the chance for a collision, (i.e., two fact/rule pairs with different \texttt{:ts} values multiplying into rules or derived facts with the same \texttt{:ts} values), is minimized. The \texttt{+} operator will not do a good job here, because, for example, the pairs \texttt{[1000 2000]} and \texttt{[1001 1999]} have the same sum. The \texttt{*} operator will do a better job, given that all our timestamps are within the same order of magnitude, but the result will be out of that range, and as we apply more multipliers the result will grow to be unnecessarily large or overflow (if \texttt{bigint} is not used). We therefore use a modular multiplication as our operation.
\begin{lstlisting}
(let [ts1 (* (bigint (rand-int 2000000000)) 1234)
     ts2 (* (bigint (rand-int 2000000000)) 1234)
     mult (multiplier timeline 1)
     ev (first (mult (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"] :ts (long ts1))
                     (event :fact ":test/tweeted" "bob" ["hello"] :ts (long ts2))))]
 (:ts ev) => (mod (* ts1 ts2) (bit-shift-left 1 48)))
\end{lstlisting}
\par Why? because we need to keep the value unique per \texttt{:key}. Consider the above example.  If we take the rule \texttt{:ts} value, the \texttt{:ts} for each entry in Alice's timeline will be the \texttt{:ts} of the rule that was applied, which takes its \texttt{:ts} from the \texttt{:test/follows} fact. This means that every tweet made by Bob will appear in Alice's timeline with the same \texttt{:ts} value, and hence tweets will overrun one another.\par But what guarantee do we have that if we take the fact's \texttt{:ts} we do not get into such a situation? There is no hard guarantee for that.  Hoever, the whole point of using rules it to denormalize the data so that it is searchable with different keys.  It is pointless to have a rule that keeps the same \texttt{:key}. Such rules can be easily converted to clauses, which do not require redundant information to be stored.
\subsection{matcher: Matches Rules and Facts}\par multipliers apply rules to facts, and expect to be given both as parameters.  However, in most cases we are only given one -- a rule or a fact, and we need to apply that rule or that fact to all matching rules and facts. These matching rule and fact events are typically stored in some database. The database can provide all events that match a combination of \texttt{:kind}, \texttt{:name} and \texttt{:key}.\par As we wish to decouple Cloudlog's implementation from any particular database, we use \texttt{core.async} channels to interact with the database.  We provide the event to be matched on a channel, along with a channel for the output, and in return \emph{someone} provides us with the matching events on the channel we provided, and closes the channel. On the other side of the channel there could be an interface to a cloud database, an in-memory cache or a combination of the two.  We don't care as long as we get what we need from the other side of the channel.\par A matcher instance is constructed by the \texttt{matcher} function, which is given a rule function, a link number and a channel to the database.
\begin{lstlisting}
(def db-chan (async/chan 1000))
(def timeline-matcher (matcher timeline 1 db-chan))
\end{lstlisting}
\subsubsection{Matching Rules for Facts}\par The returned matcher is a function that takes an event and an output channel for the resulting events.
\begin{lstlisting}
(def res-chan (async/chan 1000))
(timeline-matcher (event :fact ":test/tweeted" "bob" ["hello"]) res-chan)
\end{lstlisting}
\par The matcher will emit a query to the \texttt{db-chan}, specifying what it is looking for
\begin{lstlisting}
(def db-request
  (async/alts!! [db-chan
                 (async/timeout 1000)]))
\end{lstlisting}
\begin{lstlisting}
(-> db-request second) => db-chan
\end{lstlisting}
\par The request consists of a pair \texttt{[req chan]}, where \texttt{req} is a partial event that matches what we are looking for:
\begin{lstlisting}
(-> db-request first first) => {:kind :rule
                               :name "cloudlog-events.core_test/timeline!0"
                               :key "bob"}
\end{lstlisting}
\par And \texttt{chan} is the channel on which the database is expected to provide the reply
\begin{lstlisting}
(def reply-chan (-> db-request first second))
\end{lstlisting}
\par Next, the database emits matching rules on the reply channel, and closes it.
\begin{lstlisting}
(async/>!! reply-chan (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"]))
 (async/>!! reply-chan (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["eve" "bob"]))
 ;; The following two events should cancel one another
 (async/>!! reply-chan (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["fred" "bob"]))
 (async/>!! reply-chan (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["fred" "bob"] :change -1))
 (async/close! reply-chan)
\end{lstlisting}
\par For each such event the matcher will emit the events obtained by multiplying the fact and the rules.
\begin{lstlisting}
(async/alts!! [res-chan
              (async/timeout 1000)]) => [(event :fact "cloudlog-events.core_test/timeline" "eve" ["hello"]) res-chan]
 (async/alts!! [res-chan
              (async/timeout 1000)]) => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["hello"]) res-chan]
\end{lstlisting}
\par Finally, the channel needs to be closed.
\begin{lstlisting}
(async/alts!! [res-chan
              (async/timeout 1000)]) => [nil res-chan]
\end{lstlisting}
\subsubsection{Matching Facts for Rules}\par A matcher function can accept either a fact event or a rule event.
\begin{lstlisting}
(def res-chan (async/chan 1000))
(timeline-matcher (event :rule "cloudlog-events.core_test/timeline!0" "bob" ["alice" "bob"]) res-chan)
\end{lstlisting}
\par For a rule, the matcher will query the database for matching facts.
\begin{lstlisting}
(def db-request
  (async/alts!! [db-chan
                 (async/timeout 1000)]))
\end{lstlisting}
\begin{lstlisting}
(-> db-request second) => db-chan
\end{lstlisting}
\begin{lstlisting}
(-> db-request first first) => {:kind :fact
                               :name "test/tweeted"
                               :key "bob"}
 (def reply-chan (-> db-request first second))
\end{lstlisting}
\par Now the database replies fact events.
\begin{lstlisting}
(async/>!! reply-chan (event :fact "test/tweeted" "bob" ["hello"]))
 (async/>!! reply-chan (event :fact "test/tweeted" "bob" ["world"]))
 (async/close! reply-chan)
\end{lstlisting}
\par The results are emitted on the \texttt{res-chan}:
\begin{lstlisting}
(async/alts!! [res-chan
              (async/timeout 1000)]) => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["world"]) res-chan]
 (async/alts!! [res-chan
              (async/timeout 1000)]) => [(event :fact "cloudlog-events.core_test/timeline" "alice" ["hello"]) res-chan]
 (async/alts!! [res-chan
              (async/timeout 1000)]) => [nil res-chan]
\end{lstlisting}
\subsection{Accumulating Events}\par emitters multipliers and matchers treat each event individually. This approach is consistent with the practice of Event Sourcing. However, sometimes we wish to see the complete picture and accumulate events. The following functions support event accumulation.
\subsubsection{accumulate}\par \texttt{accumulate} is a \emph{reducing function} that accumulates events into a map for which the keys are the events themselves, excluding their \texttt{:change} and \texttt{:ts} fields, and the values are tuples, containing the sums of the \texttt{:change} and the maximum \texttt{:ts} for each entry.\par With arity 0, \texttt{accumulate} returns and empty map.
\begin{lstlisting}
(accumulate) => {}
\end{lstlisting}
\par With arity 2, it will take a map and an event, and if the event is not already a key in the map, it will be added so that the \texttt{:change} and \texttt{:ts} fields move from the key to the value.
\begin{lstlisting}
(accumulate {} (event :fact "foo/bar" "k1" [1 2] :ts 1000))
 => {(-> (event :fact "foo/bar" "k1" [1 2])
       (dissoc :change)
       (dissoc :ts)) [1 1000]}
\end{lstlisting}
\par If the event exists as a key in the map (possibly with a different \texttt{:change} and \texttt{:ts} values), the entry is updated to include the sum of the existing value and the event's \texttt{:change}, and the latest \texttt{:ts}.
\begin{lstlisting}
(accumulate {(-> (event :fact "foo/bar" "k1" [1 2])
                (dissoc :change)
                (dissoc :ts)) [1 1000]}
           (event :fact "foo/bar" "k1" [1 2] :ts 2000))
 => {(-> (event :fact "foo/bar" "k1" [1 2])
       (dissoc :change)
       (dissoc :ts)) [2 2000]}
\end{lstlisting}
\par Atomic update events are accumulated as two different events. In the following example the first event sets the value of \texttt{k1} to \texttt{[1 2]}, and the second event is an atomic update, updating its value to \texttt{[2 3]}. The accumulation shows only a single event with the updated value. (The old value is still present, but with value of 0).
\begin{lstlisting}
(reduce accumulate {}
       [(event :fact "foo/bar" "k1" [1 2] :ts 1000)
        (event :fact "foo/bar" "k1" [2 3]
               :removed [1 2] :ts 2000)])
 => {(-> (event :fact "foo/bar" "k1" [2 3])
       (dissoc :change)
       (dissoc :ts)) [1 2000]
   (-> (event :fact "foo/bar" "k1" [1 2])
       (dissoc :change)
       (dissoc :ts)) [0 2000]}
\end{lstlisting}
\subsubsection{accumulated-events}\par With an accumulated map at hand, we can get a sequence of the underlying accumulated events by calling \texttt{accumulated-events}.
\begin{lstlisting}
(set (accumulated-events {(-> (event :fact "foo/bar" "k1" [1 2])
                             (dissoc :change)
                             (dissoc :ts)) [1 1000]
                         (-> (event :fact "foo/bar" "k2" [3 4])
                             (dissoc :change)
                             (dissoc :ts)) [2 2000]}))
 => #{(event :fact "foo/bar" "k1" [1 2] :ts 1000)
    (event :fact "foo/bar" "k2" [3 4] :change 2 :ts 2000)}
\end{lstlisting}
\par Events for which the accumulated \texttt{:change} value is zero or negative are ignored.
\begin{lstlisting}
(accumulated-events {(-> (event :fact "foo/bar" "k1" [1 2])
                        (dissoc :change)
                        (dissoc :ts)) [0 9999]
                    (-> (event :fact "foo/bar" "k2" [3 4])
                        (dissoc :change)
                        (dissoc :ts)) [-1 8888]})
 => []
\end{lstlisting}
\subsubsection{accumulate-db-chan}\par Given a \texttt{database-chan}, such as the one provided for DynamoDB, and the one consumed by matchers, \texttt{accumulate-db-chan} returns a new channel which implements the same protocol but accumulates the events coming from the given database interface.\par Consider for example the following mock database, which will answer each request with the same three events:
\begin{lstlisting}
(def mock-db-chan (async/chan))
 (async/go
 (loop []
   (let [[req resp-chan] (async/<! mock-db-chan)]
     (async/>! resp-chan (event :fact "foo/bar" "k1" [1 2]))
     (async/>! resp-chan (event :fact "foo/bar" "k2" [3 4]))
     (async/>! resp-chan (event :fact "foo/bar" "k1" [1 2] :change -1))
     (async/close! resp-chan))
   (recur)))
\end{lstlisting}
\par Please note that the first and third events cancel each other. Now we use \texttt{accumulate-db-chan} to create a new channel.
\begin{lstlisting}
(def my-db-chan (accumulate-db-chan mock-db-chan))
\end{lstlisting}
\par When sending a request to \texttt{my-db-chan}, we should get the events provided on \texttt{mock-db-chan}, but accumulated.
\begin{lstlisting}
;; Read everything from the response channel
 (defn slurp-response [resp-chan]
 (loop [res #{}]
   (let [ev (async/<!! resp-chan)]
     (cond ev
           (recur (conj res ev))
           :else
           res))))

 (let [resp-chan (async/chan)]
 (async/>!! my-db-chan [{:some :request} resp-chan])
 (slurp-response resp-chan) => #{(event :fact "foo/bar" "k2" [3 4])})
\end{lstlisting}
\par This should work multiple times...
\begin{lstlisting}
(let [resp-chan (async/chan)]
 (async/>!! my-db-chan [{:some :request} resp-chan])
 (slurp-response resp-chan) => #{(event :fact "foo/bar" "k2" [3 4])})
\end{lstlisting}
\subsection{Under the Hood}
\subsubsection{split-atomic-update}\par The function \texttt{split-atomic-update} takes an event that may or may not have a \texttt{:changed} field (an atomic update), and returns a sequence of one or two events.\par For events without a \texttt{:changed} field, \texttt{split-atomic-update} returns the event as-is.
\begin{lstlisting}
(split-atomic-update (event :fact "test/tweeted" "bob" ["hello"]))
 => [(event :fact "test/tweeted" "bob" ["hello"])]
\end{lstlisting}
\par For events that do have a \texttt{:changed} field, \texttt{split-atomic-update} returns two events, one based on \texttt{:data} and the other based on \texttt{:removed}.
\begin{lstlisting}
(split-atomic-update (event :fact "test/tweeted" "bob" ["hello"]
                           :removed ["hola"]))
 => [(event :fact "test/tweeted" "bob" ["hello"])
   (event :fact "test/tweeted" "bob" ["hola"]
          :change -1)]
\end{lstlisting}
\subsubsection{join-atomic-updates}\par Given a collection of events, \texttt{join-atomic-updates} returns a possibly smaller collection of events where all events that form atomic updates are unified into single events.\par If no events match, the function returns a collection with all original events
\begin{lstlisting}
(join-atomic-updates [(event :fact "foo" "key1" [1 2 3])
                     (event :fact "foo" "key2" [2 3 4])
                     (event :fact "foo" "key3" [3 4 5])])
 => [(event :fact "foo" "key1" [1 2 3])
   (event :fact "foo" "key2" [2 3 4])
   (event :fact "foo" "key3" [3 4 5])]}
\end{lstlisting}
\par If some events match, \texttt{join-atomic-updates} joins them into a single event
\begin{lstlisting}
(join-atomic-updates [(event :fact "foo" "key1" [2 3 4])
                     (event :fact "foo" "key2" [1 2 3])
                     (event :fact "foo" "key2" [2 3 4] :change -1)
                     (event :fact "foo" "key3" [3 4 5] :change -1)])
 => [(event :fact "foo" "key1" [2 3 4])
   (event :fact "foo" "key2" [1 2 3]
          :removed [2 3 4])
   (event :fact "foo" "key3" [3 4 5] :change -1)]
\end{lstlisting}
\subsubsection{find-atomic-update}\par The key to implementing \texttt{join-atomic-updates} is being able to find, for a given event, a matching event within a given collection. \texttt{find-atomic-update} takes an event and a collection of other events, and returns a pair: \texttt{[match rest]}, where \texttt{match} is an event or \texttt{nil}, and \texttt{rest} is a collection of events.\par If the collection of events does not contain a match for the given event, \texttt{nil} and the original collection are returned.
\begin{lstlisting}
(find-atomic-update (event :fact "foo" "key1" [1 2 3])
                   [(event :fact "foo" "key1" [2 3 4])
                    (event :fact "foo" "key2" [3 4 5] :change -1)])
 => [nil [(event :fact "foo" "key1" [2 3 4])
        (event :fact "foo" "key2" [3 4 5] :change -1)]]
\end{lstlisting}
\par If the collection of events contains a match, that match is returned, and the collection is returned with the match removed.
\begin{lstlisting}
(find-atomic-update (event :fact "foo" "key1" [1 2 3])
                   [(event :fact "foo" "key1" [2 3 4])
                    (event :fact "foo" "key1" [2 3 4] :change -1)
                    (event :fact "foo" "key2" [3 4 5] :change -1)])
 => [(event :fact "foo" "key1" [2 3 4] :change -1)
   [(event :fact "foo" "key1" [2 3 4])
    (event :fact "foo" "key2" [3 4 5] :change -1)]]
\end{lstlisting}
\subsubsection{matching?}\par \texttt{matching?} takes two events and returns whether they can be unified to a single atomic update. Two events are considered to match if they share all fields except \texttt{:data} and \texttt{:change}, and the values of \texttt{:change} are the negation of one another.
\begin{lstlisting}
(matching? (event :fact "foo" "key1" [1 2 3])
          (event :fact "foo" "key1" [2 3 4] :change -1)) => true
 (matching? (event :fact "foo" "key1" [1 2 3])
          (event :fact "foo" "key1" [2 3 4])) => false
 (matching? (event :fact "foo" "key1" [1 2 3])
          (event :fact "foo" "key2" [2 3 4] :change -1)) => false
\end{lstlisting}


==> axiom/cloudlog.interset.tex <==
\section{Intersection Sets}\footnote{\SANITIZEDURL{http://axiom-clj.org/cloudlog.interset.html}}
        

          
              
\subsection{Introduction}\par In Axiom, \emph{mathematical sets} are at the base of how we provide integrity and confidentiality. Each fact is assigned a \emph{writers set} and a \emph{readers set}, representing the set of users who may have stated this fact, and the set of users allowed to know about it.\par To be able to efficiently reason upon theses sets, we need to find a Clojure representation that is both expressive enough, and efficient enough to represent and reason upon.\par Intersets (intersection sets) are the representation we chose for Axiom. Each interset is represented as either a Clojure set (a \emph{simple interset}), or a vector of such set (a \emph{canonical interset}). The Clojure sets represent \emph{intersection}, and the vectors represent \emph{union}, so together we have a set expression that represents \emph{a union of intersections} of basic components. The basic components of these sets are either \emph{strings} or \emph{vectors}, each representing an opaque set, i.e., a set one cannot further reason upon using interset operations. Strings represent identities (e.g., user-IDs), and vectors represent logic terms that are true for a set of users, such as \emph{a friend of some user X}.\par The following example interset may represent the friends of user \texttt{alice} in some application:
\begin{lstlisting}
#{[:some-app/friend "alice"]}
\end{lstlisting}
\par The following interset represents the exclusive group of users who are friends with both \texttt{alice} and \texttt{bob}:
\begin{lstlisting}
#{[:some-app/friend "alice"]
         [:some-app/friend "bob"]}
\end{lstlisting}
\par The following interset represents \texttt{alice}, but only if she's friends with \texttt{bob} (otherwise the sent is considered empty):
\begin{lstlisting}
#{"alice" [:some-app/friend "bob"]}
\end{lstlisting}
\par The following interset includes both \texttt{alice} and all of \texttt{alice}'s friends:
\begin{lstlisting}
[#{"alice"} #{[:some-app/friend "alice"]}]
\end{lstlisting}
\par The following inteset is empty, because \texttt{alice} and \texttt{bob} are two seperate identities:
\begin{lstlisting}
#{"alice" "bob"}
\end{lstlisting}
\subsection{universe and empty-set}\par The universal set is the intersection of no sets.  It is therefore:
\begin{lstlisting}
interset/universe => #{}
\end{lstlisting}
\par Similarly, the empty set is a union of no sets:
\begin{lstlisting}
interset/empty-set => []
\end{lstlisting}
\subsection{intersection}\par Intersecting two simple intersets is a union of their underlying sets:
\begin{lstlisting}
(interset/intersection #{[:some-app/friend "alice"]
                        [:some-app/friend "bob"]}
                      #{[:some-app/friend "alice"]
                        [:some-app/friend "charlie"]})
 => #{[:some-app/friend "alice"]
    [:some-app/friend "bob"]
    [:some-app/friend "charlie"]}
\end{lstlisting}
\par This is true because element \texttt{x} is a member of the intersection of intersets \texttt{A} and \texttt{B} if and only if it is a member of the both \texttt{A} and \texttt{B}.  To be a member of \texttt{A} it needs to be a member of all the named sets composing \texttt{A}, and to be a member of \texttt{B} it needs to be a member of all of \texttt{B}'s components.  Therefore, \texttt{x} needs to be a member of all the named sets composing both \texttt{A} and \texttt{B} -- their union (as Clojure sets).\par For canonical intersets we return a union of the intersections of all simple intersets on one side, with all intersets on the other side, as long as they are not disjoint.\par Consider for example two intersets containing, for \texttt{alice} and \texttt{bob} respectively, the user \emph{and} his or her friends. Intersecting these two sets will result in a 3-component canonical set:\begin{enumerate}\item Friends of both \texttt{alice} and \texttt{bob}.\item \texttt{alice}, as long as she's friends with \texttt{bob}, and\item \texttt{bob}, as long as he's friends with \texttt{alice}.The fourth combination -- the intersection of \texttt{alice} and \texttt{bob} is omitted, because the set of \emph{all \texttt{alice}s who are also \texttt{bob}s} is empty.\end{enumerate}
\begin{lstlisting}
(interset/intersection [#{[:some-app/friend "alice"]} #{"alice"}]
                      [#{[:some-app/friend "bob"]} #{"bob"}])
 => [#{[:some-app/friend "alice"]
     [:some-app/friend "bob"]}
   #{"bob" [:some-app/friend "alice"]}
   #{"alice" [:some-app/friend "bob"]}]
\end{lstlisting}
\subsection{union}\par A union of two inrsets can be acheived by concatenating their canonical forms. For example, a set containing either \texttt{alice} or \texttt{bob} is derived the following way:
\begin{lstlisting}
(interset/union #{"alice"} #{"bob"}) => [#{"alice"} #{"bob"}]
\end{lstlisting}
\par However, a union can be more minimal than that. If any of the components of the second arguments are subsets of the first argument, they are omitted.
\begin{lstlisting}
(interset/union [#{"alice"} #{"bob"}] #{"bob" [:some-app/friend "alice"]}) => [#{"alice"} #{"bob"}]
\end{lstlisting}
\subsection{subset?}\par The \texttt{subset?} predicate checks if one interset is a subset of the other.  For example:
\begin{lstlisting}
(interset/subset? #{:a} interset/universe) => true
 (interset/subset? interset/universe #{:a}) => false
 (interset/subset? #{:a} interset/empty-set) => false
 (interset/subset? interset/empty-set #{:a}) => true
 (interset/subset? (interset/intersection #{:a} #{:b}) #{:a}) => true
 (interset/subset? (interset/intersection #{:a} #{:b}) #{:c}) => false
\end{lstlisting}
\par In particular, a set is considered a subset of itself.
\begin{lstlisting}
(interset/subset? #{:a} #{:a}) => true
\end{lstlisting}
\par For simple intersets, interset \texttt{A} is subset of interset \texttt{B} if and only if Clojure set \texttt{B} is a subset of Clojure set \texttt{A}.
\begin{lstlisting}
(interset/subset? #{"alice" [:some-app/friend "bob"]}
                 #{[:some-app/friend "bob"]}) => true
 ;; but...
(interset/subset? #{[:some-app/friend "bob"]}
                  #{"alice" [:some-app/friend "bob"]}) => false
\end{lstlisting}
\par This is true because the set containing \texttt{alice} only if \texttt{alice} is friends with \texttt{bob} is a subset of \texttt{bob}'s friends.\par If the right-hand argument is a canonical interset, \texttt{subset?} returns \texttt{true} if it is true for \emph{at least one} of the right-hand argument's components.
\begin{lstlisting}
(interset/subset? #{"alice" [:some-app/friend "bob"]}
                 [#{[:some-app/friend "bob"]} #{[:some-app/friend "charlie"]}]) => true
\end{lstlisting}
\par If the left-hand argument is canonical, \texttt{subset?} returns \texttt{true} only if \emph{all} components are subsets.
\begin{lstlisting}
(interset/subset? [#{"alice" [:some-app/friend "bob"]} #{[:some-app/friend "charlie"]}]
                 [#{[:some-app/friend "bob"]} #{[:some-app/friend "charlie"]}]) => true
 ;; but...
(interset/subset? [#{"alice" [:some-app/friend "bob"]} #{[:some-app/friend "charlie"]}]
                  #{[:some-app/friend "bob"]}) => false
\end{lstlisting}
\subsection{enum-groups}\par Sometimes we wish to iterate over all groups mentioned in an interset. \texttt{enum-groups} allows us to do so by returning a sequence of these groups.\par For an empty or universal intersets, an empty sequence is returned.
\begin{lstlisting}
(interset/enum-groups interset/universe) => []
 (interset/enum-groups interset/empty-set) => []
\end{lstlisting}
\par For a simple interset, all compoments are returned.
\begin{lstlisting}
(interset/enum-groups #{[:foo "bar"] [:bar "foo"]}) => [[:foo "bar"] [:bar "foo"]]
\end{lstlisting}
\par For a cannonical interset, all components of all elements are returned.
\begin{lstlisting}
(interset/enum-groups [#{[:foo "bar"]} #{[:bar "foo"]}]) => [[:foo "bar"] [:bar "foo"]]
\end{lstlisting}
\subsection{Under the Hood}
\subsubsection{canonical}\par \texttt{canonical} takes an interset of any kind, and returns a canonical interset.\par If the given interset is already canonical, it returns the interset as-is.
\begin{lstlisting}
(interset/canonical [#{"foo"} #{"bar"}]) => [#{"foo"} #{"bar"}]}
\end{lstlisting}
\par If the given interset is a simple one, it wraps it in a vector.
\begin{lstlisting}
(interset/canonical #{"foo"}) => [#{"foo"}]
\end{lstlisting}
\subsubsection{uncanonical}\par \texttt{uncanonical} inverts the effect of \texttt{canonical}, if it is possible.\par When given a canonical interset of size 1, it returns the underlying set.
\begin{lstlisting}
(interset/uncanonical [#{"foo"}]) => #{"foo"}
\end{lstlisting}
\par When given a canonical interset with more elements, it returns the canonical interset.
\begin{lstlisting}
(interset/uncanonical [#{"foo"} #{"bar"}]) => [#{"foo"} #{"bar"}]
\end{lstlisting}
\par \texttt{uncanonical} is idempotent in the sense that calling it on a simple interset will result in the same interset.
\begin{lstlisting}
(interset/uncanonical #{"foo"}) => #{"foo"}
\end{lstlisting}

\subsubsection{disjoint?}\par Two simple intersets are (definitely) disjoint when each of them references a concrete user identity (a string), and these identities are different.\par The \texttt{disjoint?} function takes two \emph{simple} intersets and returns whether they are disjoint.\par It will return \texttt{false} if at least one of the two sets does not have an identity.
\begin{lstlisting}
(interset/disjoint? #{"foo"} #{[:some-app/friend "bar"]}) => false
\end{lstlisting}
\par In this case, \texttt{disjoint?} does not know for sure whether or not \texttt{foo} is a friend of \texttt{bar}, so it returns the safe answer \texttt{false}.\par In case each inteset has a different identity we know for sure these sets are disjoint.
\begin{lstlisting}
(interset/disjoint? #{"foo"} #{[:some-app/friend "bar"] "baz"}) => true
\end{lstlisting}
\par However, if both sets reference the same identity, they are not disjoint.
\begin{lstlisting}
(interset/disjoint? #{"foo"} #{[:some-app/friend "bar"] "foo"}) => false
\end{lstlisting}


==> axiom/gateway.tex <==
\section{gateway.core}
          
\subsection{Introduction}
\par This library implement Axiom's gateway tier. Axiom's architecture is a bit different than that of traditional web apps. The server side of traditional apps consists of a \emph{logic tier} and a \emph{data tier}. The logic tier consists of a web server that is typically extended with application code to answer requests coming from the client side (the \emph{presentation tier}). To do that it typically consults a database comprising the data tier.\par This traditional three-tier architecture puts a lot of burden on the shoulders of the logic tier. On the one hand, the client side can be malicious -- an attacker trying to make unauthorized access to user data, and on the other hand, the data tier stores plain, unencapsulated data, so it typically does not protect itself agains such attacks. The logic tier alone is thus responsible for proteecting user data against attackers, while also being responsible for properly serving the application.\par Axiom makes a different distinction between tiers on the server side. It upgrades the data tier one step up the DIKW pyramid to become an \emph{information tier}, While downgrading the logic tier to being a mere \emph{gateway} to the information tier. The information tier stores both \emph{facts} and \emph{rules}, and is capable of answering queries based on them. The facts and the rules together define the requirements in terms confidentiality and integrity. This makes it fully capable of deciding who can see what, and who can do what.\par The gateway tier provides an external interface to the information tier. Among its roles are authenticating users, querying the information tier for user rights and filtering results according to these rights. It implements an HTTP server that provides access to events -- both creating and querying them.

\subsection{identity-pred}\par Axiom has a unique method for managing user rights. Instead of checking, for each action, if a user may or may not perform that action, Axiom marks each event that flows through its information tier with two annotations: it \emph{reader set} and its \emph{writer set}. The reader set represents a mathematical set of users who are allowed to know about this event, and the writer set represents a mathematical set of users who may have caused this event. The reader sets are used to guarantee confidentiality,  while writer sets guarantee integrity.\par We treat these sets as mathematical sets, but in reality we need an efficient programatic representation for them. We use intersets for that. The intersets are expressed in terms of \emph{user groups}, which are (mathematical) sets of users that are provided by name, and not by content. Without further information it is impossible to determine if a user \texttt{u} is or is not a member of a writer set or a reader set attached to an event.\par Instead of asking the question \emph{which users belong in a readers/writers set}, the \texttt{identity-pred} function answers the opposite question: \emph{does user \texttt{u} belong to a given readers/writers set?}\par \texttt{identity-pred} is a DI resource that depends on the following resource:\begin{itemize}\item \texttt{database-chan} -- A \texttt{core.async} channel for retreiving events stored in a database (e.g., DynamoDB).\end{itemize}\par \texttt{identity-pred} is a higher-order function. It takes a user identity as parameter, and returns a predicate on user sets.
\begin{lstlisting}
(def db-chan (async/chan))
 (let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [identity-pred]
              (def nobody-in-set? (identity-pred nil))
              (def alice-in-set? (identity-pred "alice"))))
\end{lstlisting}
\par For an unauthenticated user (user ID of \texttt{nil}), the predicate returned by \texttt{identity-pred} always returns \texttt{false}. that is to say that the user does not belong to any set.
\begin{lstlisting}
(nobody-in-set? [:this :is :ignored]) => false
\end{lstlisting}
\par A porper (not \texttt{nil}) user belongs to his or her \emph{singleton group} -- a group containing only that user.
\begin{lstlisting}
(alice-in-set? #{"alice"}) => true
\end{lstlisting}
\par A user can belong to many groups, and is therefore a member of the intersection of all these groups with his or her own singleton group. But how do we determine which user belongs to which group?\par Axiom has an original solution for that as well. Instead of explicitly assigining users to groups (as some access control systems suggest), Axiom uses rules to define user groups.\par Any rule that create derived facts of the form \texttt{[rule-name user args...]} defines a user group of the form \texttt{[rule-name args...]}, which contains any \texttt{user} for which such a derived fact exists.\par Let us consider a Facebook-like application, in which users can have rights based on who their friends are, and which groups they own. Two rules: \texttt{perm.AAA/friend} and \texttt{perm.BBB/group-owner} convey this relationships, respectively. Now consider we wish to find out if \texttt{alice} is \emph{either} a \texttt{perm.AAA/friend} of \texttt{bob} or a \texttt{perm.BBB/group-owner} of "Cats for Free Speach".
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (def res (async/thread
            (alice-in-set? [#{[:perm.AAA/friend "bob"]}
                            #{[:perm.BBB/group-owner "Cats for Free Speach"]}]))))
\end{lstlisting}
\par We will use the following function to safely retrieve request made to our mock database:
\begin{lstlisting}
(defn get-query []
  (let [[req chan] (async/alts!! [db-chan
                                  (async/timeout 1000)])]
    (when (nil? req)
      (throw (Exception. "Timed out waiting for DB request")))
    req))
\end{lstlisting}
\par \texttt{alice-in-set?}, the predicate we got from \texttt{identity-pred}, queries the database for all derived facts created by these rules, where \texttt{:key} is \texttt{alice}.
\begin{lstlisting}
(let [[query reply-chan] (get-query)]
 query => {:kind :fact
           :name "perm.AAA/friend"
           :key "alice"}
 ;; Alice has two friends: bob and charlie
 (doseq [friend ["bob" "charlie"]]
   (async/>!! reply-chan {:kind :fact
                          :name "perm.AAA/friend"
                          :key "alice"
                          :data [friend]
                          :ts 1000
                          :change 1
                          :readers #{}
                          :writers #{"perm.AAA"}}))
 (async/close! reply-chan))
 (let [[query reply-chan] (get-query)]
 query => {:kind :fact
           :name "perm.BBB/group-owner"
           :key "alice"}
 ;; Alice owns two groups
 (doseq [grp ["Dogs for Free Wifi"
              "Hansters for Free Time"]]
   (async/>!! reply-chan {:kind :fact
                          :name "perm.BBB/group-owner"
                          :key "alice"
                          :data [grp]
                          :ts 2000
                          :change 1
                          :readers #{}
                          :writers #{"perm.BBB"}}))
 (async/close! reply-chan))
\end{lstlisting}
\par Because \texttt{alice} is a friend of \texttt{bob}, the result we get is \texttt{true}.
\begin{lstlisting}
(async/<!! res) => true
\end{lstlisting}
\par The predicate function caches the query results, so further calls concerning the same type of groups (in our case, \texttt{perm.AAA/friend} and \texttt{perm.BBB/group-owner}), are answered immediately.
\begin{lstlisting}
(alice-in-set? #{[:perm.AAA/friend "eve"]}) => false
 (alice-in-set? #{[:perm.BBB/group-owner "Dogs for Free Wifi"]}) => true
\end{lstlisting}
 
\subsubsection{Accumulation}\par Axiom is an event sourcing system. This means that it doesn't store \emph{state}, but rather events that record \emph{change of state}.\par When discussing user rights, we need to refer to user rights at a specific point in time. When a user makes some query, the result he or she is supposed to see depend on which groups he or she blongs to at \emph{the moment of the query}. To know this, we need to look at an accumulation of the events, and not at the individual events, that is, the current state of each group and not the individual changes in this state.\par For example, consider \texttt{alice} was once a friend of \texttt{eve} and then they parted ways. When checking if \texttt{alice} belongs to \texttt{eve}'s friends, the answer will be \texttt{false}.
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (let [alice-in-set?
       (di/do-with! \$ [identity-pred]
                    (identity-pred "alice"))
       res (async/thread
             (alice-in-set? #{[:perm.AAA/friend "eve"]}))
       [query reply-chan] (get-query)]
   (doseq [[ts change] [[1000 1] ;; Became friends at time 1000
                        [2000 -1] ;; Parted ways at time 2000
                        ]]
     (async/>!! reply-chan {:kind :fact
                            :name "perm.AAA/friend"
                            :key "alice"
                            :data ["eve"]
                            :ts ts
                            :change change
                            :writers #{"perm.AAA"}
                            :readers #{}}))
   (async/close! reply-chan)
   (async/<!! res) => false))
\end{lstlisting}
   
\subsubsection{Integrity}\par Integrity and confidentiality are important to take into consideration when calculating a user's identity set.\par Integrity is important because we do not want users to be able to assume permissions they are not entitled to. This could happen if they publish a fact that looks like a derived fact from a rule giving them access to something the wouldn't have otherwise.\par To avoid this kind of problem we require that facts taken into consideration by \texttt{identity-pred} are created by rules,  so that their writer sets include the fact's namespace.\par Imagine \texttt{eve} wishing to gain access to \texttt{alice}'s inner-circle by forging an event that makes her one of \texttt{alice}'s friends.
\begin{lstlisting}
(def forged-event
  {:kind :fact
   :name "perm.AAA/friend"
   :key "eve"
   :data ["alice"]
   :ts 3000
   :change 1
   :writers #{"eve"}
   :readers #{}})
\end{lstlisting}
\par Note the \texttt{:writers} set in this event. \texttt{eve} can only set it to a set she is a member of. Specifically, she cannot pose as \texttt{perm.AAA} -- the identity associated with the rule.\par When \texttt{eve} tries to access Axiom and perform operations (such as reading statuses on our Facebook-like application), the gateway tier will first consult \texttt{identity-pred} to see whether or not she has access to the requested content. As she will try to pose as \texttt{alice}'s friend, the predicate function will query \texttt{perm.AAA/friend} facts. However, it will only consider facts created by the \texttt{perm.AAA/friend} \emph{rule}, by checking for \texttt{perm.AAA} in the \texttt{:writers} set.
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (let [eve-in-set?
       (di/do-with! \$ [identity-pred]
                    (identity-pred "eve"))
       res (async/thread
             (eve-in-set? #{[:perm.AAA/friend "alice"]}))
       [query reply-chan] (get-query)]
   (async/>!! reply-chan forged-event)
   (async/close! reply-chan)
   (async/<!! res) => false))
\end{lstlisting}
   
\subsubsection{Confidentiality}\par The role confidentiality plays here is a bit less obvious. While the results of the queries made by the predicate function are not visible to users directly, if we do not take special measures to prefent this, users can indirectly learn about things they should not.\par Consider a private message written by \texttt{alice} to \texttt{bob}:
\begin{lstlisting}
(def bobs-message
  {:kind :fact
   :name "social-app/message"
   :key "bob"
   :data ["alice" "I like you!"]
   :ts 1234
   :change 1
   :writers #{"alice"}
   :readers #{"bob"}})
\end{lstlisting}
\par Note that the \texttt{:readers} set includes only \texttt{bob}, so \texttt{bob} alone can see this message or even know it exists.\par \texttt{eve} suspects \texttt{alice}'s effection to \texttt{bob}, and is willing to go through extreme measures to see if she is correct. To do so she creates her own application, and submits code containing the following rule:
\begin{lstlisting}
(clg/defrule evil-plan ["eve" msg]
  [:social-app/message "bob" "alice" msg] (clg/by "alice"))
\end{lstlisting}
\par Note that although the message facts were created by a different application, Axiom does not restrict facts to be used only by that application. This is a fundemental principle in Axiom: User data belongs to \emph{users}, not \emph{applications}.\par If we apply \texttt{eve}'s rule to \texttt{bob}'s message we get the following event:
\begin{lstlisting}
(let [em (ev/emitter evil-plan)]
 (def evil-facts (em bobs-message))
 evil-facts => [{:kind :fact
                 :name "gateway.core-test/evil-plan"
                 :key "eve"
                 :data ["I like you!"]
                 :ts 1234
                 :change 1
                 :writers #{"gateway.core-test"}
                 :readers #{"bob"}}])
\end{lstlisting}
\par Axiom's confidentiality mechanism made sure that although it was \texttt{eve}'s evil rule that created this event, \texttt{eve} herself cannot read it, as its \texttt{:readers} set contains only \texttt{bob}.\par But this is where \texttt{identity-pred} could (potentially) help \texttt{eve} with her plan. Her exploit consists of the following facts she stores in Axiom:
\begin{lstlisting}
[{:kind :fact
  :name "eve-the-evil/exploit"
  :key "love-life"
  :data ["It's toast"]
  :ts 2345
  :change 1
  :writers #{"eve"}
  :readers #{[[:gateway.core-test/evil-plan "I like you!"]]}}
 {:kind :fact
  :name "eve-the-evil/exploit"
  :key "love-life"
  :data ["It's over"]
  :ts 2346
  :change 1
  :writers #{"eve"}
  :readers #{[[:gateway.core-test/evil-plan "I love you!"]]}}
 {:kind :fact
  :name "eve-the-evil/exploit"
  :key "love-life"
  :data ["There's still hope..."]
  :ts 2347
  :change 1
  :writers #{"eve"}
  :readers #{[[:gateway.core-test/evil-plan "I hate you!"]]}}]
\end{lstlisting}
\par In all these facts she sets the \texttt{:readers} set to groups defined by the rule she created herself. Each of these facts will be visible to her if \texttt{alice} sent \texttt{bob} a message with the text that appears in the group's description.\par Now all \texttt{eve} has to do is make a query (through the gateway) and look for a fact \texttt{eve-the-evil/exploit} with key \texttt{love-life},  providing \texttt{gateway.core-test/evil-plan} in the rule-list. Then she just needs to wait and see if any of her guesses got lucky (or unlucky...).\par To make sure \texttt{eve}'s evel plan cannot succeed,  predicate functions returned by \texttt{identity-pred} only takes into consideration results for which the user for which the query is made is allowed to know about. In our case, \texttt{eve} is not allowed to know about the different \texttt{gateway.core-test/evil-plan} results, and therefore she is not considered a member of these groups.
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (let [eve-in-set?
       (di/do-with! \$ [identity-pred]
                    (identity-pred "eve"))
       res (async/thread
             (eve-in-set? #{[:gateway.core-test/evil-plan "I like you!"]}))
       [query reply-chan] (get-query)]
   (async/pipe (async/to-chan evil-facts) reply-chan)
   (async/<!! res) => false))
\end{lstlisting}
\par One subtle point to note is the potentially circular relationship between a user's identity set and the confidentiality requirement. We need to know what a user's identity set is in order to know what facts to consider for the identity set. We resolve this circular relationship by making the confidentiality requirement event more strict than it (theorecitally) have to be. For the purpose of group membership (the identity set) we only consider facts that are accessible to the user itself, without looking up group membership.
   
\subsection{authenticator}\par The starting point for identity-pred is an authenticated user identity. But how do we get one? In practice, user authentication is a difficult problem with many possibilities and serious trade-offs between them. In this library we defer this problem. Instead of defining a single authentication scheme, we provide an extension point in the form of a DI resource, and expect concrete implementations to implement it.\par The interface we define here is simple. An authenticator is a Ring middleware, that is, a higher-order function that takes and returns a Ring handler. It should be placed after middleware for parsing the request, e.g., handling cookies and parameters, but before any middleware that performs operations on behalf of a user.\par Upon successful authentication, an \texttt{:identity} field should be added to the request map.

\subsubsection{dummy-authenticator}\par To define this extension point, as well as to allow testing of this library and "raw" Axiom in general, we provide an \emph{unsafe}, \texttt{dummy-authenticator} which does something you are not supposed to do on the internet: trust the user... The \texttt{dummy-authenticator} takes the user's identity from a query parameter or a cookie.\par The \texttt{dummy-authenticator} is based on the \texttt{:use-dummy-authenticator} configuration parameter. If it exists (regardless of its value), a \texttt{dummy-authenticator} will be provided as the \texttt{authenticator}.
\begin{lstlisting}
(let [\$ (di/injector {:use-dummy-authenticator true})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [authenticator]
              (def dummy-authenticator authenticator)))
\end{lstlisting}
\par \texttt{dummy-authenticator} assumes the existence of \texttt{:cookies} and \texttt{:params} keys in the request, so the cookie and params middleware should be wrapped around it.\par If a request contains a cookie named \texttt{user\_identity}, the dummy authenticator takes its value as the user's identity.
\begin{lstlisting}
(let [id (atom nil)
     handler (fn [req]
               (reset! id (:identity req))
               {:status 200
                :body "hi"})
     app (-> handler
             dummy-authenticator)]
 (app {:cookies {"user_identity" {:value "foobar"}}
       :params {}})
 @id => "foobar")
\end{lstlisting}
\par If a query parameter named \texttt{\_identity} exists, its value becomes the \texttt{:identity}. Additionally, the new value is stored in a cookie for future reference.
\begin{lstlisting}
(let [handler (fn [req]
               {:body (str "Hello, " (:identity req))})
     app (-> handler
             dummy-authenticator)]
 (app {:cookies {}
       :params {"_identity" "barfoo"}})
 => {:body "Hello, barfoo"
     :cookies {"user_identity" {:value "barfoo"}}})
\end{lstlisting}
\par Adding a cookie works in concert with other cookies...
\begin{lstlisting}
(let [handler (fn [req]
               {:body "Hello"
                :cookies {"some" {:value "cookie"}}})
     app (-> handler
             dummy-authenticator)]
 (app {:cookies {}
       :params {"_identity" "barfoo"}})
 => {:body "Hello"
     :cookies {"user_identity" {:value "barfoo"}
               "some" {:value "cookie"}}})
\end{lstlisting}
\par If both a cookie and a parameter exist with different identity values, the \emph{parameter wins}.
\begin{lstlisting}
(let [id (atom nil)
     handler (fn [req]
               (reset! id (:identity req))
               {:status 200
                :body "hi"})
     app (-> handler
             dummy-authenticator)]
 (app {:cookies {"user_identity" {:value "foobar"}}
       :params {"_identity" "barfoo"}})
 @id => "barfoo")
\end{lstlisting}
\par If none are present, the authenticator does not add an \texttt{:identity} entry to the request.
\begin{lstlisting}
(let [handler (fn [req]
               (when (contains? req :identity)
                 (throw (Exception. "Request should not have an :identity field")))
               {:body "Hello"})
     app (-> handler
             dummy-authenticator)]
 (app {:cookies {}
       :params {}})
 => {:body "Hello"})
\end{lstlisting}
 
 
\subsection{version-selector}\par Axiom is intended to be multi-tenant. In is not only intended to host multiple applications, but also to host different \emph{versions} of the same application. Control over this allows features to be introduced gradually and things like A/B testing.\par A \texttt{version-selector} in Axiom is a DI resource that acts as Ring middleware, and adds a \texttt{:app-version} key to the request.

\subsubsection{cookie-version-selector}\par The most straightforward way to determine a version is by taking it off a cookie. By managing versions in cookies, applications can manipulate them through Javascript. The \texttt{cookie-version-selector} is a middleware function that does just that. It assumes a \texttt{:cookies} field exists in the request (i.e., the cookies middleware is wrapping it), and that a cookie named \texttt{app-version} is defined. It copies its content to the \texttt{:app-version} key in the request.
\begin{lstlisting}
(let [ver (atom nil)
     handler (fn [req]
               (reset! ver (:app-version req))
               {:status 200})
     app (cookie-version-selector handler)]
 (app {:cookies {"app-version" {:value "ver123"}}})
 @ver => "ver123")
\end{lstlisting}
\par While the name does not so indicate, the \texttt{cookie-version-selector} can also take a version value from a parameter \texttt{\_ver}.
\begin{lstlisting}
(let [ver (atom nil)
     handler (fn [req]
               (reset! ver (:app-version req))
               {:status 200})
     app (cookie-version-selector handler)]
 (app {:params {"_ver" "ver234"}}) => {:status 200
                                       :cookies {"app-version" {:value "ver234"}}}
 @ver => "ver234")
\end{lstlisting}
 
\subsubsection{Picking a Version based on Domain}\par But how do we get the initial version value? The complete answer is complicated and involves a few factors. The best way to determine a version starts with the domain name. Since Axiom is multi-tenant, different applications are expected to have different domain names. The application provides own their domains, and direct traffic to an instance of Axiom by managing DNS records. The \texttt{HOST} HTTP header conveys the domain name used by the user when accessing the application, and can be used to determine which application needs to run. But how do we determine the version?\par First, we need to know who to trust. We want to take the domain owner's word for it. A common way to establish this kind of trust is by asking the domain owner to set up some \texttt{TXT} DNS record, with some fixed text and his or her identity, Something like: \texttt{TXT: Axiom Identity: foo@example.com}, where \texttt{foo@example.com} is an identity verifyable by the authenticator we use. This tells Axiom the the owner of the domain trusts the mentioned user to manage content in Axiom for that domain.\par The mapping between domain names and user identities should be queried using a DNS lookup and cached. Then a query should be made for a fact stated by that user, connecting the domain to a version. If more than one such version exists, one of them should be picked at random. Javascript code that runs on behalf of the application can update the \texttt{app-version} cookie with another version if a random choice is not the correct one for this application.\par At this point we do not implement this selector.

\subsubsection{dummy-version-selector}\par To support development, we provide \texttt{dummy-version-selector}. It is a provider of the \texttt{version-selector} resource. It depends on \texttt{:dummy-version} -- a string containing a version.
\begin{lstlisting}
(let [\$ (di/injector {:dummy-version "ver456"})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [version-selector]
              (def ver-selector version-selector)))
\end{lstlisting}
\par If an \texttt{app-version} cookie already exists, the \texttt{dummy-version-selector} lets it be, to allow Javascript code to manipulate the version as it sees fit, and allowes the \texttt{cookie-version-selector} to expose its value as \texttt{:app-version}.
\begin{lstlisting}
(let [ver (atom nil)
     handler (fn [req]
               (reset! ver (:app-version req)))
     app (ver-selector handler)]
 (app {:cookies {"app-version" {:value "ver123"}}})
 @ver => "ver123")
\end{lstlisting}
\par If an \texttt{app-version} cookie does not exist, \texttt{dummy-version-selector} creates one with the value from \texttt{:dummy-version}.
\begin{lstlisting}
(let [ver (atom nil)
     handler (fn [req]
               (reset! ver (:app-version req)))
     app (ver-selector handler)]
 (app {:cookies {}})
 @ver => "ver456")
\end{lstlisting}
 
\subsection{static-handler}\par Axiom applications serve static files that originate in the \texttt{/static} directory of the source repository when pushing a new version. The content of these files is hashed, and the hash-code is stored in \texttt{axiom/perm-versions} events, keyed by the git version of the application.\par \texttt{static-handler} is a DI resource that provides a Ring handler for retreiving static files. It is depends on the following:\begin{enumerate}\item \texttt{version-selector}, to determine the version for which to retrieve the static file.\item \texttt{database-chan}, to retrieve \texttt{axiom/perm-versions} events.\item \texttt{hasher}, to retrieve the static content.\end{enumerate}
\begin{lstlisting}
(let [unhash (fn [h]
              (when (not= h "the-hash-code")
                (throw (Exception. (str "Bad hashcode: " h))))
              (.getBytes "the content"))
     \$ (di/injector {:dummy-version "ver123"
                     :database-chan db-chan
                     :hasher [:hash unhash]})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [static-handler]
              (def static-handler static-handler)))
\end{lstlisting}
\par \texttt{static-handler} handles requests by querying the database for the \texttt{axiom/perm-versions} for the given version.
\begin{lstlisting}
(def response (async/thread
               (static-handler {:cookies {} :uri "/foo.html"})))
 (let [[query resp-chan] (get-query)]
 query => {:kind :fact
           :name "axiom/perm-versions"
           :key "ver123"}
 (async/>!! resp-chan {:kind :fact
                       :name "axiom/perm-versions"
                       :key "ver123"
                       :data [{} {"/foo.html" "the-hash-code"}]})
 (async/close! resp-chan))
\end{lstlisting}
\par Upon receiving the response, \texttt{static-handler} gets the file's content from the hasher, and creates a \texttt{200} response.
\begin{lstlisting}
(let [[res chan] (async/alts!! [response
                               (async/timeout 1000)])]
 chan => response
 (:status res) => 200
 (:body res) => #(instance? java.io.InputStream %)
 (slurp (:body res)) => "the content"
 ;; Content-Type is assigned according to file extension
 (get-in res [:headers "Content-Type"]) => "text/html")
\end{lstlisting}
\par If the path does not exist in that version of the application, \texttt{static-handler} responds with a status of \texttt{404}.
\begin{lstlisting}
(def response
 (async/thread
   (static-handler {:cookies {}
                    :uri "/bar.html"})))
 ;; Same response as before...
 (let [[query resp-chan] (get-query)]
 (async/>!! resp-chan {:kind :fact
                       :name "axiom/perm-versions"
                       :key "ver123"
                       :data [{} {"/foo.html" "the-hash-code"}]})
 (async/close! resp-chan))
 (let [[res chan] (async/alts!! [response
                               (async/timeout 1000)])]
 chan => response
 (:status res) => 404)
\end{lstlisting}
\par If the version record cannot be found, a status of \texttt{404} is returned as well.
\begin{lstlisting}
(def response
 (async/thread
   (static-handler {:cookies {}
                    :uri "/bar.html"})))
 (let [[query resp-chan] (get-query)]
 ;; No response...
 (async/close! resp-chan))
 (let [[res chan] (async/alts!! [response
                               (async/timeout 1000)])]
 chan => response
 (:status res) => 404
 (:body res) => "No Such Version: ver123")
\end{lstlisting}
 
\subsection{event-gateway}\par \texttt{event-gateway} is a function that sets up a bidirectional event filter for events flowing between a client and a server. It is intended to support confidentiality and integrity, protecting both the connected client and the rest of the users against this client.\par It is a DI resource that depends on rule-version-verifier and identity-pred.
\begin{lstlisting}
(let [\$ (di/injector {:rule-version-verifier
                      (fn [ver writers]
                        (contains? writers (str "hash-in-" ver)))
                      :identity-pred
                      (fn [id]
                        (fn [s]
                          (interset/subset? #{id :some-cred} s)))})]
  (module \$)
  (di/startup \$)
  (di/do-with! \$ [event-gateway]
               (def event-gateway event-gateway)))
\end{lstlisting}
\par This function works on a bidirectional channel pair of the form \texttt{[c2s s2c]}, where \texttt{c2s} stands for \emph{client to server}, and \texttt{s2c} stands for \emph{server to client}. \texttt{event-gateway} takes such a pair as its first parameter, and returns such a pair. The pair it is given is intended to connect the gateway to the client (\texttt{[c-c2s c-s2c]}), and the returned pair (\texttt{[s-c2s s-s2c]}) is intended to connect the gateway to the server (e.g., to an event bridge). Apart for a channel-pair, \texttt{event-gateway} takes the \texttt{:identity} of the connected user and the \texttt{:app-version} of the application the user logged on to.
\begin{lstlisting}
(def c-c2s (async/chan 10))
 (def c-s2c (async/chan 10))
 (let [[s-c2s s-s2c] (event-gateway [c-c2s c-s2c] "alice" "ver123")]
 (def s-c2s s-c2s)
 (def s-s2c s-s2c))
\end{lstlisting}
\par Once called, events pushed to \texttt{c-c2s} flow to \texttt{s-c2s}...
\begin{lstlisting}
(async/>!! c-c2s {:kind :fact
                 :name "foo"
                 :writers #{"alice"}
                 :readers #{}})
 (async/<!! s-c2s) => {:kind :fact
                     :name "foo"
                     :writers #{"alice"}
                     :readers #{}}
\end{lstlisting}
\par ... and from \texttt{s-s2c} to \texttt{c-s2c}:
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "foo"
                 :writers #{"alice"}
                 :readers #{}})
 (async/<!! c-s2c) => {:kind :fact
                     :name "foo"
                     :writers #{"alice"}
                     :readers #{}}
\end{lstlisting}
		     
\subsubsection{Integrity Protection for the Client}\par The \texttt{event-gateway} will pass an event from the server to the client if one of three conditions hold for the event's \texttt{:writers} set. First, an event will pass if the user's \texttt{:identity-set} is included in the \texttt{:writers} set, that is, the user could have written this event.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "foo"
                 :writers #{"alice"}
                 :readers #{}})
 (let [[ev chan] (async/alts!! [c-s2c
                              (async/timeout 1000)])]
 chan => c-s2c)
\end{lstlisting}
\par Second, an event will pass if it was written by the application the client logged on to.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "foo"
                 :writers #{"hash-in-ver123"}
                 :readers #{}})
 (let [[ev chan] (async/alts!! [c-s2c
                              (async/timeout 1000)])]
 chan => c-s2c)
\end{lstlisting}
\par Third, an event will pass if it is self-verified, that is, if its \texttt{:writers} set is a subset of \texttt{\#\{ns\}}, where \texttt{ns} is the event's namespace.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "some-ns/foo"
                 :writers #{"some-ns" :some-other-cred}
                 :readers #{}})
 (let [[ev chan] (async/alts!! [c-s2c
                              (async/timeout 1000)])]
 chan => c-s2c)
\end{lstlisting}
\par However, it will be blocked in any other case.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "foo"
                 :writers #{"unauthorized"}
                 :readers #{}})
 (let [to (async/timeout 100)
     [ev chan] (async/alts!! [c-s2c to])]
 ;; We expect a timeout...
 chan => to)
\end{lstlisting}
 
\subsubsection{Integrity Protection Against Mallicious Clients}\par A mallicious client may attempt to state a fact on behalf of someone else. To protect against that, we block events for which the \texttt{:writers} set does not represent a \emph{superset} of the user's \texttt{:identity-set}. In other words, a user may only publish a fact if he or she belongs to the \texttt{:writers} set of that fact.
\begin{lstlisting}
(async/>!! c-c2s {:kind :fact
                 :name "foo"
                 :writers #{"bob" :some-cred}
                 :readers #{}})
 (let [to (async/timeout 100)
     [ev chan] (async/alts!! [s-c2s to])]
 ;; We expect a timeout...
 chan => to)
\end{lstlisting}
 
\subsubsection{Confidentiality Protection}\par For confidentiality, we need to make sure that regardless of what the client requested, events from the server only reach it if the client's \texttt{identity-set} is included in the event's \texttt{:readers} set, that is, if all possible users who can identify themselves this way are allowed to see this event.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "foo"
                 :writers #{"alice"}
                 :readers #{"not-alice" :some-cred}})
 (let [to (async/timeout 100)
     [ev chan] (async/alts!! [c-s2c to])]
 ;; We expect a timeout...
 chan => to)
\end{lstlisting}
 
\subsubsection{Ensuring Readability}\par One potential probelm that may occur in Axiom is that an event created by a user is created with a \texttt{:readers} set that does not allow that same user to read it. To eliminate this problem, the \texttt{event-gateway} checks each event created by the client, and in case the \texttt{:readers} does not include the user, the \texttt{:readers} set is modified to include the user.
\begin{lstlisting}
(defn read-from-chan [ch]
 (let [[item read-ch] (async/alts!! [ch (async/timeout 1000)])]
   (when-not (= read-ch ch)
     (throw (Exception. "Timed out trying to read from channel")))
   item))
 (async/>!! c-c2s {:kind :fact
                 :name "foo"
                 :writers #{"alice"}
                 :readers #{[:perm.AAA/friend "alice"]}}) ;; Alice is not a friend of herself
 (let [ev (read-from-chan s-c2s)]
 ev => {:kind :fact
        :name "foo"
        :writers #{"alice"}
        :readers [#{[:perm.AAA/friend "alice"]} #{"alice"}]}
 (:readers ev) => vector? ;; Midje doesn't check this by itself...
 )
\end{lstlisting}
\par This operation is only performed on \texttt{:fact} events. \texttt{:reg} events are left alone.
\begin{lstlisting}
(defn read-from-chan [ch]
 (let [[item read-ch] (async/alts!! [ch (async/timeout 1000)])]
   (when-not (= read-ch ch)
     (throw (Exception. "Timed out trying to read from channel")))
   item))
 (async/>!! c-c2s {:kind :reg
                 :name "foo"
                 :key 123})
 (let [ev (read-from-chan s-c2s)]
 ev => {:kind :reg
        :name "foo"
        :key 123})
\end{lstlisting}
	
\subsubsection{Registration Events}\par Valid \texttt{:reg}istration events should pass from client to server.
\begin{lstlisting}
(async/>!! c-c2s {:kind :reg
                 :name "foo"
                 :key "bar"})
 (let [[ev chan] (async/alts!! [s-c2s
                              (async/timeout 1000)])]
 chan => s-c2s)
\end{lstlisting}
\par However, if a \texttt{:reg} event is missing either a \texttt{:name} or a \texttt{:key}, it is blocked by the \texttt{event-gateway}.
\begin{lstlisting}
(async/>!! s-c2s {:kind :reg
                 :name "foo"})
 (async/>!! s-c2s {:kind :reg
                 :key "bar"})
 (let [to (async/timeout 100)
     [ev chan] (async/alts!! [s-c2s to])]
 ;; We expect a timeout...
 chan => to)
\end{lstlisting}
 
\subsection{name-translator}\par Axiom uses content addressing as a way to handle multiple versions of an application. While content addressing has its clear advantages, it also has the caveat that referencing content-addressed artifacts requires knowing the version hash.\par Recall that Axiom uses rules to specify user groups. In the above examples we used rule names such as \texttt{perm.AAA/friend} and \texttt{perm.BBB/group-owner}. The namespaces depicted as \texttt{perm.AAA} and \texttt{perm.BBB} are in reality long and change for every version of the rule's definition. This makes it impractical to be included in the client code.\par To solve this problem we place a \texttt{name-translator} between the client and the event-gateway (which consults these rules). The \texttt{name-translator} translates between rule-namespaces as they appear in the application's source code, while the \texttt{event-gateway} receives them with permacode hashes as namespaces.\par \texttt{name-translator} is a DI resource that depends on \texttt{database-chan} for retreiving the translation map for a specific application version.
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [name-translator]
              (def name-translator name-translator)))
\end{lstlisting}
\par The \texttt{name-translator}, like the \texttt{event-gateway}, is a bidirectional event processor. It takes as its first argument a tuple \texttt{[c2s s2c]} of \texttt{core.async} channels. As a second argument it expects the application version identifier (the \texttt{:app-version} key provided by the version-selector).
\begin{lstlisting}
(def c-c2s (async/chan 10))
 (def c-s2c (async/chan 10))
 (def fut (future (name-translator [c-c2s c-s2c] "ver123")))
\end{lstlisting}
\par Upon invocation, \texttt{name-translator} will perform a query for the \texttt{axiom/perm-versions} fact related to the given version.
\begin{lstlisting}
(let [[query ch] (get-query)]
 query => {:kind :fact
           :name "axiom/perm-versions"
           :key "ver123"}
 (async/>!! ch {:kind :fact
                :name "axiom/perm-versions"
                :key "ver123"
                :data [{'foo.core 'perm.AAA
                        'bar.core 'perm.BBB}
                       {"/foo.html" "some-hash"}]}))
\end{lstlisting}
\par It returns a pair of channels, similar to the one it received as its first argument.
\begin{lstlisting}
(let [[s-c2s s-s2c] @fut]
 (def s-c2s s-c2s)
 (def s-s2c s-s2c))
\end{lstlisting}
\par Events that do not mention a namespace associated with the version are passed as-is from side to side.
\begin{lstlisting}
(async/>!! c-c2s {:kind :fact
                 :name "some/name"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone"}
                 :readers #{}})
(read-from-chan s-c2s) => {:kind :fact
                          :name "some/name"
                          :key 123
                          :data [1 2 3]
                          :writers #{"someone"}
                           :readers #{}}
(async/>!! s-s2c {:kind :fact
                  :name "some/name"
                  :key 123
                  :data [1 2 3]
                  :writers #{"someone"}
                  :readers #{}})
(read-from-chan c-s2c) => {:kind :fact
                           :name "some/name"
                           :key 123
                           :data [1 2 3]
                           :writers #{"someone"}
                           :readers #{}}
\end{lstlisting}
\par Names in events coming from the client are translated using the translation map in the \texttt{axiom/perm-versions} event.
\begin{lstlisting}
(async/>!! c-c2s {:kind :fact
                 :name "some/name"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone"}
                 :readers #{[:foo.core/friend "someone"]}})
 (read-from-chan s-c2s) => {:kind :fact
                          :name "some/name"
                          :key 123
                          :data [1 2 3]
                          :writers #{"someone"}
                          :readers #{[:perm.AAA/friend "someone"]}}
\end{lstlisting}
\par Names in events coming from the server are translated in the other direction.
\begin{lstlisting}
(async/>!! s-s2c {:kind :fact
                 :name "some/name"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone"}
                 :readers #{[:perm.AAA/friend "someone"]}})
 (read-from-chan c-s2c) => {:kind :fact
                          :name "some/name"
                          :key 123
                          :data [1 2 3]
                          :writers #{"someone"}
                          :readers #{[:foo.core/friend "someone"]}}
\end{lstlisting}
			  
\subsubsection{Under the Hood}\par Internally, \texttt{name-translator} uses a helper function: \texttt{traslate-names}, which takes an event and a traslation map, and returns an event with all names traslated.\par When there is nothing to translate, \texttt{traslate-names} returns the event unchanged.
\begin{lstlisting}
(translate-names {:kind :fact
                 :name "some/name"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone"}
                 :readers #{}} {'foo.core 'perm.AAA})
 => {:kind :fact
   :name "some/name"
   :key 123
   :data [1 2 3]
   :writers #{"someone"}
   :readers #{}}
\end{lstlisting}
\par When the namespace of the \texttt{:name} field of the event appears in the translation table, it is translated accordingly.
\begin{lstlisting}
(translate-names {:kind :fact
                 :name "foo.core/something"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone"}
                 :readers #{}} {'foo.core 'perm.AAA})
 => {:kind :fact
   :name "perm.AAA/something"
   :key 123
   :data [1 2 3]
   :writers #{"someone"}
   :readers #{}}
\end{lstlisting}
\par Similarly, rule names inside \texttt{:writers} and \texttt{:readers} are translated.
\begin{lstlisting}
(translate-names {:kind :fact
                 :name "foo.core/something"
                 :key 123
                 :data [1 2 3]
                 :writers #{"someone" [:foo.core/bar 8]}
                 :readers #{[:foo.core/baz 15]}}
                {'foo.core 'perm.AAA})
 => {:kind :fact
   :name "perm.AAA/something"
   :key 123
   :data [1 2 3]
   :writers #{"someone" [:perm.AAA/bar 8]}
   :readers #{[:perm.AAA/baz 15]}}
\end{lstlisting}
\par If the original event does not have \texttt{:writers} or \texttt{:readers} (or both), these fields are ignored.
\begin{lstlisting}
(translate-names {:kind :fact
                 :name "foo.core/something"
                 :key 123
                 :data [1 2 3]}
                {'foo.core 'perm.AAA})
 => {:kind :fact
   :name "perm.AAA/something"
   :key 123
   :data [1 2 3]}
\end{lstlisting}
   
\subsection{websocket-handler}\par The gateway tier exposes Axiom's information tier through WebSockets. The \texttt{websocket-handler} is a RING handler that provides this functionality. It assumes it is wrapped with chord's \texttt{wrap-websocket-handler} or something equivalent, which translates WebSockets to \texttt{core.async} channels.\par \texttt{websocket-handler} is a DI resource that depends on event-gateway to filter events, name-translator to translate namespaces between the client and the server, and \texttt{event-bridge} (e.g., this) to interact with the information tier. It also depends on the middleware resources wrap-websocket-handler, authenticator and version-selector.
\begin{lstlisting}
(def pair [(async/chan 10) (async/chan 10)])
 (def ws-pair [(async/chan 10) (async/chan 10)])
 (let [\$ (di/injector {:event-gateway
                     (fn [[c-c2s c-s2c] id app-ver]
                       (let [s-c2s (async/chan 10 (comp
                                                   (map #(assoc % :id id))
                                                   (map #(assoc % :app-ver app-ver))))
                             s-s2c (async/chan 10 (comp
                                                   (map #(assoc % :id id))
                                                   (map #(assoc % :app-ver app-ver))))]
                         (async/pipe c-c2s s-c2s)
                         (async/pipe s-s2c c-s2c)
                         [s-c2s s-s2c]))
                     :name-translator
                     (fn [[c-c2s c-s2c] app-ver]
                       (let [s-c2s (async/chan 10 (map #(assoc % :trans-app-ver app-ver)))
                             s-s2c (async/chan 10 (map #(assoc % :trans-app-ver app-ver)))]
                         (async/pipe c-c2s s-c2s)
                         (async/pipe s-s2c c-s2c)
                         [s-c2s s-s2c]))
                     :event-bridge
                     (fn [[c2s s2c]]
                       (async/pipe c2s (first pair))
                       (async/pipe (second pair) s2c))
                     :version-selector
                     (fn [handler]
                       (fn [req]
                         (-> req
                             (assoc :app-version :the-app-ver)
                             handler)))
                     :authenticator
                     (fn [handler]
                       (fn [req]
                         (-> req
                             (assoc :identity :the-user-id)
                             handler)))
                     :wrap-websocket-handler
                     (fn [handler]
                       (fn [req]
                         (-> req
                             (assoc :ws-channel-pair ws-pair)
                             handler)))})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [websocket-handler]
              (def websocket-handler websocket-handler)))
\end{lstlisting}
\par \texttt{websocket-handler} is a RING handler function that assumes a \texttt{:ws-channel-pair} field exists in the request, which has the form \texttt{[c2s s2c]}, where \texttt{c2s} contains messages went from the client to the server, and \texttt{s2c} can take messages from the server to the client. (Please not that chord's \texttt{wrap-websocket-handler} provides only one channel (\texttt{:ws-channel}), which is bidirectional. We use our own \texttt{wrap-websocket-handler} middleware similar to chord's, which provides the channel as a pair). To use \texttt{websocket-handler} with \texttt{wrap-websocket-handler} one needs to add a wrapper that converts \texttt{:ws-channel} to \texttt{:ws-channel-pair}.)\par In the following example, we call the \texttt{websocket-handler} we constructed above. The first thing it does once active is pass to the client an \texttt{:init} event, containing the user's \texttt{:identity}. Then we pass two events through the channels -- one from client to server and one from server to client. We note that the event processors we mocked add the correct data.
\begin{lstlisting}
(let [[c2s s2c] ws-pair]
 (websocket-handler {})
 ;; `:init` event
 (read-from-chan s2c) => {:kind :init
                          :name "axiom/client-info"
                          :identity :the-user-id}
 ;; Client to server
 (async/>!! c2s {:foo :bar})
 (let [ev (read-from-chan (first pair))]
   (:foo ev) => :bar
   (:app-ver ev) => :the-app-ver
   (:id ev) => :the-user-id
   (:trans-app-ver ev) => :the-app-ver)
 ;; Server to client
 (async/>!! (second pair) {:bar :foo})
 (let [ev (read-from-chan s2c)]
   (:bar ev) => :foo
   (:app-ver ev) => :the-app-ver
   (:id ev) => :the-user-id
   (:trans-app-ver ev) => :the-app-ver))
\end{lstlisting}

\subsection{ring-handler}\par \texttt{ring-handler} is the main entry-point for the gateway tier.\par It is a DI resource that depends on websocket-handler and static-handler -- the two handlers it serves.
\begin{lstlisting}
(def the-handler (atom nil))
 (let [\$ (di/injector {:static-handler (fn [req]
                                       (reset! the-handler :static)
                                       {:status 200
                                        :body "foo bar"})
                     :websocket-handler (fn [req]
                                          (reset! the-handler :ws)
                                          {:status :200
                                           :body "bar foo"})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [ring-handler]
              (def ring-handler ring-handler)))
\end{lstlisting}
\par The location \texttt{/ws} is handled by the websocket-handler.
\begin{lstlisting}
(ring-handler {:request-method :get
              :uri "/ws"})
 @the-handler => :ws
\end{lstlisting}
\par Any other location is handled by the \texttt{/static} handler.
\begin{lstlisting}
(ring-handler {:request-method :get
              :uri "/something/else"})
 @the-handler => :static
\end{lstlisting}
 
\subsection{http-server}\par At its essence, the gateway tier is an HTTP server, represented by the \texttt{http-server} resource.\par As a DI resource, it depends on ring-handler to provide content, and \texttt{http-config} to provide parameters such as \texttt{:ip} and \texttt{:port}. See http-kit's documentation for the complete list.
\begin{lstlisting}
(let [\$ (di/injector {:http-config {:port 44444}
                     :ring-handler (fn [req]
                                     {:status 200
                                      :body "hello"})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [http-server]
              (let [resp @(http/get "\url{http://localhost:44444")}
                    {:keys [status headers body error]} resp]
                (when error
                  (throw error))
                status => 200
                (slurp body) => "hello"))
 (di/shutdown \$))
\end{lstlisting}
\par The server resource contains information about the server, such as its \texttt{:local-port} -- the actual port that was allocated to it on the local machine (as in the case where we provided \texttt{:port 0}, requesting it to choose a random available port).
\begin{lstlisting}
(let [\$ (di/injector {:http-config {:port 0}
                     :ring-handler (fn [req]
                                     {:status 200
                                      :body "hello"})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [http-server]
              (let [resp @(http/get (str "\url{http://localhost:"} (:local-port http-server)))
                    {:keys [status headers body error]} resp]
                (when error
                  (throw error))
                status => 200))
 (di/shutdown \$))
\end{lstlisting}
\par The \texttt{ring-handler} is wrapped with a parameters middleware, so query params are parsed into the \texttt{:params} field of the request.
\begin{lstlisting}
(let [\$ (di/injector {:http-config {:port 44444}
                     :ring-handler (fn [req]
                                     {:status 200
                                      :body (str "hello, " (get-in req [:params "name"]))})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [http-server]
              (let [resp @(http/get "\url{http://localhost:44444?name=foo")}
                    {:keys [status headers body error]} resp]
                (when error
                  (throw error))
                status => 200
                (slurp body) => "hello, foo"))
 (di/shutdown \$))
\end{lstlisting}
\par It is also wrapped with the cookies middleware.
\begin{lstlisting}
(let [\$ (di/injector {:http-config {:port 44444}
                     :ring-handler
                     (fn [req]
                       {:status 200
                        :body (str "hello, " (get-in req [:cookies "name" :value]))})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [http-server]
              (let [resp @(http/get "\url{http://localhost:44444"}
                                    {:headers {"Cookie" "name=foo"}})
                    {:keys [status headers body error]} resp]
                (when error
                  (throw error))
                status => 200
                (slurp body) => "hello, foo"))
 (di/shutdown \$))
\end{lstlisting}
 
\subsection{Under the Hood}
\subsubsection{rule-version-verifier}\par To maintain the integrity of query results, we need to associate the \texttt{:writers} set of an event to a version of an application (given as the \texttt{:app-version} key in the request).\par \texttt{rule-version-verifier} is a DI resource that depends on \texttt{database-chan}.
\begin{lstlisting}
(let [\$ (di/injector {:database-chan db-chan})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [rule-version-verifier]
              (def rule-version-verifier rule-version-verifier)))
\end{lstlisting}
\par It is a function that takes two arguments:\begin{enumerate}\item a version (the \texttt{:app-version} from the request, as provided by the version-selector), and\item the \texttt{:writers} set of an event.\end{enumerate}
\begin{lstlisting}
(def result (async/thread
             (rule-version-verifier "ver123" #{"some-hash" :something-else})))
\end{lstlisting}
\par It queries the database for a \texttt{axiom/perm-versions} fact associated with the given version.
\begin{lstlisting}
(let [[q reply-chan] (get-query)]
 q => {:kind :fact
       :name "axiom/perm-versions"
       :key "ver123"}
 (async/>!! reply-chan {:kind :fact
                        :name "axiom/perm-versions"
                        :key "ver123"
                        :data [{'foo 'some-hash
                                'bar 'some-other-hash} {}]})
 (async/close! reply-chan))
\end{lstlisting}
\par Because \texttt{some-hash} exists in the \texttt{axiom/perm-versions} for this version, the function should return \texttt{true}.
\begin{lstlisting}
(async/<!! result) => true
\end{lstlisting}
\par If the \texttt{:writers} set does not mention a hash that exists, we return \texttt{false}.
\begin{lstlisting}
(def result (async/thread
             (rule-version-verifier "ver234" #{"some-hash-that-does-not-exist" :something-else})))
 (let [[q reply-chan] (get-query)]
 q => {:kind :fact
       :name "axiom/perm-versions"
       :key "ver234"}
 (async/>!! reply-chan {:kind :fact
                        :name "axiom/perm-versions"
                        :key "ver234"
                        :data [{'foo 'some-hash
                                'bar 'some-other-hash} {}]})
 (async/close! reply-chan))
 (async/<!! result) => false
\end{lstlisting}
\par Database output is cached, so that when we ask about a version we already asked about, the answer is given without involving the database.
\begin{lstlisting}
(rule-version-verifier "ver123" #{"some-other-hash" :something-else})
 => true
 (rule-version-verifier "ver123" #{"some-hash-that-does-not-exist" :something-else})
 => false
\end{lstlisting}
\subsubsection{wrap-websocket-handler}\par \texttt{wrap-websocket-handler} is based on chord's implementation of middleware of the same name. It does the same, i.e., exposes WebSockets as \texttt{core.async} channels, but with the following differences:\begin{enumerate}\item Instead of providing one bidirectional channel in \texttt{:ws-channel}, it provides two unidirectional channels in \texttt{:ws-channel-pair}.\item It extracts the \texttt{:message} packaging, and provides raw content on the channels.\end{enumerate}\par To demonstrate how it works we will create a handler that receives maps,  and replies to each such event with a similar event, with the \texttt{:data} field (a number) incremented.
\begin{lstlisting}
(defn handler [req]
 (if-let [[ws-in ws-out] (:ws-channel-pair req)]
   (async/go-loop []
     (let [input (async/<! ws-in)
           output (update-in input [:data] inc)]
       (async/>! ws-out output)))
   ;; else
   {:status 200
    :body "No WebSockets..."}))
\end{lstlisting}
\par Now we launch a web server based on this handler with the \texttt{wrap-websocket-handler} middleware.
\begin{lstlisting}
(def srv (htsrv/run-server (-> handler
                               wrap-websocket-handler) {:port 33333}))
\end{lstlisting}
\par Now let's connect a client to that server and send a map.
\begin{lstlisting}
(def client-resp (async/chan 2))
 (def socket (ws/connect
             "ws://localhost:33333"
             :on-receive #(async/>!! client-resp %)))
 (ws/send-msg socket "{:data 1 :foo :bar}")
\end{lstlisting}
\par Now we wait for the response.
\begin{lstlisting}
(let [[resp chan] (async/alts!! [client-resp (async/timeout 1000)])]
 chan => client-resp
 resp  => "{:data 2, :foo :bar}")
\end{lstlisting}
\par Finally, let's close both server and client connections.
\begin{lstlisting}
(ws/close socket)
 (srv)}
\end{lstlisting}
\subsubsection{info-from-param-or-cookie-middleware}\par The \texttt{info-from-param-or-cookie-middleware} function takes the following parameters:\begin{enumerate}\item A key to be added to the \texttt{req},\item A parameter name (for a URL parameter), and\item A name of a cookie.It returns a middleware function.\end{enumerate}
\begin{lstlisting}
(let [wrap-foo (info-from-param-or-cookie-middleware :foo "foo-param" "foo-cookie")]
 (def handler (-> (fn [req]
                    {:req req
                     :status 200})
                  wrap-foo)))
\end{lstlisting}
\par When none of the cookie nor the param are present in a given request, it passes the request unchanged.
\begin{lstlisting}
(handler {:some :req}) => {:req {:some :req}
                          :status 200}
 (handler {:cookies {"some" {:value "cookie"}}}) => {:req {:cookies {"some" {:value "cookie"}}}
                                                   :status 200}
 (handler {:params {"some" "param"}}) => {:req {:params {"some" "param"}}
                                        :status 200}
\end{lstlisting}
\par When the request contains the specified cookie, the cookie's value is returned as the specified key.
\begin{lstlisting}
(handler {:cookies {"foo-cookie" {:value "bar"}}}) => {:req {:foo "bar"
                                                            :cookies {"foo-cookie" {:value "bar"}}}
                                                      :status 200}
\end{lstlisting}
\par When the request contains the specified parameter, it is taken for the specified key, and a cookie is set with that value.
\begin{lstlisting}
(handler {:params {"foo-param" "bar"}}) => {:req {:params {"foo-param" "bar"}
                                                 :foo "bar"}
                                           :status 200
                                           :cookies {"foo-cookie" {:value "bar"}}}
\end{lstlisting}
\par When both a cookie and a parameter exist in the request (with different values), the \emph{parameter} wins.
\begin{lstlisting}
(handler {:cookies {"foo-cookie" {:value "bar"}}
         :params {"foo-param" "baz"}}) => {:req {:params {"foo-param" "baz"}
                                                 :cookies {"foo-cookie" {:value "bar"}}
                                                 :foo "baz"}
                                           :status 200
                                           :cookies {"foo-cookie" {:value "baz"}}}
\end{lstlisting}


==> axiom/migrator.tex <==
\section{migrator.core}\footnote{\SANITIZEDURL{http://axiom-clj.org/migrator.html}}
%Initiating Data Migrations for Rules
            
\subsection{Introduction}\par \texttt{migrator} is a microservice that listens to events describing new rules being published, and initiates data migration using zk-plan.\par Consider for example the following definitions:
\begin{lstlisting}
(clg/defrule timeline [user author tweet]
  [:test/follows user author] (clg/by-anyone)
  [:test/tweeted author tweet] (clg/by-anyone))

(clg/defrule trending [tweet]
  [:test/influencer influencer] (clg/by-anyone)
  [timeline influencer tweet] (clg/by-anyone))

(def stop-words #{"a" "is" "to" "the"})
(clg/defrule index-docs [word id]
  [:test/doc id text] (clg/by-anyone)
  (for [word (clojure.string/split text #"[,!.? ]+")])
  (let [word (clojure.string/lower-case word)])
  (when-not (contains? stop-words word)))

(clg/defclause multi-keyword-search
  [:test/multi-keyword-search keywords -> text]
  (let [keywords (map clojure.string/lower-case keywords)
        first-kw (first keywords)])
  [index-docs first-kw id]
  [:test/doc id text] (clg/by-anyone)
  (let [lc-text (clojure.string/lower-case text)])
  (when (every? #(clojure.string/includes? lc-text %)
                (rest keywords))))
\end{lstlisting}
	\par If we introduce these rules when \texttt{:test/follows}, \texttt{:test/tweeted} and \texttt{:test/influencer} facts already exist, a migration process is necessary to do the following:\begin{enumerate}\item Create timeline entries for all the tweets that already have followers.\item Create trending entries based on newly-calculated timeline entries for all existing influencers.\item Create intermediate data so that new followers will receive existing tweets in their timelines.\item Create intermediate data so that new tweets will be added to the timelines of existing followers.\item Create intermediate data so that new timeline entries of existing influencers will be taken into account for trending.\end{enumerate}\par To allow this to happen, we need to go through all the \texttt{:test/follows} facts first and create intermediate rule tuples based on them. Then we need to go through all the \texttt{:test/tweeted} facts and match them against the tuples we generated in the previous step to know to which timelines each tweet needs to go. Then, after all timeline entries are calculated we can go through all influencers and create trending data.\par Going through all the existing facts with a certain name can be a lengthy process. To speed things up we do the following:\begin{itemize}\item We use zk-plan to distribute this work across multiple workers.\item We scan the facts in the database in shards, to allow different computer nodes to process different pieces of data in parallel.\end{itemize}
		
\subsection{push-handler}\par When developers push a new version of their code, they publish an \texttt{:axiom/app-version} event stating the clone URL and git commit hash for that new version. The origin of such operation could be a handler for a GitHub webhook or something similar.\par This service uses git to clone the specified version into the local file system. It relies on the following resources:\begin{enumerate}\item \texttt{sh}: A shell to run \texttt{git} commands in.\item \texttt{migration-config}: where the \texttt{:clone-location} -- the directory where all clones are performed, is specified, and the \texttt{:clone-depth}.\item deploy-dir: which publishes the contents of the git repo in the Axiom instance.\item \texttt{declare-service} and \texttt{assign-service}: which registers this function with the \texttt{:axiom/app-version} event.\end{enumerate}
\begin{lstlisting}
(def cmds (transient []))
 (def staticdir (atom nil))
 (let [decl (transient {})
     assign (transient {})
     \$ (di/injector {:sh (fn [& args]
                           (conj! cmds args)
                           {:exit 0
                            :out "some output"
                            :err ""})
                     :migration-config {:clone-location "/my/clone/location"
                                        :clone-depth 12}
                     :declare-service (fn [q partial]
                                        (assoc! decl q partial))
                     :assign-service (fn [q func]
                                       (assoc! assign q func))
                     :deploy-dir (fn [ver dir publish]
                                   (publish {:ver ver
                                             :dir dir}))})]
 (module \$)
 (di/startup \$)
 ((persistent! decl) "migrator.core/push-handler") => {:kind :fact
                                                       :name "axiom/app-version"}
 (def push-handler ((persistent! assign) "migrator.core/push-handler")))
 push-handler => fn?
\end{lstlisting}
\par The \texttt{push-handler} function responds to such events by calling \texttt{git clone} and \texttt{git checkout}  to get the specified version of the specified repo inside the given directory. Then \texttt{permacode.publish/hash-all} and \texttt{hash-static-files} are called on the local repo, and then the directory is removed.
\begin{lstlisting}
(def published (transient []))
 (push-handler {:kind :fact
              :name "axiom/app-version"
              :key "https://example.com/some/repo"
              :data ["ABCD1234"]}
             (fn [ev]
               (conj! published ev))) => nil
 (provided
(rand-int 1000000000) => 12345)
 (persistent! cmds) => [["git" "clone" "-$\,$-depth" "12" "https://example.com/some/repo" "/my/clone/location/repo12345"]
                      ["git" "checkout" "ABCD1234" :dir "/my/clone/location/repo12345"]
                      ["rm" "-rf" "/my/clone/location/repo12345"]]
\end{lstlisting}
\par The handler publishes an \texttt{:axiom/perm-versions} event, for which the key is the new version,  and the data consists of two maps:\begin{enumerate}\item A mapping between namespaces in the logic code to their permacode hashes, and\item A mapping between static resouce paths to their permacode hashes.\end{enumerate}
\begin{lstlisting}
(persistent! published) => [{:ver "ABCD1234"
                            :dir "/my/clone/location/repo12345"}]
\end{lstlisting}
\subsection{perm-tracker}\par \texttt{perm-tracker} registers to \texttt{:axiom/perm-versions} and tracks the quantity of each permacode module by summing the \texttt{:change} field of the event.\par It depends on the resources zookeeper-counter-add \texttt{declare-service} and \texttt{assign-service}, which we will mock.
\begin{lstlisting}
(def mock-counters (transient {"/perms/perm.ABCD123" 2}))
 (def calls (transient []))
 (let [\$ (di/injector {:zookeeper-counter-add (fn [path change]
                                              (let [old (mock-counters path 0)
                                                    new (+ old change)]
                                                (assoc! mock-counters path new)
                                                new))
                     :declare-service (fn [key reg] (conj! calls [:declare-service key reg]))
                     :assign-service (fn [key func] (conj! calls [:assign-service key func]))})]
 (module \$)
 (di/startup \$)
 (def calls (persistent! calls))
 (first calls) => [:declare-service "migrator.core/perm-tracker" {:kind :fact
                                                                  :name "axiom/perm-versions"}])
\end{lstlisting}
\par The function \texttt{rule-tracker} is the second argument given to \texttt{assign-service}.
\begin{lstlisting}
(let [call (second calls)]
 (take 2 call) => [:assign-service "migrator.core/perm-tracker"]
 (def rule-tracker (call 2)))
\end{lstlisting}
\par The \texttt{perm-tracker} service function is given an \texttt{:axiom/perm-versions} event and a \texttt{publish} function.
\begin{lstlisting}
(rule-tracker {:kind :fact
              :name "axiom/perm-versions"
              :key "ABCD1234"
              :data [{'foo 'perm.ABCD123} {}]
              :change 3}
             (fn publish [ev]
               (throw (Exception. "This should not be called")))) => nil
\end{lstlisting}
\par It calls \texttt{zookeeper-counter-add} to increment the counter corresponding to the rule.
\begin{lstlisting}
(mock-counters "/perms/perm.ABCD123") => 5
\end{lstlisting}
\par If one or more perms go from 0 to a positive count, an \texttt{:axiom/perms-exist} event with \texttt{:change = 1} is published.
\begin{lstlisting}
(rule-tracker {:kind :fact
              :name "axiom/perm-versions"
              :key "ABCD1234"
              :data [{'foo 'perm.ABCD123
                      'bar 'perm.EFGH456} {}]
              :change 3} ..pub..) => nil
 (provided
(..pub.. {:kind :fact
          :name "axiom/perms-exist"
          :key "ABCD1234"
          :data [#{'perm.EFGH456}]
          :change 1}) => irrelevant)
\end{lstlisting}
\par This of-course only happens when the change is positive.
\begin{lstlisting}
(rule-tracker {:kind :fact
              :name "axiom/perm-versions"
              :key "ABCD1234"
              :data [{'foobar 'perm.FOOBAR} {}]
              :change -3} (fn publish [ev]
                            (throw (Exception. "This should not be called")))) => nil
\end{lstlisting}
\par If the aggregated value of the rule goes down to 0, an \texttt{:axiom/perms-exist} event with \texttt{:change = -1} is published.
\begin{lstlisting}
(rule-tracker {:kind :fact
              :name "axiom/perm-versions"
              :key "ABCD1234"
              :data [{'foo 'perm.ABCD123
                      'bar 'perm.EFGH456} {}]
              :change -3} ..pub..) => nil
 (provided
(..pub.. {:kind :fact
          :name "axiom/perms-exist"
          :key "ABCD1234"
          :data [#{'perm.EFGH456}]
          :change -1}) => irrelevant)
\end{lstlisting}
	  
\subsection{rule-migrator}\par When the perm-tracker finds out new permacode modules have been introduced (for the first time), a migration process needs to take place to process all the existing facts that interact with any new rules defined in these modules, to create all the derived facts and intermediate rule tuples that are the result of this interaction.\par \texttt{rule-migrator} is the service function responsible for this. It depends on zk-plan, which it uses to create the migration plan. We will mock this module with functions that record their own operation, so that we will later be able to view the plan that was created.
\begin{lstlisting}
(def calls (transient []))
 (def last-task (atom 0))
 (def mock-zk-plan
 {:create-plan (fn [parent]
                 (when-not (= permval/*hasher* [:my-hasher])
                   (throw (Exception. "A custom hasher needs to be bound")))
                 (conj! calls [:create-plan parent])
                 :plan-node)
  :add-task (fn [plan func args]
              (conj! calls [:add-task plan func args])
              (swap! last-task inc)
              @last-task)
  :mark-as-ready (fn [node]
                   (conj! calls [:mark-as-ready node]))})
\end{lstlisting}
\par With this mock, \texttt{calls} will contain a list of the calls that were made. \texttt{create-plan} always returns \texttt{:plan-node}, and \texttt{add-task} returns an ordinal number.\par Since \texttt{rule-migrator} is a service, we mock \texttt{declare-service} and \texttt{assign-service} to get the actual function. We also provides it a \texttt{migration-config} resource containing the \texttt{:number-of-shards} parameter, determining how much parallelism we wish to have. The \texttt{hasher} resource is used to retrieve the content of the permacode modules.
\begin{lstlisting}
(def published (atom []))
 (let [calls-chan (async/chan 10)
     decl (transient {})
     assign (transient {})
     \$ (di/injector {:declare-service (fn [key reg]
                                        (assoc! decl key reg))
                     :assign-service (fn [key func]
                                       (assoc! assign key func))
                     :zk-plan mock-zk-plan
                     :migration-config {:number-of-shards 3
                                        :plan-prefix "/my-plans"}
                     :hasher [:my-hasher]})]
 (module \$)
 (di/startup \$)
 ((persistent! decl) "migrator.core/rule-migrator")
 => {:kind :fact
     :name "axiom/perms-exist"}
 (def migrate-rules ((persistent! assign) "migrator.core/rule-migrator")))
\end{lstlisting}
\par Now, if we call the migration function \texttt{migrate-rules} on a rule, it will create a migration plan. First, it will extract the rules out of the given permacode modules by calling extract-version-rules. Then it will sort them according to their dependencies by calling sort-rules. Finally, it will create a migration plan that will cover all rule functions in these modules, to be migrated one by one, in topological order.\par The plan will include, for each rule, a singleton fact-declarer tasks that will start collecting events to be processed by the given rule once the migration is complete; a first phase of initial-migrators to process link 0 of the rule and any number of link-migrator phases to process the rest of the links.
\begin{lstlisting}
(migrate-rules {:kind :fact
               :name "axiom/perms-exist"
               :key "ABCD1234"
               :data [#{'perm.ABC1234 'perm.DEF5678}]
               :writers #{:some-writers}
               :change 1}) => nil
 (provided
(extract-version-rules 'perm.ABC1234) => [timeline]
(extract-version-rules 'perm.DEF5678) => [trending]
(clg/sort-rules [trending timeline]) => [timeline trending])
 (persistent! calls)
 => [[:create-plan "/my-plans"]
   [:add-task :plan-node `(fact-declarer 'migrator.core-test/timeline 0) []] ;; => 1
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/timeline 0 3) [1]] ;; => 2
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/timeline 1 3) [1]] ;; => 3
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/timeline 2 3) [1]] ;; => 4
   [:add-task :plan-node `(fact-declarer 'migrator.core-test/timeline 1) [2 3 4]] ;; => 5
   [:add-task :plan-node `(link-migrator 'migrator.core-test/timeline 1 0 3) [5]] ;; => 6
   [:add-task :plan-node `(link-migrator 'migrator.core-test/timeline 1 1 3) [5]] ;; => 7
   [:add-task :plan-node `(link-migrator 'migrator.core-test/timeline 1 2 3) [5]] ;; => 8
   [:add-task :plan-node `(migration-end-notifier 'migrator.core-test/timeline
                                                  #{:some-writers}) [6 7 8]] ;; => 9
   [:add-task :plan-node `(fact-declarer 'migrator.core-test/trending 0) [9]] ;; => 10
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/trending 0 3) [10]] ;; => 11
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/trending 1 3) [10]] ;; => 12
   [:add-task :plan-node `(initial-migrator 'migrator.core-test/trending 2 3) [10]] ;; => 13
   [:add-task :plan-node `(fact-declarer 'migrator.core-test/trending 1) [11 12 13]] ;; => 14
   [:add-task :plan-node `(link-migrator 'migrator.core-test/trending 1 0 3) [14]] ;; => 15
   [:add-task :plan-node `(link-migrator 'migrator.core-test/trending 1 1 3) [14]] ;; => 16
   [:add-task :plan-node `(link-migrator 'migrator.core-test/trending 1 2 3) [14]] ;; => 17
   [:add-task :plan-node `(migration-end-notifier 'migrator.core-test/trending
                                                  #{:some-writers}) [15 16 17]] ;; => 18
   [:mark-as-ready :plan-node]]
\end{lstlisting}
   
\subsection{clause-migrator}\par Clauses, unlike rules, do not require migration. When a new clause is introduced we need to declare its input queues (for the query and all contributing facts), and then we need to initiate a topology by publishing an \texttt{axiom/rule-ready} event.\par \texttt{clause-migrator} is a microservice that registers to \texttt{axiom/perms-exist} events. It depends on \texttt{publish} (e.g., this for publishing the \texttt{axiom/perms-exist} events, \texttt{hasher}, to retrieve the clause's definition, and on \texttt{declare-service} and \texttt{assign-service} for registering itself. \texttt{declare-service} is also used for declaring the input queues for the clause's topology.
\begin{lstlisting}
(def declared-queues (atom {}))
 (def published (atom []))
 (let [decl (atom {})
     assign (transient {})
     \$ (di/injector
        {:publish (partial swap! published conj)
         :hasher [:hash :unhash]
         :declare-service (fn [key part]
                            (swap! declared-queues assoc key part))
         :assign-service (fn [key func]
                           (assoc! assign key func))})]
 (module \$)
 (di/startup \$)
 (@declared-queues "migrator.core/clause-migrator") => {:kind :fact
                                                        :name "axiom/perms-exist"}
 (def clause-migrator ((persistent! assign) "migrator.core/clause-migrator")))}
\end{lstlisting}
\par In response to an \texttt{axiom/perms-exist} event with a positive \texttt{:change} value, \texttt{clause-migrator} look up all clauses in the new perms.
\begin{lstlisting}
(with-redefs-fn {#'extract-version-clauses
                (fn [perm]
                  (when-not (= permval/*hasher* [:hash :unhash])
                    (throw (Exception. "Hasher not set in call to extract-version-clauses")))
                  (cond (= perm 'perm.ABC1234)
                        [multi-keyword-search]
                        (= perm 'perm.DEF5678)
                        []
                        :else
                        (throw (Exception. "Unexpected perm value"))))}
 #(clause-migrator {:kind :fact
                    :name "axiom/perms-exist"
                    :key "ABCD1234"
                    :data [#{'perm.ABC1234 'perm.DEF5678}]
                    :writers #{:some-writers}
                    :change 1})) => nil
\end{lstlisting}
\par Then it declares a queue associated with the facts that feed each link of each clause:
\begin{lstlisting}
(loop [link multi-keyword-search
      n 0]
 (when link
   (@declared-queues (str "fact-for-rule/migrator.core-test/multi-keyword-search!" n))
   => {:kind :fact
       :name (["test/multi-keyword-search?"
               "migrator.core-test/index-docs"
               "test/doc"] n)}
   (recur (-> link meta :continuation) (inc n))))
\end{lstlisting}
\par Finally, it publishes an \texttt{axiom/rule-ready} event for each clause.
\begin{lstlisting}
@published => [{:kind :fact
               :name "axiom/rule-ready"
               :key 0
               :data ['migrator.core-test/multi-keyword-search]}]
\end{lstlisting}

\subsection{Usage Example}\par In this example we will migrate the rules provided in our tweetlog example.\par First, we need to provide configuration to connect to Zookeeper, RabbitMQ, DynamoDB (local) and S3  (where we provide coordinates using environment variables).
\begin{lstlisting}
(def config
  {:zookeeper-config {:url "127.0.0.1:2181"}
   :zk-plan-config {:num-threads 5
                    :parent "/my-plans"}
   :dynamodb-config {:access-key "FOO"
                     :secret-key "BAR"
                     :endpoint "\url{http://localhost:8006"}}
   :num-database-retriever-threads 1
   :dynamodb-default-throughput {:read 1 :write 1}
   :dynamodb-event-storage-num-threads 3
   :rabbitmq-config {:username "guest"
                 :password "guest"
                 :vhost "/"
                 :host "localhost"
                 :port 5672}
   :migration-config {:number-of-shards 3
                      :plan-prefix "/my-plans"
                      :clone-location "/tmp"
                      :clone-depth 10}
   :s3-config {:bucket-name (System/getenv "PERMACODE_S3_BUCKET")
               :access-key (System/getenv "AWS_ACCESS_KEY")
               :secret-key (System/getenv "AWS_SECRET_KEY")}})
\end{lstlisting}
\par We now create an injector based on the config, and inject dependencies to the migrator and its dependencies.
\begin{lstlisting}
:integ
 (def \$ (di/injector config))
 (module \$)
 (rms/module \$)
 (zkp/module \$)
 (dyn/module \$)
 (s3/module \$)
 (di/startup \$)
\end{lstlisting}
\par Let's create the root elements we need in Zookeeper
\begin{lstlisting}
:integ
 (di/do-with! \$ [zookeeper]
 (when (zk/exists @zookeeper "/perms")
   (zk/delete-all @zookeeper "/perms"))
 (zk/create @zookeeper "/perms" :persistent? true)
 (when (zk/exists @zookeeper "/my-plans")
   (zk/delete-all @zookeeper "/my-plans"))
 (zk/create @zookeeper "/my-plans" :persistent? true))
\end{lstlisting}
\par The next step would be to generate test data. We will start with tweets:
\begin{lstlisting}
:integ
 (def users ["alice" "bob" "charlie"])
 (def time (atom 1000))
 (di/do-with! \$ [publish]
 (doseq [greeting ["hello" "hi" "howdy"]
         greeted ["world" "clojure" "axiom"]
         user users]
   (publish {:kind :fact
             :name "tweetlog/tweeted"
             :key user
             :data [(str greeting " " greeted " from " user)]
             :ts @time
             :change 1
             :writers #{user}
             :readers #{}})
   (swap! time inc)))
\end{lstlisting}
\par Now let's create a full-factorial following matrix (everyone follows everyone else).
\begin{lstlisting}
:integ
 (di/do-with! \$ [publish]
 (doseq [u1 users
         u2 users]
   (when-not (= u1 u2)
     (publish {:kind :fact
               :name "tweetlog/follows"
               :key u1
               :data [u2]
               :ts @time
               :change 1
               :writers #{u1}
               :readers #{}}))
   (swap! time inc))
 :not-nil)
\end{lstlisting}
\par Let's give the microservices a few seconds to store all the facts.
\begin{lstlisting}
:integ
 (Thread/sleep 5000)
\end{lstlisting}
\par To know when our migration is complete we need to listen to \texttt{axiom/rule-ready} events. The following service function listens to such events and for the rule \texttt{followee-tweets} it closes a channel to indicate it is done.
\begin{lstlisting}
:integ
 (def done (async/chan))
 (di/do-with! \$ [serve]
 (serve (fn [ev]
          (when (= (-> ev :data first name) "followee-tweets")
            (async/close! done)))
        {:kind :fact
         :name "axiom/rule-ready"}))
\end{lstlisting}
\par To kick the migration, we need to publish an \texttt{axiom/app-version} event with a version of the example application.
\begin{lstlisting}
:integ
 (di/do-with! \$ [publish]
 (publish {:kind :fact
           :name "axiom/app-version"
           :key "https://github.com/brosenan/tweetlog-clj.git"
           :data ["d3a8c6c5b946279186f857381e751801a657f70c"]
           :ts 1000
           :change 1
           :writers #{}
           :readers #{}}))
\end{lstlisting}
\par So now we wait for the migration to complete.
\begin{lstlisting}
:integ
 (async/<!! done)
\end{lstlisting}
\par After the migration, all facts have been processed by the rules. This means that Alice's timeline should contain 18 tweets.
\begin{lstlisting}
:integ
 (di/do-with! \$ [database-chan]
 (let [chan-out (async/chan 30)]
   (async/>!! database-chan [{:kind :fact
                              :name "perm.QmdLhmeiaJTMPdv7oT7mUsztdtjHq7f16Dw6nkR6JhxswP/followee-tweets"
                              :key "alice"} chan-out])
   (loop [res 0]
     (let [ev (async/<!! chan-out)]
       (cond (nil? ev)
             res
             :else
             (recur (inc res))))))) => 18
\end{lstlisting}
\par Finally, we shut down the injector to stop the workers.
\begin{lstlisting}
:integ
 (di/shutdown \$)
\end{lstlisting}
 
\subsection{Under the Hood}
\subsubsection{zookeeper-counter-add}\par \texttt{zookeeper-counter-add} depends on the \texttt{zookeeper} resource as dependency, and uses it to implement a global atomic counter.
\begin{lstlisting}
(let [\$ (di/injector {:zookeeper (atom :zk)})]
  (module \$)
  (di/startup \$)
  (def zookeeper-counter-add (di/do-with! \$ [zookeeper-counter-add] zookeeper-counter-add)))
\end{lstlisting}
\par \texttt{zookeeper-counter-add} takes a path to a counter and a number to be added. If a node corresponding to the given path does not exist, it is assumed to be equal 0, and is therefore created using the given number. The new value, which is the given number, is returned.
\begin{lstlisting}
(zookeeper-counter-add "/rules/foobar" 3) => 3
 (provided
(zk/exists :zk "/rules/foobar") => nil
(zk/create-all :zk "/rules/foobar" :persistent? true) => "/rules/foobar"
(zkp/set-initial-clj-data :zk "/rules/foobar" 3) => irrelevant)
\end{lstlisting}
\par If a node exists, its value is updated to add the given number.
\begin{lstlisting}
(zookeeper-counter-add "/rules/foobar" 3) => 5
 (provided
(zk/exists :zk "/rules/foobar") => {:some :values
                                    :version 7}
(zkp/get-clj-data :zk "/rules/foobar") => 2
(zkp/to-bytes "5") => ..bin..
(zk/set-data :zk "/rules/foobar" ..bin.. 7) => irrelevant)
\end{lstlisting}
\par \texttt{zookeeper-counter-add} takes an extra \texttt{retries} parameter which defaults to 3. If \texttt{zk/set-data} throws an exception for any reason, the update is retried. This is to account for the possibility of concurrent update.
\begin{lstlisting}
(zookeeper-counter-add "/rules/foobar" 3) => 6
 (provided
(zk/exists :zk "/rules/foobar") =streams=> [{:some :values
                                             :version 7}
                                            {:some :values
                                             :version 8}]
(zkp/get-clj-data :zk "/rules/foobar") =streams=> [2 3]
(zkp/to-bytes "5") => ..bin1..
(zk/set-data :zk "/rules/foobar" ..bin1.. 7) =throws=> (Exception. "boo")
(zkp/to-bytes "6") => ..bin2..
(zk/set-data :zk "/rules/foobar" ..bin2.. 8) => irrelevant)
\end{lstlisting}
\par When the retries are exhasted, the function throws.
\begin{lstlisting}
(zookeeper-counter-add "/rules/foobar" 3) => (throws "boo")
 (provided
(zk/exists :zk "/rules/foobar") =streams=> [{:some :values
                                             :version 7}
                                            {:some :values
                                             :version 8}
                                            {:some :values
                                             :version 9}]
(zkp/get-clj-data :zk "/rules/foobar") =streams=> [2 3 4]
(zkp/to-bytes irrelevant) => irrelevant
(zk/set-data :zk "/rules/foobar" irrelevant irrelevant) =throws=> (Exception. "boo"))
\end{lstlisting}

\subsubsection{fact-declarer}\par \texttt{fact-declarer} is used to declare the service that will accept events related to a certain fact. We call it before we start migration based on that fact so that new events related to this fact that come during the migration process are accumulated in the queue. Once the migration is done, functions assigned to it will receive these events as well as new ones, so there will not be any data loss.\par \texttt{fact-declarer} is a generator function that takes the name of the rule and the link number (as a unique identifier)
\begin{lstlisting}
(def decl-my-fact (fact-declarer 'perm.ABC123/my-rule 1))
\end{lstlisting}
\par The returned fact declarer is intended to be used in a zk-plan, as a task function. As such, it needs to accept one or more arguments. It ignores all but the first one, which is an injector (\texttt{\$}) passed to it directly by \texttt{zk-plan}.\par The injector must be able to resolve the resources \texttt{declare-service} (e.g., the one implemented for RabbitMQ), and \texttt{hasher} (e.g., the one implemented for S3). We will mock them here.
\begin{lstlisting}
(let [calls (async/chan 10)
     \$ (di/injector {:hasher [:my-hasher]
                     :declare-service (fn [key reg]
                                        (when-not (= permval/*hasher* [:my-hasher])
                                          (throw (Exception.
                                                  "A custom hasher needs to be bound")))
                                        (async/>!! calls [:declare-service key reg]))})]
 (decl-my-fact \$ :some :args :that :are :ignored) => nil
 (provided
  (perm/eval-symbol 'perm.ABC123/my-rule) => timeline)
 ;; Assert the calls
 (async/alts!! [calls
                (async/timeout 1000)])
 => [[:declare-service "fact-for-rule/perm.ABC123/my-rule!1" {:kind :fact
                                                              :name "test/tweeted"}] calls])
\end{lstlisting}
							      
\subsubsection{initial-migrator}\par \texttt{initial-migrator} creates a migration function for link 0 of a rule. Link 0 is special in that it only depends on a fact, creates rule tuples based on fact tuples. Other links also depend on previous rule tuples.\par \texttt{initial-migrator} takes the following arguments:\begin{enumerate}\item \texttt{rule}: The name of a rule (as a symbol).\item \texttt{shard}: The shard number\item \texttt{shards}: The total number of shards being used.It returns a closure (function) that operates from within a zk-plan.\end{enumerate}
\begin{lstlisting}
(def my-migrator (initial-migrator 'perm.ABC/my-rule 2 6))
\end{lstlisting}
\par The migration process requires a \texttt{database-scanner} (e.g., this) to scan given shard of the given table (fact). We mock this function by providing \texttt{:test/follows} facts for Alice, who follows Bob, Charlie and Dave. 
\begin{lstlisting}
(defn mock-scanner [name shard shards chan]
  (when-not (= [name shard shards] ["test/follows" 2 6])
    (throw (Exception. (str "Unexpected args in mock-scanner: " [name shard shards]))))
  (when-not (= permval/*hasher* [:my-hasher])
    (throw (Exception. "A custom hasher needs to be bound")))
  (doseq [followee ["bob" "charlie" "dave"]]
    (async/>!! chan {:kind :fact
                     :name name
                     :key "alice"
                     :data [followee]
                     :change 1
                     :ts 1}))
  (async/close! chan))
\end{lstlisting}
\par To store the resulting tuples it depends on a \texttt{database-event-storage-chan} (e.g., this), a channel to which all generated events need to be sent.
\begin{lstlisting}
(def rule-tuple-chan (async/chan 10))
\end{lstlisting}
\par As a \texttt{zk-plan} task function, the first argument of the returned closure (\texttt{my-migrator} in our case), is expected to be an injector (\texttt{\$}), and all other arguments should be ignored. Once called, it will use permacode.core/eval-symbol to get the rule function. Evaluation leverages the \texttt{hasher} resource. It will evaluate this function on each result comming from the \texttt{database-scanner}.
\begin{lstlisting}
(let [\$ (di/injector {:hasher [:my-hasher]
                     :database-scanner mock-scanner
                     :database-event-storage-chan rule-tuple-chan})]
 (my-migrator \$ :ignored) => nil
 (provided
  (perm/eval-symbol 'perm.ABC/my-rule) => timeline))
\end{lstlisting}
\par The migrator function should push to \texttt{database-event-storage-chan} rule events. In our case, these should be one per each fact.
\begin{lstlisting}
(defn read-event []
 (let [resp (async/alts!! [rule-tuple-chan
                           (async/timeout 1000)])]
   (when-not (= (second resp) rule-tuple-chan)
     (throw (Exception. "Opration timed out")))
   (async/close! (second (first resp))) ;; ack
   (first (first resp))))
 
 (read-event) => {:change 1
                :data ["alice" "bob"]
                :key "bob"
                :kind :rule
                :name "migrator.core-test/timeline!0"
                :readers nil
                :writers #{"migrator.core-test"}
                :ts 1}
 (read-event) => {:change 1
                :data ["alice" "charlie"]
                :key "charlie"
                :kind :rule
                :name "migrator.core-test/timeline!0"
                :readers nil
                :writers #{"migrator.core-test"}
                :ts 1}
 (read-event) => {:change 1
                :data ["alice" "dave"]
                :key "dave"
                :kind :rule
                :name "migrator.core-test/timeline!0"
                :readers nil
                :writers #{"migrator.core-test"}
                :ts 1}
\end{lstlisting}
		
\subsubsection{link-migrator}\par For links other than 0, migration requires applying a matcher. A matcher takes one event (a fact event in our case), and matches it against all matching events (rule events in our case). We need to provide a \texttt{database-chan} to allow the matcher to cross reference facts and rules.\par The \texttt{link-migrator} function takes the following arguments:\begin{enumerate}\item \texttt{rule}: The rule to be migrated.\item \texttt{link}: The link number within the rule (> 0).\item \texttt{shard}: The shard number to be processed by this node.\item \texttt{shards}: The overall number of shards.It returns a closure to be processed as a \texttt{zk-plan} task.\end{enumerate}
\begin{lstlisting}
(def my-link-migrator (link-migrator 'perm.ABC/my-rule 1 3 17))
\end{lstlisting}
\par For the migration process we will need a \texttt{database-scanner} that will provide fact events. We will mock one to produce \texttt{:test/tweeted} facts, stating that Bob, Charlie and Dave all tweeted 'hello'.
\begin{lstlisting}
(defn mock-scanner [name shard shards chan]
  (when-not (= [name shard shards] ["test/tweeted" 3 17])
    (throw (Exception. (str "Unexpected args in mock-scanner: " [name shard shards]))))
  (when-not (= permval/*hasher* [:my-hasher])
    (throw (Exception. "A custom hasher needs to be bound")))
  (doseq [user ["bob" "charlie" "dave"]]
    (async/>!! chan {:kind :fact
                     :name name
                     :key user
                     :data ["hello"]
                     :change 1
                     :ts 1}))
  (async/close! chan))
\end{lstlisting}
\par We also need to provide a \texttt{database-chan} (e.g., this), which in our case, will answer that regardless of who was making the tweet, both Alice and Eve are followers. These events are similar to the ones we got from the initial-migrator.
\begin{lstlisting}
(def mock-db-chan (async/chan 10))
 (async/go
 (loop []
   (let [[query out-chan] (async/<! mock-db-chan)]
     (when-not (nil? query)
       ;; The query is for rule tuples of link 0
       (when-not (= (:name query) "migrator.core-test/timeline!0")
         (throw (Exception. (str "Wrong fact in query: " (:name query)))))
       (async/>!! out-chan {:change 1
                            :data ["alice" (:key query)]
                            :key (:key query)
                            :kind :rule
                            :name "migrator.core-test/timeline!0"
                            :readers nil
                            :writers #{:some-writer}
                            :ts 1})
       (async/>!! out-chan {:change 1
                            :data ["eve" (:key query)]
                            :key (:key query)
                            :kind :rule
                            :name "migrator.core-test/timeline!0"
                            :readers nil
                            :writers #{:some-writer}
                            :ts 1})
       (async/close! out-chan)
       (recur)))))
\end{lstlisting}
\par Once more, we will need a \texttt{database-event-storage-chan} (e.g., this) to store the events we get.
\begin{lstlisting}
(def mock-store-chan (async/chan 10))
\end{lstlisting}
\par The closure we got from \texttt{link-migrator} (\texttt{my-link-migrator} in our case) takes an injector as a first argument, and ignores all others. It calls permacode.core/eval-symbol to get the rule and then creates a matcher based on it.
\begin{lstlisting}
(let [\$ (di/injector {:database-scanner mock-scanner
                     :database-chan mock-db-chan
                     :database-event-storage-chan mock-store-chan
                     :hasher [:my-hasher]})]
 (my-link-migrator \$ :ignored) => nil
 (provided
  (perm/eval-symbol 'perm.ABC/my-rule) => timeline))
\end{lstlisting}
\par The migration function reads all fact events from the scanner,  for each event it consults the \texttt{database-chan} for matching rule tuples, and the resulting events (timeline facts in our case) are pushed to the \texttt{database-event-storage-chan}.
\begin{lstlisting}
(defn read-event []
 (let [resp (async/alts!! [mock-store-chan
                           (async/timeout 1000)])]
   (when-not (= (second resp) mock-store-chan)
     (throw (Exception. "Operation timed out")))
   (async/close! (second (first resp))) ;; ack
   (first (first resp))))
 ;; For Bob
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "eve"
                :data ["bob" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "alice"
                :data ["bob" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "eve"
                :data ["charlie" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "alice"
                :data ["charlie" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "eve"
                :data ["dave" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
 (read-event) => {:kind :fact
                :name "migrator.core-test/timeline"
                :key "alice"
                :data ["dave" "hello"]
                :change 1
                :readers nil
                :writers #{:some-writer}
                :ts 1}
\end{lstlisting}
\par For good citizenship, let's close the mock \texttt{database-chan} and allow the service we started shut down.
\begin{lstlisting}
(async/close! mock-db-chan)}
\end{lstlisting}
		
\subsubsection{migration-end-notifier}\par rule-migrator finishes when a plan is created and is ready to be executed. However, the actual migration operation only starts at that point. We therefore need a way to tell other parts of \emph{axiom} that the rule has been migrated, once migration is complete. For this purpose, the plan will include a final piece: \texttt{migration-end-notifier}, which will publish a \texttt{axiom/rule-ready} event holding the rule identifier as its \texttt{:key}.
\begin{lstlisting}
(def my-end-notifier (migration-end-notifier 'perm.ABC123/my-rule #{:some-writer}))
\end{lstlisting}
\par The returned closure (\texttt{my-end-notifier}) takes an injector and any number of other parameters. From the injector it takes the \texttt{publish} resource to publish the desired event.
\begin{lstlisting}
(def events (transient []))
 (let [\$ (di/injector {:publish (fn [ev] (conj! events ev))})]
 (my-end-notifier \$ :some :other :params))
\end{lstlisting}
\par Once called it should \texttt{publish} an \texttt{axiom/rule-ready} event (we ignore the \texttt{:ts} field which changes with time).
\begin{lstlisting}
(-> events
   persistent!
   first
   (dissoc :ts)) => {:kind :fact
                     :name "axiom/rule-ready"
                     :key 0
                     :data ['perm.ABC123/my-rule]
                     :change 1
                     :writers #{:some-writer}}
\end{lstlisting}
		     
\subsubsection{extract-version-rules}\par \texttt{extract-version-rules} extracts all the rule functions from such a version and publishes corresponding \texttt{:axiom/rule} events.\par It returns only rule functions, identified by having a \texttt{:source-fact} meta field.
\begin{lstlisting}
(let [foo (with-meta (fn []) {:source-fact ["foo" 1]})
     bar (with-meta (fn []) {:source-fact ["bar" 1]})
     baz (fn [])]
 (extract-version-rules 'perm.1234ABC) => [foo
                                           bar]
 (provided
  (perm/module-publics 'perm.1234ABC) => {'foo foo
                                          'bar bar
                                          'baz baz} ; baz will not be returned
  ))
\end{lstlisting}
\par It excludes clauses, for which the \texttt{:source-fact} ends with a question mark (\texttt{?}).
\begin{lstlisting}
(let [foo (with-meta (fn []) {:source-fact ["foo" 1]})
     bar (with-meta (fn []) {:source-fact ["bar?" 1]})]
 (extract-version-rules 'perm.1234ABC) => [foo]
 (provided
  (perm/module-publics 'perm.1234ABC) => {'foo foo
                                          'bar bar} ; bar will not be returned
  ))
\end{lstlisting}
  
\subsubsection{extract-version-clauses}\par Like extract-version-rules, \texttt{extract-version-rules} takes a symbol representing a permacode namespace, and returns a collection of clauses defined in that namespace.
\begin{lstlisting}
(let [foo (with-meta (fn []) {:source-fact ["foo" 1]}) ;; not a clause
     bar (with-meta (fn []) {:source-fact ["bar?" 1]})
     baz (fn [])] ;; not a clause
 (extract-version-clauses 'perm.1234ABC) => [bar]
 (provided
  (perm/module-publics 'perm.1234ABC) => {'foo foo
                                          'bar bar
                                          'baz baz}))
\end{lstlisting}
					  
\subsubsection{hash-static-file}\par When a new version is pushed we wish to scan everything under its \texttt{/resources/public} directory (if exists), and store all these files in a way that will allow the gateway tier to retrieve them.\par We use the \texttt{hasher} resource (e.g., the one provided for S3) to store the content of files. This way, if a file is not modifed, we store only one copy of it.\par The resource \texttt{hash-static-file} depends on a \texttt{hasher}. It is a function that takes a path to a file in the local file system, reads its content and hashes it.\par To demonstrate how it works we create a temporary file:
\begin{lstlisting}
(with-open [f (clojure.java.io/writer "/tmp/foo.txt")]
 (doseq [i (range 1000)]
   (.write f (str "This is line number " i "$\backslash$n"))))
\end{lstlisting}
\par Now, when we call \texttt{hash-static-file} it will use the \texttt{hash} part of the \texttt{hasher} to store the content of the file, given as a binary array.
\begin{lstlisting}
(let [content (atom nil)
     hash (fn [c]
            (reset! content c)
            "some-hash")
     unhash (fn [h]
              (throw (Exception. "unhash should not be called")))
     \$ (di/injector {:hasher [hash unhash]})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [hash-static-file]
              (hash-static-file (io/file "/tmp/foo.txt")) => "some-hash")
 (class @content) => (class (byte-array 1))
 (-> @content
     String.
     (str/split #"$\backslash$n")
     (get 745)) => "This is line number 745")
\end{lstlisting}
     
\subsubsection{hash-static-files}\par To recursively store all files under a given directory (the \texttt{/resources/public} directory in the repo), the function \texttt{hash-static-files} applies \texttt{hash-static-file} to each file in the subtree under the given root. It returns a map from relative paths to hash values.\par To demonstrate this we will create a directory under \texttt{/tmp} and populate it with three file -- \texttt{a.html}, \texttt{b.css} and \texttt{c.js}.
\begin{lstlisting}
(let [dir (io/file "/tmp/mock-static")]
 (.mkdirs dir)
 (with-open [a (io/writer (io/file dir "a.html"))]
   (.write a "Some html..."))
 (with-open [b (io/writer (io/file dir "b.css"))]
   (.write b "Some CSS..."))
 (with-open [c (io/writer (io/file dir "c.js"))]
   (.write c "Some JavaScript...")))
\end{lstlisting}
\par Calling \texttt{hash-static-files} on \texttt{/tmp/mock-static} will return a map containing entries for \texttt{/a.html}, \texttt{/b.css} and \texttt{c.js}.
\begin{lstlisting}
(let [\$ (di/injector {:hash-static-file
                     (fn [f]
                       (str "hash-for-" (.getPath f)))})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [hash-static-files]
              (hash-static-files (io/file "/tmp/mock-static"))
              => {"/a.html" "hash-for-/tmp/mock-static/a.html"
                  "/b.css" "hash-for-/tmp/mock-static/b.css"
                  "/c.js" "hash-for-/tmp/mock-static/c.js"}))
\end{lstlisting}
		  
		  
\subsubsection{deploy-dir}\par \texttt{deploy-dir} is a function that takes a base directory and publishes an \texttt{axiom/perm-versions} event containing  all permacode source files and all static content in this directory. It is a DI resource based on a \texttt{hasher}, hash-static-files and \texttt{publish}.
\begin{lstlisting}
(def staticdir (atom nil))
 (let [\$ (di/injector {:hasher [:my-hasher]
                     :hash-static-files (fn [root]
                                          (reset! staticdir root)
                                          {"/a.html" "hash1"
                                           "/b.css" "hash2"
                                           "/c.js" "hash3"})})]
 (module \$)
 (di/startup \$)
 (di/do-with! \$ [deploy-dir]
              (def deploy-dir deploy-dir)))
\end{lstlisting}
\par This function takes version identifier, a root directory and a \texttt{publish} function, and does the following:\begin{itemize}\item Calls \texttt{permacode.publish/hash-all} on its \texttt{src} sub-directory with the \texttt{hasher} bound as the \texttt{*hasher*}, to get a source-code map.\item Calls \texttt{hash-static-files} on the \texttt{/resources/public} sub-directory to get a map for the static files.\end{itemize}
\begin{lstlisting}
(def published (atom []))
 (deploy-dir "some-ver" "/path/to/deploy" (partial swap! published conj)) => nil
 (provided
(permacode.publish/hash-all [:my-hasher] (io/file "/path/to/deploy" "src")) => {'foo 'perm.AAA
                                                                   'bar 'perm.BBB}
(io/file "/path/to/deploy" "resources/public") => ..static..)
 @staticdir => ..static..
\end{lstlisting}
\par Then it uses the given \texttt{publish} function to publish an \texttt{axiom/perm-versions} event containing both maps.
\begin{lstlisting}
@published => [{:kind :fact
               :name "axiom/perm-versions"
               :key "some-ver"
               :data [{'foo 'perm.AAA
                       'bar 'perm.BBB}
                      {"/a.html" "hash1"
                       "/b.css" "hash2"
                       "/c.js" "hash3"}]}]
\end{lstlisting}
        
      
    

    


==> axiom/permacode.tex <==
\section{Permacde}\footnote{\SANITIZEDURL{http://axiom-clj.org/permacode.html}}

\subsection{Introduction}\par Just like the term \emph{permalink} refers to a URL that will always link to the same content, \emph{permacode} refers to code that will always behave the same way.\par There are a few challenges in acheiving this in general code:\begin{itemize}\item State changes.  Imperative code can store state which affects its own execution.\item The world changes.  Code that queries the state of the world (e.g., \texttt{(System/currentTimeMillis)}) will give different results when the state of the world changes.\item Code changes.  One version of the code will not behave the same way as its predecessors.\end{itemize}\par Making permacode possible in the context of Clojure is a two-step process. First, we need to extract the \emph{purely-functional core} of Clojure, to avoid the first to issues. Purely-functional code is not affected by the outer world and does not affect it, guaranteeing that the same code will always run the same way. To address the second problem we add \emph{content addressing} to replace Clojure's module system.
			  
\subsubsection{A Purely-Functional Clojure}\par permacode attempts to create a purely-functional dialect of Clojure. This is a stripped-down Clojure, with only the purely-functional parts, including:\begin{itemize}\item Functions (well duh...)\item \texttt{let}, \texttt{loop}, \texttt{if} etc.\item maps, sets, vectors and lists\item A subset of the \texttt{clojure.core} library functions and macros, as well as\item \texttt{clojure.string}, \texttt{clojure.set} and potentially other pure libraries.\end{itemize}\par It does not include:\begin{itemize}\item Variables\item Atoms, refs, agents, etc.\item Java interop\item Imperative functions from \texttt{clojure.core}\item Arbitrary (non-permacode) libraries\end{itemize}
		
\subsubsection{Content Addressing}\par The term \emph{content addressing} means that some objects (in our case, permacode modules) are \emph{addressed} by their \emph{content}, as opposed to addressing them by \emph{name}, which is the way Clojure works by default.\par In Clojure, a \texttt{:require} clause states a name of a module, relative to the classpath of the containing project.  This has two problems as far as permacode is concerned. First, it relies on the concept of a \emph{project}, so in two different projects there could be a different module with the same name. Second, while a name is stated explicitly, the \emph{version} is not. It is stated in the project description, but that could just as well be a \texttt{SNAPSHOT} version, which is not a version at all.\par In Permacode, we would like code artifacts to be explicitly stated. Content addressing allows us to do that, because instead of referring to modules by their names, we refer to them by their \emph{content}.\par Someone reading these lines could think, what is the point of having modules in the first place, if we refer to them by their content, that  is, including them instead if \texttt{:require}ing them? Well, the answer is that we do not \emph{include} one module in another, we just use a \emph{cryptographic hash} over its content as its name. This is similar to how git represents objects like directories and commits. A directory in git is merely a list of hash codes for versions of underlying files and sub-dirs. A commit contains the hash code of the root directory at the time of the commit. This data structure is called a Merkle Tree.\par To support this, we use an abstraction of a \emph{hasher}, some data-store that can either \emph{hash} an s-expression (serialize, hash and store its content, returning the hash code), and \emph{unhash} a hash-code (retrieve from the data-store, de-serialize and return the s-expression).\par With such a hasher in place we can:\begin{enumerate}\item Given a set of Clojure files (typically the source tree of a Clojure project),\begin{itemize}\item Validate that all *.clj files conform with permacode, and if so --\item Hash all these files, modifying them to reference each other by hash rather than by name.\item Return a map from module name to module hash.\end{itemize}\item Given a module hash, load the module.\item Given a fully-qualified symbol (where the namespace is a permacode hash), return the value of that symbol.  This value is guaranteed to always be the same, regardless of where and when it is evaluated.\end{enumerate}
			
\subsection{pure: Compile-time Verification}\par A permacode module should be wrapped in a \texttt{permacode.core/pure} macro. This macro validates the underlying code under the module's own namespace. Validation involves macro expansion, and macros are expanded based on how they are defined relative to that module.\par A valid set of definitions evaluates to a \texttt{do} block with the same content.
\begin{lstlisting}
(pure
(defn foo [x y]
  (+ x y))
(defn bar [x y]
  (* x y)))
 =expands-to=> (do
               (defn foo [x y]
                 (+ x y))
               (defn bar [x y]
                 (* x y)))
\end{lstlisting}
\par For definitions that use disallowed symbols \texttt{pure} throws an exception during macro expansion.
\begin{lstlisting}
(macroexpand '(pure
              (def some-atom (atom 0))))
 => (throws "symbols #{atom} are not allowed")
\end{lstlisting}
\par Allowed symbols should be available unqualified or fully-qualified.
\begin{lstlisting}
	(pure
(def x (+ 1 2))
(def y (clojure.core/+ 2 3)))
 =expands-to=> (do
               (def x (+ 1 2))
               (def y (clojure.core/+ 2 3)))
\end{lstlisting}
\par Some namespaces, such as \texttt{clojure.string} and \texttt{clojure.set} are white-listed, and all their publics are allowed.
\begin{lstlisting}
(pure
(def x (clojure.string/join ", " (clojure.set/union #{1 2} #{3}))))
\end{lstlisting}
\par When namespaces are aliased (like \texttt{clojure.string} is aliased to \texttt{string} in this file), symbols referring to the alias are also allowed.
\begin{lstlisting}
(pure
(def x (string/join ", " (set/union #{1 2} #{3}))))
\end{lstlisting}

\subsubsection{Stress Testing}\par The following is a usage example coming from cloudlog. It is supposed to be all pure, so it's a good test case...
\begin{lstlisting}
(permacode.core/pure
 (declare generate-rule-func)

 (defmulti propagate-symbols (fn [cond symbols] (first cond)) :default :no-bindings)
 (defmethod propagate-symbols :no-bindings [cond symbols]
   symbols)

 (defn binding-symbols [bindings cond]
   (symbols/symbols (map bindings (range 0 (count bindings) 2))))

 (defmethod propagate-symbols 'let [cond symbols]
   (set/union symbols (binding-symbols (second cond) cond)))

 (defmethod propagate-symbols 'for [cond symbols]
   (set/union symbols (binding-symbols (second cond) cond)))

 (defmulti process-conds (fn [conds symbols] (class (first conds))))

                                        ; fact
 (defmethod process-conds  clojure.lang.IPersistentVector [conds symbols]
   (let [target (first conds)
         target-name (first target)]
     (if (= (count conds) 1)
       (do ; Target fact
         [[(vec (rest target))] {:target-fact [target-name (count (rest target))]}])
                                        ; Continuation
       (let [[func meta] (generate-rule-func (first conds) (rest conds) symbols)
             key (second target)
             params (vec (set/intersection symbols (symbols/symbols func)))
             missing (set/difference (symbols/symbols key) symbols)
             meta {:continuation (with-meta `(fn [[key# ~@params]] ~func) meta)}]
         (when-not (empty? missing)
           (permacode.core/error "variables " missing " are unbound in the key for " (first target)))
         [`[[~key ~@params]] meta]))))

                                        ; guard
 (defmethod process-conds  clojure.lang.ISeq [conds symbols]
   (let [cond (first conds)
         [body meta] (process-conds (rest conds) (propagate-symbols cond symbols))
         body (seq (concat cond [body]))
         meta (if (string/starts-with? (str (first cond)) "by")
                (assoc meta :checked true)
                meta)]
     (if (= (first cond) 'for)
       [`(apply concat ~body) meta]
                                        ; else
       [body meta])))

 (defn generate-rule-func [source-fact conds ext-symbols]
   (let [symbols (set/difference (symbols/symbols (rest source-fact)) ext-symbols)
         [body meta] (process-conds conds (set/union symbols ext-symbols))
         meta (merge meta {:source-fact [(first source-fact) (count (rest source-fact))]})
         vars (vec symbols)
         func `(fn [input#]
                 ~(if (empty? vars)
                                        ; No unbound variables
                    `(if (= input# [~@(rest source-fact)])
                       ~body
                       [])
                                        ; vars contains the unbound variables
                    `(let [poss# ((unify/unify-fn ~vars [~@(rest source-fact)] ~vars) input#)]
                       (apply concat (for [~vars poss#] 
                                       ~body)))))]
     [func meta]))

 (defn validate-rule [metadata]
   (loop [metadata metadata
          link 0]
     (when-not (:checked metadata)
       (permacode.core/error "Rule is insecure. Link " link " is not checked."))
     (when (:continuation metadata)
       (recur (-> metadata :continuation meta) (inc link)))))

 (defmacro defrule [rulename args source-fact & body]
   (let [conds (concat body [`[~(keyword (str *ns*) (name rulename)) ~@args]])
         [func meta] (generate-rule-func source-fact conds #{})]
     (validate-rule meta)
     `(def ~rulename (with-meta ~func ~(merge meta {:ns *ns* :name (str rulename)})))))

 (defn append-to-keyword [keywd suffix]
   (keyword (namespace keywd) (str (name keywd) suffix)))

 (defmacro defclause [clausename pred args-in args-out & body]
   (let [source-fact `[~(append-to-keyword pred "?") unique# ~@args-in]
         conds (concat body [`[~(append-to-keyword pred "!") unique# ~@args-out]])
         [func meta] (generate-rule-func source-fact conds #{})]
     `(def ~clausename (with-meta ~func ~(merge meta {:ns *ns* :name (str clausename)})))))

 (defn with* [seq]
   (apply merge-with set/union
          (for [fact seq]
            (let [fact-name (first fact)
                  metadata (meta fact)
                  arity (-> fact rest count)]
              {[fact-name arity] #{(with-meta (vec (rest fact)) metadata)}}))))

 (defn simulate* [rule factmap]
   (let [source-fact (-> rule meta :source-fact)
         input-set (factmap source-fact)
         after-first (into #{} (apply concat (map rule input-set)))
         cont (-> rule meta :continuation)]
     (if cont
       (let [next-rules (map cont after-first)]
         (into #{} (apply concat (for [next-rule next-rules]
                                   (simulate* (with-meta next-rule (meta cont)) factmap)))))
                                        ;else
       after-first)))

 (defn simulate-with [rule & facts]
   (simulate* rule (with* facts)))

 (defmulti fact-table (fn [[name arity]] (class name)))

 (defmethod fact-table clojure.lang.Named [[name arity]]
   (str (namespace name) "/" (clojure.core/name name)))
 (defmethod fact-table clojure.lang.IFn [[name arity]]
   (let [ns (-> name meta :ns)
         name (-> name meta :name)]
     (str ns "/" name)))
 (prefer-method fact-table clojure.lang.Named clojure.lang.IFn)

 (defmacro by [set body]
   `(when (contains? (-> input# meta :writers) ~set)
      ~body))

 (defmacro by-anyone [body]
   body))
\end{lstlisting}
   
\subsection{error: A Replacement for throw}\par We do not allow pure code to \texttt{throw}, because throwing exceptions involves creating Java classes. Instead, we provide the \texttt{error} function, which throws an \texttt{Exception} with the given string.
\begin{lstlisting}
(error 1000 " bottles of beer on the wall") => (throws #"1000 bottles of beer")}
\end{lstlisting}

\subsection{eval-symbol: Evaluate a Permacode Definition}\par At the end, all we want is to be able to take a certain definition and evaluate it. For example, consider the following Permacode module:
\begin{lstlisting}
(def my-module
  '[(ns example.my-module
      (:require [clojure.string :as str]
                [permacode.core]))
    (permacode.core/pure
     (defn tokenize [text]
       (str/split text #"[ ,.!?:]+")))])

(def my-other-module
  '[(ns example.my-other-module
      (:require [perm.QmXGe3DdhRGKfLgs1Dp9sNa2VFktfqj32XicKRcUeLXMxG :as mine]
                [permacode.core]))
    (permacode.core/pure
     (defn extract-hashtags [text]
       (->> text mine/tokenize (filter (fn [x] (clojure.string/starts-with? x "#")))))
     (def foo (with-meta [2] {:some :meta})))])
\end{lstlisting}
\par Let's save these to files.
\begin{lstlisting}
(def example-dir (io/file "/tmp/permacode.core/example"))
(.mkdirs example-dir)
(with-open [f (io/writer (io/file example-dir "my_module.clj"))]
  (doseq [expr my-module]
    (.write f (pr-str expr))))
(with-open [f (io/writer (io/file example-dir "my_other_module.clj"))]
  (doseq [expr my-other-module]
    (.write f (pr-str expr))))
\end{lstlisting}
\par Now let's publish the \texttt{example} directory.
\begin{lstlisting}
(remove-ns 'perm.QmXGe3DdhRGKfLgs1Dp9sNa2VFktfqj32XicKRcUeLXMxG)
 (remove-ns 'perm.QmVxcd8ooha7JtZvh5AD3QhAiLMm7Zjm5YAqkXitVbVSfo)
 (def hasher (hasher/nippy-multi-hasher (hasher/atom-store)))
(def published
  (publish/hash-all hasher example-dir))
published => map?
published =not=> empty?}
\end{lstlisting}
\par Now we want to use the \texttt{extrat-hashtags} function.  To do so we use \texttt{eval-symbol}:
\begin{lstlisting}
(published 'example.my-module) => 'perm.QmXGe3DdhRGKfLgs1Dp9sNa2VFktfqj32XicKRcUeLXMxG
 (published 'example.my-other-module) => 'perm.QmVxcd8ooha7JtZvh5AD3QhAiLMm7Zjm5YAqkXitVbVSfo
 (binding [validate/*hasher* hasher]
 (let [extract-hashtags (eval-symbol 'perm.QmVxcd8ooha7JtZvh5AD3QhAiLMm7Zjm5YAqkXitVbVSfo/extract-hashtags)]
   (extract-hashtags "These #days #tweets are all about #hashtags...") => ["#days" "#tweets" "#hashtags"]))}
\end{lstlisting}
\par Metadata is maintained (the actual value is returned, not a variable pointing to it).
\begin{lstlisting}
	(binding [validate/*hasher* hasher]
 (let [foo (eval-symbol 'perm.QmVxcd8ooha7JtZvh5AD3QhAiLMm7Zjm5YAqkXitVbVSfo/foo)]
   (-> foo meta :some) => :meta))}
\end{lstlisting}
   
\subsection{module-publics: Get All Symbols}\par \texttt{module-publics} (similar to \texttt{ns-publics} in \texttt{clojure.core}) returns all the public definitions in a permacode module in form of a map.
\begin{lstlisting}
(binding [validate/*hasher* hasher]
 (let [pubs (module-publics 'perm.QmVxcd8ooha7JtZvh5AD3QhAiLMm7Zjm5YAqkXitVbVSfo)]
   pubs => map?
   (pubs 'foo) => [2]))}
\end{lstlisting}


==> figs/challenges.tex <==
% Graphic for TeX using PGF
% Title: C:\Users\lorenz\Documents\NucGit\LOP-Private\ecoop18\figs\challenges.dia
% Creator: Dia v0.97.2
% CreationDate: Sun Jan 07 15:21:21 2018
% For: lorenz
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (27.175000\du,5.100000\du)--(27.175000\du,7.000000\du)--(30.535000\du,7.000000\du)--(30.535000\du,5.100000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.175000\du,5.100000\du)--(27.175000\du,7.000000\du)--(30.535000\du,7.000000\du)--(30.535000\du,5.100000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (28.855000\du,6.290000\du){Security};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (25.766300\du,8.250000\du)--(25.766300\du,11.750000\du)--(29.333800\du,11.750000\du)--(29.333800\du,8.250000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (25.766300\du,8.250000\du)--(25.766300\du,11.750000\du)--(29.333800\du,11.750000\du)--(29.333800\du,8.250000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (27.550050\du,9.840000\du){Access};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (27.550050\du,10.640000\du){Control};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (29.885000\du,8.350000\du)--(29.885000\du,10.350000\du)--(34.915000\du,10.350000\du)--(34.915000\du,8.350000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (29.885000\du,8.350000\du)--(29.885000\du,10.350000\du)--(34.915000\du,10.350000\du)--(34.915000\du,8.350000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (32.400000\du,9.590000\du){Vulnerabilities};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
{\pgfsetcornersarced{\pgfpoint{0.000000\du}{0.000000\du}}\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.550000\du,8.250000\du)--(27.550000\du,7.000000\du)--(32.400000\du,7.000000\du)--(32.400000\du,8.350000\du);
}}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (18.000000\du,5.025000\du)--(18.000000\du,7.725000\du)--(21.750000\du,7.725000\du)--(21.750000\du,5.025000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (18.000000\du,5.025000\du)--(18.000000\du,7.725000\du)--(21.750000\du,7.725000\du)--(21.750000\du,5.025000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (19.875000\du,6.215000\du){Data};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (19.875000\du,7.015000\du){Size};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (17.500000\du,8.600000\du)--(17.500000\du,11.300000\du)--(23.162500\du,11.300000\du)--(23.162500\du,8.600000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (17.500000\du,8.600000\du)--(17.500000\du,11.300000\du)--(23.162500\du,11.300000\du)--(23.162500\du,8.600000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (20.331250\du,9.790000\du){Denormalization};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (20.331250\du,10.590000\du){};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (18.915600\du,8.600000\du)--(18.937500\du,7.725000\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (22.000000\du,5.100000\du)--(22.000000\du,9.250000\du)--(26.900000\du,9.250000\du)--(26.900000\du,5.100000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (24.450000\du,7.015000\du){Software};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (24.450000\du,7.815000\du){Evolution};
\end{tikzpicture}


==> figs/db-vs-ap.tex <==
% Graphic for TeX using PGF
% Title: /Users/boazrosenan/LOP-Private/ecoop18/db-vs-ap.dia
% Creator: Dia v0.97.2
% CreationDate: Thu Dec  7 20:09:29 2017
% For: boazrosenan
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.435008\du}{5.219722\du}}{\pgfpoint{3.546295\du}{0\du}}{\pgfpoint{0\du}{3.300000\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.435008\du}{5.219722\du}}{\pgfpoint{3.546295\du}{0\du}}{\pgfpoint{0\du}{3.300000\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (54.435008\du,5.462222\du){};
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (47.969591\du,0.234115\du)--(49.446089\du,1.633647\du)--(47.969591\du,3.033178\du)--(46.493092\du,1.633647\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (47.969591\du,0.234115\du)--(49.446089\du,1.633647\du)--(47.969591\du,3.033178\du)--(46.493092\du,1.633647\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (47.969591\du,1.752119\du){Client};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{48.707840\du}{2.333412\du}}
\pgfpathcurveto{\pgfpoint{49.587490\du}{2.748564\du}}{\pgfpoint{49.533676\du}{3.233155\du}}{\pgfpoint{51.137381\du}{3.883155\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{48.672448\du}{6.696898\du}}
\pgfpathcurveto{\pgfpoint{49.097448\du}{6.390648\du}}{\pgfpoint{49.361812\du}{6.028636\du}}{\pgfpoint{50.890516\du}{5.784886\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{59.024212\du}{6.074747\du}}
\pgfpathcurveto{\pgfpoint{58.832713\du}{5.805216\du}}{\pgfpoint{58.545358\du}{5.737000\du}}{\pgfpoint{57.999063\du}{5.668250\du}}
\pgfusepath{stroke}
}
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (47.890302\du,5.860972\du)--(49.366800\du,7.260503\du)--(47.890302\du,8.660034\du)--(46.413803\du,7.260503\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (47.890302\du,5.860972\du)--(49.366800\du,7.260503\du)--(47.890302\du,8.660034\du)--(46.413803\du,7.260503\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (47.890302\du,7.378975\du){Client};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (59.722802\du,5.461788\du)--(61.406800\du,7.058003\du)--(59.722802\du,8.654218\du)--(58.038803\du,7.058003\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (59.722802\du,5.461788\du)--(61.406800\du,7.058003\du)--(59.722802\du,8.654218\du)--(58.038803\du,7.058003\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (59.722802\du,7.176475\du){Attacker};
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.418803\du}{5.213472\du}}{\pgfpoint{3.287500\du}{0\du}}{\pgfpoint{0\du}{3.025000\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.200000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.418803\du}{5.213472\du}}{\pgfpoint{3.287500\du}{0\du}}{\pgfpoint{0\du}{3.025000\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (54.418803\du,5.455972\du){};
\definecolor{dialinecolor}{rgb}{0.800000, 1.000000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.418803\du}{5.213472\du}}{\pgfpoint{2.475000\du}{0\du}}{\pgfpoint{0\du}{2.162500\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 1.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{54.418803\du}{5.213472\du}}{\pgfpoint{2.475000\du}{0\du}}{\pgfpoint{0\du}{2.162500\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (54.418803\du,5.455972\du){};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (55.013446\du,3.488472\du)--(55.324160\du,3.488472\du)--(55.531303\du,3.750972\du)--(55.324160\du,4.013472\du)--(55.013446\du,4.013472\du)--(54.806303\du,3.750972\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (55.013446\du,3.488472\du)--(55.324160\du,3.488472\du)--(55.531303\du,3.750972\du)--(55.324160\du,4.013472\du)--(55.013446\du,4.013472\du)--(54.806303\du,3.750972\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (55.013446\du,3.488472\du)--(55.324160\du,3.488472\du)--(55.531303\du,3.750972\du)--(55.324160\du,4.013472\du)--(55.013446\du,4.013472\du)--(54.806303\du,3.750972\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (52.909639\du,3.710972\du)--(53.220353\du,3.710972\du)--(53.427496\du,3.973472\du)--(53.220353\du,4.235972\du)--(52.909639\du,4.235972\du)--(52.702496\du,3.973472\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (52.909639\du,3.710972\du)--(53.220353\du,3.710972\du)--(53.427496\du,3.973472\du)--(53.220353\du,4.235972\du)--(52.909639\du,4.235972\du)--(52.702496\du,3.973472\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (52.909639\du,3.710972\du)--(53.220353\du,3.710972\du)--(53.427496\du,3.973472\du)--(53.220353\du,4.235972\du)--(52.909639\du,4.235972\du)--(52.702496\du,3.973472\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (52.867139\du,5.833472\du)--(53.177853\du,5.833472\du)--(53.384996\du,6.095972\du)--(53.177853\du,6.358472\du)--(52.867139\du,6.358472\du)--(52.659996\du,6.095972\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (52.867139\du,5.833472\du)--(53.177853\du,5.833472\du)--(53.384996\du,6.095972\du)--(53.177853\du,6.358472\du)--(52.867139\du,6.358472\du)--(52.659996\du,6.095972\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (52.867139\du,5.833472\du)--(53.177853\du,5.833472\du)--(53.384996\du,6.095972\du)--(53.177853\du,6.358472\du)--(52.867139\du,6.358472\du)--(52.659996\du,6.095972\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (55.549639\du,5.980972\du)--(55.860353\du,5.980972\du)--(56.067496\du,6.243472\du)--(55.860353\du,6.505972\du)--(55.549639\du,6.505972\du)--(55.342496\du,6.243472\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (55.549639\du,5.980972\du)--(55.860353\du,5.980972\du)--(56.067496\du,6.243472\du)--(55.860353\du,6.505972\du)--(55.549639\du,6.505972\du)--(55.342496\du,6.243472\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (55.549639\du,5.980972\du)--(55.860353\du,5.980972\du)--(56.067496\du,6.243472\du)--(55.860353\du,6.505972\du)--(55.549639\du,6.505972\du)--(55.342496\du,6.243472\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (57.872021\du,0.961802\du){Access Control};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (57.872021\du,1.623806\du){Business Logic};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (57.872021\du,2.285809\du){Database};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (57.872021\du,2.947813\du){User Data};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,0.961802\du)--(56.387524\du,2.671396\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,1.623806\du)--(56.138803\du,3.079722\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,2.285809\du)--(56.152789\du,3.671731\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,2.947813\du)--(55.902821\du,5.964697\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (57.872021\du,0.299798\du){Server Boundaries};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,0.299798\du)--(56.330046\du,2.374190\du);
}
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (55.813803\du,2.842222\du)--(55.813803\du,3.317222\du)--(56.138803\du,3.317222\du)--(56.138803\du,2.842222\du)--cycle;
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetstrokecolor{dialinecolor}
\draw (55.813803\du,2.842222\du)--(55.813803\du,3.317222\du)--(56.138803\du,3.317222\du)--(56.138803\du,2.842222\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (50.105331\du,-0.243556\du)--(50.105331\du,0.683244\du)--(55.945243\du,0.683244\du)--(55.945243\du,-0.243556\du)--cycle;
\definecolor{dialinecolor}{rgb}{1.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (50.105331\du,-0.243556\du)--(50.105331\du,0.683244\du)--(55.945243\du,0.683244\du)--(55.945243\du,-0.243556\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (53.025287\du,0.366094\du){Application Code};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.800000, 1.000000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (50.127884\du,0.877988\du)--(50.127884\du,1.804788\du)--(55.958618\du,1.804788\du)--(55.958618\du,0.877988\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 1.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (50.127884\du,0.877988\du)--(50.127884\du,1.804788\du)--(55.958618\du,1.804788\du)--(55.958618\du,0.877988\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (53.043251\du,1.487638\du){3rd-party Code};
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,0.099182\du)--(57.711527\du,0.500414\du)--(58.032514\du,0.500414\du)--(58.032514\du,0.099182\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,0.761185\du)--(57.711527\du,1.162418\du)--(58.032514\du,1.162418\du)--(58.032514\du,0.761185\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,1.423189\du)--(57.711527\du,1.824422\du)--(58.032514\du,1.824422\du)--(58.032514\du,1.423189\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,2.085193\du)--(57.711527\du,2.486426\du)--(58.032514\du,2.486426\du)--(58.032514\du,2.085193\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (57.711527\du,2.747197\du)--(57.711527\du,3.148429\du)--(58.032514\du,3.148429\du)--(58.032514\du,2.747197\du)--cycle;
\end{tikzpicture}


==> figs/db-vs-ap2.tex <==
% Graphic for TeX using PGF
% Title: /Users/boazrosenan/LOP-Private/ecoop18/db-vs-ap2.dia
% Creator: Dia v0.97.2
% CreationDate: Thu Dec  7 20:09:19 2017
% For: boazrosenan
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.686205\du}{6.503750\du}}{\pgfpoint{3.546295\du}{0\du}}{\pgfpoint{0\du}{3.300000\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.686205\du}{6.503750\du}}{\pgfpoint{3.546295\du}{0\du}}{\pgfpoint{0\du}{3.300000\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (23.686205\du,6.746250\du){};
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (17.220788\du,1.518144\du)--(18.697286\du,2.917675\du)--(17.220788\du,4.317206\du)--(15.744289\du,2.917675\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (17.220788\du,1.518144\du)--(18.697286\du,2.917675\du)--(17.220788\du,4.317206\du)--(15.744289\du,2.917675\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (17.220788\du,3.036147\du){Client};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{17.959037\du}{3.617441\du}}
\pgfpathcurveto{\pgfpoint{18.838687\du}{4.032592\du}}{\pgfpoint{18.784873\du}{4.517184\du}}{\pgfpoint{20.388577\du}{5.167184\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{17.923644\du}{7.980926\du}}
\pgfpathcurveto{\pgfpoint{18.348644\du}{7.674676\du}}{\pgfpoint{18.613008\du}{7.312665\du}}{\pgfpoint{20.141713\du}{7.068915\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{28.275408\du}{7.358776\du}}
\pgfpathcurveto{\pgfpoint{28.083910\du}{7.089245\du}}{\pgfpoint{27.796555\du}{7.021028\du}}{\pgfpoint{27.250259\du}{6.952278\du}}
\pgfusepath{stroke}
}
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (17.141498\du,7.145000\du)--(18.617997\du,8.544531\du)--(17.141498\du,9.944063\du)--(15.665000\du,8.544531\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (17.141498\du,7.145000\du)--(18.617997\du,8.544531\du)--(17.141498\du,9.944063\du)--(15.665000\du,8.544531\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (17.141498\du,8.663004\du){Client};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (28.973998\du,6.745817\du)--(30.657997\du,8.342031\du)--(28.973998\du,9.938246\du)--(27.290000\du,8.342031\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (28.973998\du,6.745817\du)--(30.657997\du,8.342031\du)--(28.973998\du,9.938246\du)--(27.290000\du,8.342031\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (28.973998\du,8.460504\du){Attacker};
\definecolor{dialinecolor}{rgb}{0.800000, 1.000000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.670000\du}{6.497500\du}}{\pgfpoint{3.287500\du}{0\du}}{\pgfpoint{0\du}{3.025000\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.200000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 1.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.670000\du}{6.497500\du}}{\pgfpoint{3.287500\du}{0\du}}{\pgfpoint{0\du}{3.025000\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (23.670000\du,6.740000\du){};
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.870858\du}{6.352508\du}}{\pgfpoint{1.529431\du}{0\du}}{\pgfpoint{0\du}{0.827117\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.070000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{23.870858\du}{6.352508\du}}{\pgfpoint{1.529431\du}{0\du}}{\pgfpoint{0\du}{0.827117\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (23.870858\du,6.595008\du){};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (24.264643\du,4.772500\du)--(24.575357\du,4.772500\du)--(24.782500\du,5.035000\du)--(24.575357\du,5.297500\du)--(24.264643\du,5.297500\du)--(24.057500\du,5.035000\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.264643\du,4.772500\du)--(24.575357\du,4.772500\du)--(24.782500\du,5.035000\du)--(24.575357\du,5.297500\du)--(24.264643\du,5.297500\du)--(24.057500\du,5.035000\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.264643\du,4.772500\du)--(24.575357\du,4.772500\du)--(24.782500\du,5.035000\du)--(24.575357\du,5.297500\du)--(24.264643\du,5.297500\du)--(24.057500\du,5.035000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (22.160836\du,4.995000\du)--(22.471550\du,4.995000\du)--(22.678693\du,5.257500\du)--(22.471550\du,5.520000\du)--(22.160836\du,5.520000\du)--(21.953693\du,5.257500\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (22.160836\du,4.995000\du)--(22.471550\du,4.995000\du)--(22.678693\du,5.257500\du)--(22.471550\du,5.520000\du)--(22.160836\du,5.520000\du)--(21.953693\du,5.257500\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (22.160836\du,4.995000\du)--(22.471550\du,4.995000\du)--(22.678693\du,5.257500\du)--(22.471550\du,5.520000\du)--(22.160836\du,5.520000\du)--(21.953693\du,5.257500\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (22.118336\du,7.117500\du)--(22.429050\du,7.117500\du)--(22.636193\du,7.380000\du)--(22.429050\du,7.642500\du)--(22.118336\du,7.642500\du)--(21.911193\du,7.380000\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (22.118336\du,7.117500\du)--(22.429050\du,7.117500\du)--(22.636193\du,7.380000\du)--(22.429050\du,7.642500\du)--(22.118336\du,7.642500\du)--(21.911193\du,7.380000\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (22.118336\du,7.117500\du)--(22.429050\du,7.117500\du)--(22.636193\du,7.380000\du)--(22.429050\du,7.642500\du)--(22.118336\du,7.642500\du)--(21.911193\du,7.380000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (24.800836\du,7.265000\du)--(25.111550\du,7.265000\du)--(25.318693\du,7.527500\du)--(25.111550\du,7.790000\du)--(24.800836\du,7.790000\du)--(24.593693\du,7.527500\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.800836\du,7.265000\du)--(25.111550\du,7.265000\du)--(25.318693\du,7.527500\du)--(25.111550\du,7.790000\du)--(24.800836\du,7.790000\du)--(24.593693\du,7.527500\du)--cycle;
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.800836\du,7.265000\du)--(25.111550\du,7.265000\du)--(25.318693\du,7.527500\du)--(25.111550\du,7.790000\du)--(24.800836\du,7.790000\du)--(24.593693\du,7.527500\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.493474\du,1.773817\du){Access Control};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.493474\du,2.675253\du){Application Platform};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.493474\du,4.023395\du){Business Logic};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.493474\du,4.686766\du){User Data};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,1.773817\du)--(25.639210\du,3.958059\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,2.675253\du)--(25.416749\du,4.497494\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,4.023395\du)--(24.789377\du,6.110474\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,4.686766\du)--(25.190295\du,7.284182\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.493474\du,1.099746\du){Server Boundaries};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,1.099746\du)--(25.599516\du,3.668495\du);
}
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.800000, 1.000000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (25.091749\du,4.259994\du)--(25.091749\du,4.734994\du)--(25.416749\du,4.734994\du)--(25.416749\du,4.259994\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.800000, 1.000000, 0.800000}
\pgfsetstrokecolor{dialinecolor}
\draw (25.091749\du,4.259994\du)--(25.091749\du,4.734994\du)--(25.416749\du,4.734994\du)--(25.416749\du,4.259994\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,0.899130\du)--(27.332981\du,1.300363\du)--(27.653967\du,1.300363\du)--(27.653967\du,0.899130\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,1.573201\du)--(27.332981\du,1.974434\du)--(27.653967\du,1.974434\du)--(27.653967\du,1.573201\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,2.474637\du)--(27.332981\du,2.875870\du)--(27.653967\du,2.875870\du)--(27.653967\du,2.474637\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,3.822779\du)--(27.332981\du,4.224011\du)--(27.653967\du,4.224011\du)--(27.653967\du,3.822779\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.332981\du,4.486150\du)--(27.332981\du,4.887383\du)--(27.653967\du,4.887383\du)--(27.653967\du,4.486150\du)--cycle;
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetfillcolor{dialinecolor}
\fill (24.464377\du,6.110474\du)--(24.464377\du,6.585474\du)--(24.789377\du,6.585474\du)--(24.789377\du,6.110474\du)--cycle;
\definecolor{dialinecolor}{rgb}{1.000000, 0.800000, 0.800000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.464377\du,6.110474\du)--(24.464377\du,6.585474\du)--(24.789377\du,6.585474\du)--(24.789377\du,6.110474\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (27.484688\du,3.324110\du){Integrity Control};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.324195\du,3.324110\du)--(24.697096\du,5.627940\du);
}
\pgfsetlinewidth{0.000000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.324195\du,3.123494\du)--(27.324195\du,3.524726\du)--(27.645181\du,3.524726\du)--(27.645181\du,3.123494\du)--cycle;
\end{tikzpicture}


==> mi-axiom.tex <==
\newpage
\sloppy
~\\~\\
\centerline{\Huge\bf Supplementary Materials}
~\\~\\
%\begin{quote}\emph{``[A]uthors may attach anonymous supplementary material to a submission, on the understanding that reviewers may choose not to look at it.''}\end{quote}
%\setcounter{tocdepth}{1}
%\tableofcontents
\contentsline {section}{\numberline {B}Permacde}{25}{appendix.B}
\contentsline {section}{\numberline {C}axiom-cljs.core}{33}{appendix.C}
\contentsline {section}{\numberline {D}gateway.core}{47}{appendix.D}
\contentsline {section}{\numberline {E}Intersection Sets}{74}{appendix.E}
\contentsline {section}{\numberline {F}migrator.core}{78}{appendix.F}
\contentsline {section}{\numberline {G}Event Processing }{100}{appendix.G}
\newpage
\input{axiom/permacode}
\newpage
\input{axiom/axiom-cljs}
\newpage
\input{axiom/gateway}
\newpage
\input{axiom/cloudlog.interset}
\newpage
\input{axiom/migrator}
\newpage
\input{axiom/cloudlog-events}


==> mi-grammar.tex <==
\begin{figure}
\begin{centering}
\fbox{%\parbox{\textwidth}{
\footnotesize
\begin{tabular}{rcl l}
        \NonTerm{fact} & ::= & \Term{[} \Regexp{keyword} \gterm{} \Many{\gterm{}} \Term{]} & Fact\\
 \gterm{} & ::= & \Regexp{keyword} | \Regexp{string} | \Regexp{number} | \Term{[} \Many{\gterm{}} \Term{]} & Ground term\\
%%
\factp{} & ::= & \Term{[} \Regexp{keyword} \NonTerm{term} \Many{\NonTerm{term}} \Term{]} & Fact pattern\\
        \NonTerm{term} & ::= & \Regexp{symbol} | \Regexp{string} | \Regexp{number} | \Regexp{keyword} | \Term{[} \Many{\NonTerm{term}} \Term{]} & Term\\
%%
  \ruledef{}   & ::= & \Term{(} \lstinline$clg/defrule$ \Regexp{symbol} \Term{[} \Many{\NonTerm{term}} \Term{]}
                              \factp{} \Many{\rulement{}} \Term{)} & Rule definition\\
  \rulement{} & ::= & \factp{} | \NonTerm{guard} & Rule element\\
%  \NonTerm{guard}     & ::= & \Term{(} \lstinline$clg/by$ \NonTerm{expr} \Term{)} | \dots & Guard\\
%%
%    \NonTerm{form} & ::= & \Term{(} \Regexp{symbol} \Many{\NonTerm{expr}} \NonTerm{expr} \Term{)} &Form\\
 \NonTerm{guard} & ::= & \NonTerm{by-guard} | \NonTerm{let-guard} | \NonTerm{for-guard} | \NonTerm{when-guard} | \NonTerm{when-not-guard} & Guard\\
 \NonTerm{by-guard} & ::= & \Term{(} \lstinline$clg/by$ \NonTerm{expr} \Term{)} & By guard\\
 \NonTerm{let-guard} &  ::=  & \Term{(} \lstinline$let$ \Term{[} \Many{\NonTerm{binding}} \Term{]} \Term{)} &Let guard\\
 \NonTerm{for-guard} &  ::=  & \Term{(} \lstinline$for$ \Term{[} \Many{\NonTerm{binding}} \Term{]} \Term{)} &For guard\\
 \NonTerm{when-guard} &  ::=  & \Term{(} \lstinline$when$ \NonTerm{bool-expr} \Term{)} & When guard\\
 \NonTerm{when-not-guard} &  ::=  & \Term{(} \lstinline$when-not$ \NonTerm{bool-expr} \Term{)} &When-not guard\\
  \clausdef{}     & ::= & \Term{(} \lstinline$clg/defclause$ \Regexp{symbol} \queryp{} 
                                  \Many{\rulement{}} \Term{)} & Clause definition\\
  \queryp{} & ::= & \Term{[} \Regexp{keyword} \Many{\NonTerm{term}} \: \lstinline$->$  \Many{\NonTerm{term}}\Term{]} &Query pattern\\
\end{tabular}
}%}
\end{centering}
\caption{Syntax for \clg{}, a DSL over \protect\Clojure{}, expressed in a dialect of EBNF}\label{fig:grammar}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{figure}

